Maximal Clique Enumeration with Hybrid Branching and Early Termination

Maximal clique enumeration (MCE) is crucial for tasks like community detection and biological network analysis. Existing algorithms typically adopt the branch-and-bound framework with the vertex-oriented Bron-Kerbosch (BK) branching strategy, which forms the sub-branches by expanding the partial clique with a vertex. In this paper, we present a novel approach called HBBMC, a hybrid framework combining vertex-oriented BK branching and edge-oriented BK branching, where the latter adopts a branch-and-bound framework which forms the sub-branches by expanding the partial clique with an edge. This hybrid strategy enables more effective pruning and helps achieve a worst-case time complexity better than the best known one under a condition that holds for the majority of real-world graphs. To further enhance efficiency, we introduce an early termination technique, which leverages the topological information of the graphs and constructs the maximal cliques directly without branching. Our early termination technique is applicable to all branch-and-bound frameworks. Extensive experiments demonstrate the superior performance of our techniques.

==> 0._abstract.tex <==
\begin{abstract}
    Maximal clique enumeration (MCE) is crucial for tasks like community detection and biological network analysis. Existing algorithms typically adopt the branch-and-bound framework with the vertex-oriented Bron-Kerbosch (BK) branching strategy, which forms the sub-branches by expanding the partial clique with a vertex. 
    % The state-of-the-arts have a time complexity no better than $O(\delta n \cdot 3^{\delta/3})$, where $n$ is the number of vertices in the graph and $\delta$ is the degeneracy of the graph. 
    {\chengc In this paper, we present} a novel approach, \texttt{HBBMC}, a hybrid framework combining vertex-oriented BK branching and edge-oriented BK branching, where the latter adopts a branch-and-bound framework which forms the sub-branches by expanding the partial clique with a edge. 
    This hybrid strategy enables more effective pruning {\chengc and helps achieve a worst-case time complexity better than the best-known one under a condition which holds for the majority of real-world graphs.}
    % with a worst-case time complexity of $O(\delta m + \tau m \cdot 3^{\tau/3})$, where $m$ is the number of edges in the graph and $\tau$ is related to the maximum truss number. This theoretical result is better than that of the state-of-the-arts when $\delta \ge \tau + \frac{3}{\ln 3}\ln \rho$, a condition satisfied by majority of real-world graphs, where $\rho=\frac{m}{n}$ is the edge density of the graph. 
    To further enhance efficiency, we introduce an early termination technique, which leverages the topological information of the graphs and constructs the maximal cliques directly without branching. 
    {\chengc Our early termination technique is} applicable to all branch-and-bound frameworks. 
    Extensive experiments 
    % on real and synthetic graphs 
    demonstrate the superior performance of our techniques. 
    % The proposed \texttt{HBBMC} algorithm with the early termination technique consistently outperforms existing algorithms.
    % Maximal clique enumeration (MCE) is crucial for tasks like community detection and biological network analysis. Existing algorithms typically adopt the branch-and-bound framework with the vertex-oriented Bron-Kerbosch (BK) branching strategy, which forms the sub-branches by expanding the partial clique with a vertex. The state-of-the-arts have a time complexity no better than $O(\delta n \cdot 3^{\delta/3})$, where $n$ is the number of vertices in the graph and $\delta$ is the degeneracy of the graph. We introduce a novel approach, \texttt{HBBMC}, a hybrid framework combining vertex-oriented BK branching and edge-oriented BK branching, where the latter adopts a branch-and-bound framework which forms the sub-branches by expanding the partial clique with a edge. This hybrid strategy enables more effective pruning, with a worst-case time complexity of $O(\delta m + \tau m \cdot 3^{\tau/3})$, where $m$ is the number of edges in the graph and $\tau$ is related to the maximum truss number. This theoretical result is better than that of the state-of-the-arts when $\delta \ge \tau + \frac{3}{\ln 3}\ln \rho$, a condition satisfied by majority of real-world graphs, where $\rho=\frac{m}{n}$ is the edge density of the graph. To further enhance efficiency, we introduce an early termination technique applicable to all branch-and-bound frameworks, which leverages the topological information of the graphs and constructs the maximal cliques directly without branching. Extensive experiments 
    % % on real and synthetic graphs 
    % demonstrate the superior performance of our techniques. 
    % % The proposed \texttt{HBBMC} algorithm with the early termination technique consistently outperforms existing algorithms.
\end{abstract}




 % {\color{red}***Place Holder***}
    % {\color{blue} 
    % $k$-clique listing is a vital graph mining operator with diverse applications in various networks. The state-of-the-art algorithms all adopt a branch-and-bound (BB) framework with a vertex-oriented branching strategy (called \texttt{VBBkC}), which forms a sub-branch by expanding a partial $k$-clique with a \emph{vertex}. These algorithms have the time complexity of $O(k\cdot m \cdot (\delta/2)^{k-2})$, where $m$ is the number of edges in the graph and $\delta$ is the degeneracy of graph. In this paper, we propose a BB framework with a new \emph{edge-oriented branching} (called \texttt{EBBkC}), which forms a sub-branch by expanding a partial $k$-clique with two vertices that connect each other (which correspond to an \emph{edge}). We explore various edge orderings for \texttt{EBBkC} such that it achieves a time complexity of $O(k\cdot m \cdot (\tau/2)^{k-2})$, where $\tau$ is an integer related to the maximum truss number of the graph and we have $\tau < \delta$. Furthermore, we develop specialized algorithms for sub-branches on dense graphs so that we can early-terminate them and apply the specialized algorithms. We conduct extensive experiments on 16 real graphs, and the results show that our newly developed \texttt{EBBkC} based algorithms with the early termination technique consistently and largely outperform the state-of-the-art (\texttt{VBBkC} based) algorithms.}
    % {\color{red}***Place Holder***}
    %$k$-clique listing is a significant graph mining operator with applications in diverse networks. Existing state-of-the-art algorithms employ a vertex-oriented branching strategy within a branch-and-bound (BB) framework, called \texttt{VBBkC}, resulting in a time complexity of $O(k\cdot m \cdot (\delta/2)^{k-2})$, where $m$ represents the number of edges in the graph and $\delta$ denotes the graph's degeneracy. In this paper, we propose a new BB framework, called \texttt{EBBkC}, with an edge-oriented branching strategy that expands a partial $k$-clique using two connected vertices (an edge). By exploring different edge orderings, \texttt{EBBkC} achieves a time complexity of $O(k\cdot m \cdot (\tau/2)^{k-2})$, where $\tau$ is an integer related to the maximum truss number of the graph, and we prove that $\tau < \delta$. Additionally, we introduce specialized algorithms for dense graph sub-branches, enabling early termination and improved performance. Extensive experiments on 16 real graphs demonstrate that our newly developed \texttt{EBBkC} algorithms, combined with the early termination technique, consistently outperform the state-of-the-art \texttt{VBBkC}-based algorithms by up to 2 orders of magnitude.}
    % Listing $k$-cliques of a graph is a fundamental problem in graph data analysis and has been used for many practical applications such as community detection and anomaly detection. While quite a few algorithms have been developed for improving both the theoretical and empirical performance, recent studies including the state-of-the-art all correspond to the same branch-and-bound framework and focus on sharpening the details of its implementation. As a result, they achieve the same time complexity of $O(k\cdot m \cdot (\delta/2)^{k-2})$ (where $m$ is the number of edges in the graph and $\delta$ is the degeneracy of graph) and have the comparable empirical performance. 
    % %
    % In this paper, we propose a new branch-and-bound framework called \texttt{EBBkC}, which differs from the existing one in the way of forming branches but is more powerful for listing $k$-cliques. Based on this framework, we develop three new branch-and-bound algorithms, among which, the best one called \texttt{EBBkC-H} improves the time complexity to $O(k\cdot m \cdot (\tau/2)^{k-2})$ where $\tau$ is a positive integer and is \emph{strictly smaller} than $\delta$ in theory. As verified in the experiments, the value of $\tau$ is around half of that of $\delta$ in the most of real graphs. We further introduce the early termination technique for boosting the empirical performance of the branch-and-bound algorithms.
    % %
    % We finally conduct extensive experiments on real datasets, and the results show that our algorithms are up to around 1-2 orders of magnitude faster than the state-of-the-art.
    % Listing $k$-cliques in a graph is a fundamental problem since it has a broad applications in community detection and dense subgraph pattern mining. 
    %
    % All existing studies impose an ordering to the vertices ahead the main listing procedure such that the whole graph can be converted in to a directed and acyclic graph, and each $k$-clique is associated with the vertex who has the highest priority. However, these algorithm fail to terminate in an affordable time when listing $k$-cliques in an input graph with some large dense structures. 
    %
    % To tackle this problem, we propose three techniques. First, we propose an effective index of the graph based on the truss decomposition, which can prune a large number of edges that cannot be in a $k$-clique in advance. Second, we propose an early-termination technique, which allows the algorithm to list all $k$-cliques efficiently without trapping into the dense structures as existing algorithms do. 
    % Third, we propose a novel vertex ordering policy, which is determined in a data-driven fashion, using a novel method based on reinforcement learning. 
    %
    % We conduct extensive experiments to verify that each technique has non-trivial contribution to the efficiency improvement. 
    % *******[Copied, Placeholder] As the popularity of graph data increases, there is a growing need to count the frequency of occurrence of subgraph patterns of interest, for a variety of applications. Many graphs are massive in scale and also fully dynamic (with insertions and deletions of edges), rendering exact computation of these counts to be infeasible. Common practice is, instead, to use a small set of edges as a sample to estimate the counts. Existing sampling algorithms for fully dynamic graphs sample the edges with uniform probability. In this paper, we show that we can do much better if we sample edges based on their individual properties. Specifically, we propose a weighted sampling algorithm called \texttt{WSD} for estimating the subgraph count in a fully dynamic graph stream, which sample the edges based on their weights that indicate their importance and reflect their properties. We determine the weights of edges in a data-driven fashion, using a novel method based on reinforcement learning. We conduct extensive experiments to verify that our technique can produce estimates with smaller errors while often running faster compared with existing algorithms.

==> 1._intro.tex <==

\section{Introduction}
\label{sec:intro}

Given a graph $G$, a clique is a complete subgraph of $G$ where any two vertices are connected by an edge. A clique is said to be \emph{maximal} if it is not a subgraph of another clique. Maximal clique enumeration (MCE), which is to enumerate all maximal cliques in a graph, is a fundamental graph problem and finds diverse applications across different networks, e.g., social networks, biological networks and Web networks. Some notable applications include the detection of the communities in social networks \cite{lu2018community, wen2016maximal}, the prediction of the functions of {\cheng proteins} in biological networks (where the vertices are the {\cheng proteins} and the edges are the interactions between proteins) \cite{yu2006predicting, matsunaga2009clique}. Moreover, maximal clique enumeration has 
% also 
{\cheng been} applied to other data mining tasks including document clustering \cite{augustson1970analysis}, image analysis and recovery \cite{horaud1989stereo}, and the discovery of frequent purchased item patterns in e-commerce \cite{zaki1997new}. 


Quite a few algorithms have been developed to solve {\cheng the} MCE problem \cite{tomita2006worst, eppstein2010listing, eppstein2013listing, li2019fast, naude2016refined, chang2013fast, conte2016sublinear, deng2023accelerating}, where most of these approaches adopt the \emph{branch-and-bound} (BB) framework \cite{tomita2006worst, eppstein2010listing, eppstein2013listing, li2019fast, naude2016refined, deng2023accelerating}. The framework involves a recursive procedure, which recursively partitions the search space (i.e., the set of all maximal cliques) into multiple sub-spaces via a conventional and widely-used branching strategy called Bron-Kerbosch (BK) branching \cite{bron1973algorithm}. Specifically, each branch $B$ is represented by a {\kaixin triplet} $(S, g_C, g_X)$, where the vertex set $S$ induces a partial clique that has been found so far, $g_C$ is the candidate graph where each vertex inside can be added to $S$ to form a larger clique and $g_X$ is the exclusion
% forbidden
graph where each vertex inside must be excluded from any maximal clique
% $S$ 
within the branch $B$. To enumerate the maximal cliques within $B$, a
set of sub-branches is created through branching operations. Each sub-branch expands $S$ 
% by adding 
{\chengc with}
a vertex $v$ from $g_C$, and updates $g_C$ and $g_X$ accordingly (by removing {\yui from $g_C$ and $g_X$ those} vertices that are not connected with $v$, respectively). This recursive process continues until $g_C$ has no vertex inside, at which point $S$ is reported as a maximal clique if $g_X$ also has no vertex inside; otherwise $S$ is not a maximal clique. Once the recursive process 
% returns $B$ from 
{\cheng finishes}
the branching step at $v$, the vertex $v$ is excluded from $S$ and moves to $g_X$. The original MCE problem on $G$ can be solved {\chengB by starting} from the initial branch $B=(S, g_C, g_X)$ with {\kaixinC $S$ being an empty set, $g_C$ being the graph $G$ and $g_X$ being an empty graph}. Since each branching step is conducted upon a vertex, we call it the \emph{vertex-oriented BK branching}. Correspondingly, we 
% term
{\chengc call}
the \underline{v}ertex-oriented BK branching based \underline{BB} framework for \underline{m}aximal \underline{c}lique enumeration as \texttt{VBBMC}. 


Existing studies target two directions to enhance the performance. One {\cheng direction} is to prune more sub-branches effectively \cite{tomita2006worst, naude2016refined}. A common practice is the \emph{pivoting} strategy. Given a branch $B=(S,g_C,g_X)$, instead of producing sub-branches {\cheng on} all vertices in $g_C$, the strategy first chooses a pivot vertex $u\in V(g_C)\cup V(g_X)$. Then the branches produced 
% on
{\chengc at}
$u$'s neighbors in $g_C$ can be safely pruned. The rationale is that those maximal cliques that have $u$’s neighbors inside either include $u$ ({\chengB in this case, they} can be enumerated from the branch produced at $u$) or include at least one $u$’s non-neighbors ({\chengB in this case, they} can be enumerated from the
branch produced {\cheng at} $u$’s non-neighbors). 
%
The other {\cheng direction} is to generate candidate graph instances with smaller {\cheng sizes} \cite{eppstein2010listing, eppstein2013listing, xu2014distributed}. When a vertex $v_i$ is added to $S$, the size of the candidate graph instance shrinks as the candidate graph instance in the sub-branch {\yui which} only considers $v_i$'s neighbors. Then it becomes possible to generate a set of sub-branches with 
% {\cheng as few} compressed 
{\chengc as shrunk}
candidate graph instances {\chengB as possible} by exploring different vertex orderings. For example, when the degeneracy ordering of $G$ is adopted at the universal branch, the maximum size of a sub-branch can be bounded by the degeneracy number $\delta$ of $G$, which is much smaller than the number of vertices $n$ in $G$ (i.e., $\delta\ll n$) \cite{eppstein2010listing, eppstein2013listing}. 
%
By 
% combining 
{\chengc employing}
the above two techniques, existing studies \cite{eppstein2010listing, eppstein2013listing} achieve the state-of-the-art time complexity of $O(n\delta\cdot 3^{\delta/3})$. 
% {\chengB While} 
{\chengc We note that while}
some recent research has improved the performance practically \cite{deng2023accelerating, li2019fast, jin2022fast}, {\chengB they do not achieve} a better theorectical {\cheng result}. 





Recently, we observe that another branching strategy called edge-oriented branching \cite{wang2024technical} has been 
% successfully adopted to 
{\cheng proposed for}
a related problem, namely $k$-clique
% \footnote{Given a graph $G$ and an integer $k>0$, a $k$-clique $g$ is a complete subgraph of $G$ with exactly $k$ vertices inside, i.e., $|V(g)|=k$.} 
listing \cite{chiba1985arboricity}, which aims to list all $k$-cliques in a graph $G$ {\chengc (a $k$-clique is a clique with $k$ vertices)}. Similarly, {\chengc in this branching,} each branch $B$ 
% of $k$-clique listing problem 
is 
% also 
associated with a partial clique $S$ and a candidate graph $g$, whose definitions are the same as those {\chengc for the MCE problem}. At a branching step,
% of $k$-clique listing problem, 
edge-oriented branching constructs a sub-branch by simultaneously including two vertices that are connected with each other (i.e., an edge) from $g$ to $S$. And the candidate graph in the sub-branch is updated to the subgraph of $g$ induced by the common neighbors of the vertices incident to the newly added edge. This strategy takes additional information of two vertices of an edge into account, which facilitates the formation of sub-branches with smaller {\cheng candidate} graphs. A nice property is that, by adopting a carefully specified ordering of edges (i.e., truss-based edge ordering \cite{wang2024technical}) at the initial branch, the largest size of a graph instance among the sub-branches can be bounded {\yui by} $\tau$, whose value is strictly smaller than the degeneracy $\delta$ of the graph $G$ (i.e., $\tau<\delta$). 



% Motivated by the above observations, we propose to 
{\chengB In this paper, we first}
migrate the edge-oriented branching strategy to {\cheng the} MCE problem. 
% Different from the recursive process in \texttt{VBBMC}, 
Given a branch $B=(S,g_C, g_X)$, 
% the 
{\chengc each}
sub-branch 
% also 
expands $S$ 
% by adding 
{\chengc with}
two vertices of an edge $e$ from $g_C$ {\chengB and} updates both $g_C$ and $g_X$ to be their subgraphs induced by the common neighbors of the two vertices incident to the edge $e$, respectively. Once the recursive process returns from the branching step at $e$, the edge $e$ is excluded from $S$ and moves to $g_X$. We call the above procedure \emph{edge-oriented BK branching}, and 
% denote 
{\chengc call}
the corresponding framework for MCE problem {\chengc as} \texttt{EBBMC}. While \texttt{EBBMC} inherits the advantage that the {\cheng sizes} of the candidate graph instances have a tigher upper bound $\tau$ with {\cheng the} truss-based edge ordering, it would explore $O(m\cdot 2^{\tau})$ sub-branches in the worst case, which undermines its superiority. 
%
To tackle this issue, we propose a hybrid branching framework, which 
% Specifically, we observe that 
jointly 
% combines 
{\chengc applies}
the vertex-oriented branching and the edge-oriented branching 
% can be jointly applied in certain cases 
so that more branches can be pruned. We show a BB algorithm that is based on the hybrid branching framework, which we call \texttt{HBBMC}, would have a worst-case time complexity of $O(\delta m + \tau m \cdot 3^{\tau/3})$. Compared with the existing algorithms, when the condition $\delta \ge \tau + \frac{3}{\ln 3}\ln \rho$ is satisfied, where $\rho=\frac{m}{n}$ is the edge density of the graph, our algorithm is asymptotically better than the state-of-the-art algorithms. We note that the condition holds for many
% almost all 
real-world graphs, {\chengB as we verify empirically}.
% {\chengc (details will be provided in Section~\ref{})}. 




To further enhance the efficiency of BB frameworks, we develop an early termination technique. The key idea is based on an observation that it would be efficient
% and straightforward 
to construct the maximal cliques directly {\chengB for} dense subgraphs without branching. For example, given a branch $B=(S,g_C,g_X)$ where the candidate graph $g_C$ is a clique and {\kaixin $g_X$ is an empty graph}, it is unnecessary to create sub-branches; instead, we can include all vertices in $g_C$ into $S$ directly.  
% and check the maximality of the induced clique. 
% However, the requirement of $g_C$ being a clique is stronger than necessary. 
% In fact, 
{\cheng Similarly,}
when $g_C$ is a 2-plex or 3-plex {\chengc (a graph $g$ is said to be a $t$-plex if each vertex $v\in V(g)$ has at most $t$ non-neighbors including itself)}, we can also efficiently construct the maximal cliques of $g_C$ in nearly optimal time. 
%
% To achieve this, 
{\chengc Specifically,}
we construct {\chengB a} complementary graph $\overline{g}_C$ of $g_C$, where the complementary graph $\overline{g}_C$ has the same set of vertices as $g_C$, with an edge between two vertices in $\overline{g}_C$ if and only if they are disconnected from each other in $g_C$. An interesting observation is that the inverse graph of a 2-plex or a 3-plex only has isolated vertices, simple paths or simple cycles. By using the topological information of the inverse graph $\overline{g}_C$, we can output all maximal cliques within the branch in the time proportional to the number of maximal cliques inside.
%
We note that the early termination technique is applicable to all BB frameworks (i.e., \texttt{VBBMC}, \texttt{EBBMC} and \texttt{HBBMC}) without impacting the worst-case time complexity of the BB frameworks.
% Although the BB algorithms with the early-termination technique would not have a better the time complexity under the worst case, 
% we provide a finer-grained analysis, showing that \texttt{HBBMC} (resp. \texttt{VBBMC}) with the early-termination technique would achieve an input-output sensitive time complexity of $O(\delta m + \tau m \cdot (\omega + 4^{\tau/4}))$ (resp. $O(\delta n \cdot (\omega + 4^{\delta/4}))$), where $\omega$ is the number of maximal cliques in $G$.






% instead of generating sub-branches upon vertices as \texttt{VBBMC} does, 
% When a new edge is added, the resulting branch can reduce the graph to
% one induced by the common neighbors of the two vertices, which is
% smaller compared to the graph generated by vertex-oriented branching. To achieve this, we explore an edge ordering technique based
% on truss decomposition [41], which we refer to as the truss-based
% edge ordering. This ordering aids in creating sub-branches with
% smaller graphs than those by vertex-oriented branching








\smallskip\noindent
\textbf{Contributions.} We summarize our contributions as follows.

\begin{itemize}[leftmargin=*]
    \item We propose a new algorithm \texttt{HBBMC} with a hybrid framework for the MCE problem, which integrates the vertex-oriented and the edge-oriented BK branching strategies. \texttt{HBBMC} has the worst-case time complexity of $O(\delta m + \tau m \cdot 3^{\tau/3})$. When $\delta \ge \tau + \frac{3}{\ln 3}\ln \rho$, which holds for many real-world graphs, \texttt{HBBMC} is asymptotically better than the state-of-the-art algorithms. (Section~\ref{sec:BBMC}) 
    
    \item {We further develop an early termination technique to enhance the efficiency of branch-and-bound frameworks including \texttt{HBBMC}, i.e., for branches with dense candidate graphs (e.g., $t$-plexes) and empty exclusion graphs, we develop algorithms to directly construct the maximal cliques based on the topological information of the inverse graphs, which would be faster. (Section~\ref{sec:early-termination})}
    
    \item We conduct extensive experiments on both real and synthetic graphs, and the results show that our \texttt{HBBMC} based algorithm with the early termination technique consistently outperforms the state-of-the-art (\texttt{VBBMC} based) algorithms. (Section~\ref{sec:exp}) 
\end{itemize}


% The rest of the paper is organized as follows. 
{\chengc In addition,} Section~\ref{sec:problem} reviews the problem and presents some preliminaries. 
% Section 3 summarizes the existing vertex-oriented branching-based BB framework. 
Section~\ref{sec:related} reviews the related work and Section~\ref{sec:conclusion} concludes the paper.




==> 2._problem.tex <==
\section{Problem and Preliminaries}
\label{sec:problem}

We consider an \emph{unweighted} and \emph{undirected} simple graph $G=(V,E)$, where $V$ is the set of vertices and $E$ is the set of edges. We denote by $n=|V|$ and $m=|E|$ the cardinalities of $V$ and $E$, respectively. Given $u,v\in V$, both $(u,v)$ and $(v,u)$ denote the undirected edge between $u$ and $v$. Given $u\in V$, we denote by $N(u,G)$ the set of neighbors of $u$ in $G$, i.e., $N(u,G)=\{v\in V\mid (u,v)\in E\}$ and define $d(u, G)=|N(u,G)|$.
%
Given $V_{sub}\subseteq V$, we use $N(V_{sub},G)$ to denote the common neighbors of vertices in $V_{sub}$, i.e., $N(V_{sub},G)=\{v\in V\mid \forall u\in V_{sub},\ (v,u)\in E\}$.
%, denote by $d_u(G)$ the degree of $u$ in $G$, i.e., $d_u(G)=|N_u(G)|$, and denote by $\Delta(G)$ the maximum degree of $G$, i.e., $\Delta(G)=\max_{u\in V}d_u(G)$. 
%We omit the symbol $G$ from the notations, {\cheng e.g., we write $N_u$, $d_u$ and $\Delta$,} when the context is clear.
%
Given $V_{sub}\subseteq V$, we denote by $G[V_{sub}]$ the subgraph of $G$ induced by $V_{sub}$, i.e., $G[V_{sub}]$ includes the set of vertices $V_{sub}$ and the set of edges $\{(u,v)\in E\mid u, v\in V_{sub}\}$.
%
Given $E_{sub}\subseteq E$, we denote by $G[E_{sub}]$ the subgraph of $G$ induced by $E_{sub}$, i.e., $G[E_{sub}]$ includes the set of edges $E_{sub}$ and the set of vertices $\{ v\in V \mid (v, \cdot) \in E_{sub} \}$.
%
Let $g$ be a subgraph of $G$ induced by either a vertex subset of $V$ or an edge subset of $E$. We denote by $V(g)$ and $E(g)$ its set of vertices and its set of edges, respectively.
%
% In this paper, we focus on a {\cheng widely-used} cohesive graph structure, namely clique~\cite{erdos1935combinatorial}, which is defined formally as below.

\begin{definition}[Clique~\cite{erdos1935combinatorial}]
A subgraph $g$ is said to be a clique if there exists an edge between every pair of vertices, i.e., $E(g)=\{(u,v)\mid u,v\in V(g), {\cheng u\neq v} \}$.
\end{definition}

% We note that 1-clique ($k=1$) and 2-clique ($k=2$) correspond to single vertex and single edge, respectively, {\cheng which are basic elements of a graph.} Therefore, we focus on those $k$-cliques with $k$ at least 3 (note that 3-clique is widely known as triangle and has found many applications \cite{ latapy2008main, ortmann2014triangle}).
%

Given a graph $G$, a clique $C$ is said to be maximal if there is no other clique $C'$ containing $C$, i.e., $V(C)\subseteq V(C')$. 

\begin{problem}
[Maximal Clique Enumeration~\cite{bron1973algorithm}]
Given a graph $G=(V,E)$ , the Maximal Clique Enumeration (MCE) problem aims to find all maximal cliques in $G$.
\end{problem}


{\kaixinC The maximal clique enumeration (MCE) problem is hard to solve since the number of maximal cliques in a graph could be exponential (e.g., $3^{n/3}$) in the worst case \cite{moon1965cliques}.}


% \smallskip
% \noindent\textbf{Remarks.} 
% The MCE problem is NP-hard~\cite{moon1965cliques} since the $n$-vertex \emph{Moon-Moser} graphs can have up to $3^{n/3}$ maximal cliques inside~\cite{moon1965cliques}. Thus, it is impossible to find a solution to enumerate all maximal cliques in these graphs with polynomial running time. 
% (2) For the rest of the paper, we assume that the graph $G$ is connected; since otherwise, we can {\cheng compute the connected components and} enumerate the maximal cliques in each connected component of $G$. 





% \smallskip
% \noindent\textbf{Remark.} The problem of listing all 3-cliques {\cheng (i.e., $k = 3$)}, known as \emph{triangle listing problem}, has been widely studied~\cite{latapy2008main,ortmann2014triangle}. There are many efficient algorithms proposed for triangle listing, which run in \emph{polynomial} time. We remark that these algorithms cannot be used to solve the general $k$-clique listing problem.


% {\kaixinB
% \smallskip
% We further review the following concepts used in this paper. 
% %several basic concepts, which will be frequently mentioned in this paper. 


% \begin{definition}[$k$-core \cite{seidman1983network}]
% {\yuiR A $k$-core of $G$ is a maximal 
% %(vertex induced)
% subgraph of $G$ such that every vertex has degree at least $k$.}
% %Given a graph $G$ and an integer $k>0$, a $k$-core, denoted by $C_k$, is a maximal induced subgraph of $G$ such that every vertex in $C_k$ has a degree no smaller than $k$, i.e., $d(u, C_k)\ge k$ for every $u\in C_k$.
% \end{definition}

% The degeneracy of a graph $G$, denoted by $\delta$, is the maximum value of $k$ such that there exists a non-empty $k$-core in $G$. 

% \begin{definition}[$k$-truss \cite{wang2012truss}]
% {\yuiR
% A $k$-truss of $G$ is a maximal 
% %(edge induced) 
% subgraph of $G$ in which every edge is part of at least $k-2$ triangles.}
% %Given a graph $G$ and an integer $k\ge 2$, a $k$-truss, denoted by $T_k$, is the maximal subgraph of $G$ in which every edge is contained in at least $k-2$ triangles within $T_k$.
% \end{definition}

% Similarly, the maximum truss number, denoted by $k_{\max}$, is the maximum value of $k$ such that there exists a non-empty $k$-truss in $G$. 

% }

==> 3._BK.tex <==




\section{Branch-and-bound Algorithms}
\label{sec:BBMC}


\subsection{The Existing Branch-and-bound {\cheng Framework}: \texttt{VBBMC}}
\label{subsec:VBBMC}

We first review a suite of \emph{branch-and-bound} algorithms for maximal clique enumeration \cite{tomita2006worst, eppstein2010listing, jin2022fast, li2019fast, deng2023accelerating, naude2016refined, xu2014distributed}, which adopt a 
% conventional and widely-used 
branching strategy called Bron-Kerbosch (BK) branching \cite{bron1973algorithm}. 
% Many algorithms have been proposed for maximal cliques enumeration problem in the literature . Most of them adopt a \emph{branch-and-bound} framework, i.e., Bron-Kerbosch framework , 
It recursively partitions the search space (i.e., the set of all maximal cliques in $G$) into several sub-spaces via \emph{branching} until some stopping {\cheng criteria} are satisfied \cite{li2019fast, jin2022fast, deng2023accelerating}. The rationale is that a maximal clique can be constructed by merging two smaller cliques, namely a partial clique $S$ and another clique {\cheng which} satisfies the maximality condition. Specifically, each branch $B$ can be represented as a triplet $(S, g_C, g_X)$, where 

\begin{itemize}[leftmargin=*]
    \item \textbf{set $S$} induces a partial clique found so far,
    \item \textbf{subgraph $g_C$} is induced by all candidate vertices that can form a larger clique with the vertices in $S$, and 
    \item \textbf{subgraph $g_X$} is induced by all {\kaixin exclusion}
    % forbidden 
    vertices that 
    {\cheng are excluded for forming cliques with $S$.}
    % cannot be participated in the new cliques with $S$.
\end{itemize}

\begin{algorithm}[t]
% \small
\caption{The vertex-oriented branching-based BB framework for maximal clique enumeration: \texttt{VBBMC}}
\label{alg:VBBMC}
\KwIn{A graph $G=(V,E)$.}
\KwOut{All maximal cliques within $G$.}
\SetKwFunction{List}{\textsf{VBBMC\_Rec}}
\SetKwProg{Fn}{Procedure}{}{}
% Let $v_1, \cdots, v_n$ be in the degeneracy ordering of $G$\;
% \For{each $v_i\in V(G)$}{
% $P_i\gets N(v_i)\cap \{v_1, \cdots, v_{i-1}\}$\;
% $X_i\gets N(v_i)\cap \{v_{i+1}, \cdots, v_n\}$\;
% \List{$\{v_i\}, P_i, X_i$}\;
% }
\List{$\emptyset, G, G[\emptyset]$}\;
\Fn{\List{$S, g_C, g_X$}} {
    % \tcc{Termination if $V(g_C)$, $V(g_X)$ are empty}
    \If{$V(g_C) \cup V(g_X)=\emptyset$}{
        \textbf{Output} a maximal clique $S$;
        \Return\;
    }
    % \tcc{Branching on the vertices}
    Let $g=G[V(g_C)\cup V(g_X)]$ and choose a pivot $u$ from $V(g)$\;
    \For{each $v_i\in V(g_C)$ based on a given vertex ordering}{
        \lIf{$(u,v_i)\in E(g)$}{\textbf{continue}}
        Create branch $B_i=(S_i,g_{C_i},g_{X_i})$ based on Eq.~(\ref{eq:vbb-branching})\;
        $g_{C_i}',~g_{X_i}'\gets$ Refine $g_{C_i}$ and $g_{X_i}$ by removing those vertices that are not adjacent to $S_i$\;
        \List{$S_i,g_{C_i}',g_{X_i}'$}\;
        % $P\gets P\setminus \{v\}$\;
        % $X\gets X\cup \{v\}$\;
    }
}
\end{algorithm}

Given a graph $G=(V,E)$, the algorithm starts from the universal search space with $S=\emptyset$, $g_C = G$ and $g_X = G[\emptyset]$. Consider the branching step at a branch $B=(S, g_C, g_X)$. Let $\langle v_1, v_2, \cdots, v_{|V(g_C)|} \rangle$ be an arbitrary ordering of the vertices in $g_C$. The branching step would produce $|V(g_C)|$ sub-branches, where the $i$-th branch, denoted by $B_i=(S_i, g_{C_i}, g_{X_i})$, includes $v_i$ to $S$ and excludes $\{v_1, v_2, \cdots, v_{i-1}\}$. 
% (and also those that are not adjacent to $v_i$). 
Formally, for $1\le i \le |V(g_C)|$, we have 
\begin{equation}
\label{eq:vbb-branching}
\begin{aligned}
    S_i&=S\cup \{v_i\}, \quad
    g_{C_i} = G[V(g_C)\setminus\{v_1, v_2 \cdots ,v_{i}\}], \\
    g_{X_i} &= G[V(g_X)\cup\{v_1, v_2\cdots, v_{i-1}\}]
\end{aligned}
\end{equation}
% where $\widehat{g}_{C_i}$ is a subgraph of $g_C$ induced by the set of vertices $\{v_i, v_{i+1}, \cdots, v_{|V(g_C)|}\}$ and $\widehat{g}_{X_i}$ is a subgraph of $G$ induced by the set of vertices $V(g_X) \cup\{v_1, v_2, \cdots, v_{i-1}\}$. 
We note that $g_{C_i}$ and $g_{X_i}$ can be further refined by removing those vertices that are not adjacent to $S_i$ since they cannot form any cliques with $S_i$ within the search space. 
The process continues until no vertex can be further included into $S$, i.e., $V(g_C)=\emptyset$, at which point $S$ is a maximal clique if $V(g_X)$ is also empty; otherwise, $S$ is not maximal. 
We call the above branching step \emph{vertex-oriented BK branching} since each sub-branch is formed by including a vertex to the set $S$. 
% Correspondingly, 
We 
% denote 
{\chengc call}
the {\chengB \underline{v}ertex-oriented \underline{b}ranch-and-\underline{b}ound framework for \underline{MC}E} 
{\chengc as} \texttt{VBBMC}. 
% We present the pseudo-code in Algorithm~\ref{alg:VBBMC}. 
% Specifically, it starts from $S=\emptyset$, $g_C=G$, $g_X=G[\emptyset]$, and recursively branches the search space following Eq.~(\ref{eq:vbb-branching}) until no vertex can be included into $S$, i.e., $V(g_C)=\emptyset$. If $V(g_X)$ is also empty, then $S$ is reported as a maximal clique. 
Furthermore, during the recursive process, the state-of-the-art algorithms \cite{tomita2006worst,eppstein2010listing,eppstein2013listing, xu2014distributed} usually adopt a pruning technique, called \emph{pivoting} strategy, {\cheng for pruning some branches}. Formally, given a branch $B=(S,g_C,g_X)$, instead of producing branches for all vertices in $g_C$, these algorithms first choose a vertex $v\in V(g_C)\cup V(g_X)$, which is called the \emph{pivot vertex}. They then create the branches only for $v$'s non-neighbors in $g_C$ (including $v$ itself if $v\in V(g_C)$), i.e., the branches produced on $v$'s neighbors are pruned. The rationale is that those maximal cliques that have $v$'s neighbors inside either include $v$ 
% (which can be enumerated from the branch produced at $v$) 
or include at least one {\cheng of} $v$'s non-neighbors, 
% (which can be enumerated from the {\cheng branches} produced at $v$'s non-neighbors), 
since otherwise, the clique is not maximal. 
%
% The branching can be {\cheng interpreted as} a recursive \emph{binary} {\cheng partitioning} process. Specifically, it first splits the current branch $B$ into two sub-branches based on $v_1$: one including $v_1$ (this is the branch $B_1$)
% , which will enumerate those maximal cliques in $B$ that include $v_1$) 
% and the other excluding $v_1$. For branch $B_1$, it also removes from $g_C$ those vertices that are not adjacent to $v_1$ since they cannot form any cliques with $v_1$. Then, it recursively splits the latter into two new sub-branches based on $v_2$: one including $v_2$ (this is the branch $B_2$)
% , which will enumerate those maximal cliques in $B$ that include $v_2$ but exclude $v_1$) 
% and the other excluding $v_2$. It continues this process, until the last branch {\cheng $B_{|V(g_C)|}$} is formed. In summary, branch $B_i$ {\cheng would} enumerate those maximal cliques in $B$ that include $v_i$ but exclude $\{v_1, \cdots, v_{i-1}\}$. Consequently, all maximal cliques in $B$ {\cheng would} be listed exactly once after branching.

% \begin{table}[t]
% \vspace{-4mm}
% \small
%     \centering
%     \caption{The worst-case time complexities of existing \texttt{VBBMC} algorithms, where $n$, $h$ and $\delta$ are the number of the vertices, the $h$-index and the degeneracy of the graph, respectively.}
%     \vspace{-3mm}
%     \begin{tabular}{c|c}
%     \hline
%        Algorithm name & Time complexity \\ \hline
%         \texttt{BK} \cite{bron1973algorithm} &  $O(n \cdot (3.14)^{n/3})$ \\
%         \texttt{BK\_Pivot} \cite{tomita2006worst}, \texttt{BK\_Ref} \cite{naude2016refined} & $O(n \cdot 3^{n/3})$ \\
%         \texttt{BK\_Degree} \cite{xu2014distributed} & $O(hn\cdot 3^{h/3})$ \\
%         \texttt{BK\_Degen} \cite{eppstein2010listing, eppstein2013listing} & $O(\delta n \cdot 3^{\delta / 3})$ \\
%         \texttt{BK\_Rcd} \cite{li2019fast}  & $O(\delta n \cdot 2^{\delta})$ \\ 
%         \texttt{BK\_Fac} \cite{jin2022fast} & $O(\delta n \cdot (3.14)^{\delta/3})$\\ \hline
%     \end{tabular}
%     \label{tab:complexity}
% \vspace{-6mm}
% \end{table}






% To reduce the maximum number of sub-branches within a branch, the vertex $v\in V(g_C)\cup V(g_X)$ that has the maximum number of neighbors in $g_C$ is usually selected as the pivot vertex. 


% Given the initial branch $B = (\emptyset, G, G[\emptyset])$, although the edge-oriented branching strategy can produce much smaller graph instance than those produced by vertex-oriented branching strategy, i.e., $\tau<\delta$ \cite{wang2023efficient}, \texttt{HBBMC-T} still produces much more branches than necessary. We observe that some existing studies of \texttt{VBBMC} algorithms \cite{tomita2006worst,naude2016refined} have successfully adopted an effective pruning technique for maximal clique enumeration, called \emph{pivoting} strategy. 

% Specifically, given a branch $B=(S,g_C,g_X)$, instead of producing branches for all vertices in $g_C$, these algorithms first choose a vertex $v\in V(g_C)\cup V(g_X)$, which is called the \emph{pivot vertex}. They then create the branches only for $v$'s non-neighbors in $g_C$ (including $v$ itself if $v\in V(g_C)$), i.e., the branches produced on $v$'s neighbors are pruned. The rationale is that those maximal cliques that have $v$'s neighbors inside either include $v$ (which can be enumerated from the branch produced at $v$) or include at least one $v$'s non-neighbors (which can be enumerated from the branch produced at $v$'s non-neighbors), since otherwise, the clique is not maximal. To reduce the maximum number of sub-branches within a branch, the vertex $v\in V(g_C)\cup V(g_X)$ that has the maximum number of neighbors in $g_C$ is usually selected as the pivot vertex. 


% Motivated by this, we apply the pivoting strategy to the \texttt{HBBMC} framework. Formally, consider an arbitrary branch $B=(S, g_C, g_X)$. Let $g$ be a subgraph of $G$ induced by the edges in $g_C$ and $g_X$, i.e., $g = G[E(g_C)\cup E(g_X)]$. We choose a pivot vertex $u\in V(g)$. Then for each vertex $v\in V(g_C)$, we can apply the following pruning rule.

% \begin{itemize}[leftmargin=*]
%     \item \textbf{Rule}: if $(u,v)\in E(g)$, the branch produced on $v$ can be pruned. 
% \end{itemize}

% Although this pruning rule has proven to be effective in existing studies, its benefit is not fully unleashed. To see this, consider the example in Figure~\ref{}. In existing studies, the



We present the pseudo-code in Algorithm~\ref{alg:VBBMC}. We remark that Algorithm~\ref{alg:VBBMC} only presents the algorithmic idea while the possible pruning techniques (e.g., detailed pivoting selection \cite{tomita2006worst, naude2016refined, jin2022fast} and graph reduction \cite{deng2023accelerating}) and detailed implementations (e.g., the data structures used for representing a branch \cite{eppstein2010listing, eppstein2013listing, li2019fast}) vary in existing algorithms. 
{\kaixinkdd {\chengB Different variants of \texttt{VBBMC} have different time complexities (which we summarize in the Appendix~\ref{sec:app-vbb-time}), among which the best time complexity is
% no algorithm achieves a better theoretical result than 
$O(n\delta \cdot 3^{\delta/3})$}, where $\delta$ is the degeneracy of the graph \cite{eppstein2010listing, eppstein2013listing}. }
% We note that \texttt{BK\_Rcd} \cite{li2019fast} and \texttt{BK\_Fac} \cite{jin2022fast} do not provide the worst-case time {\cheng complexity} analysis in their paper. We provide 
% such proofs and discussions 
% {\cheng the analysis}
% in {\kaixin Appendix~\ref{sec:app-vbb-time}}.
% technical report \cite{}. 
Some more details of variants of \texttt{VBBMC} will be provided in the related work (Section~\ref{sec:related}). 



% (resp. $\widehat{g}_i^-$) is a subgraph of induced by the set of vertices $\{v_{i}, v_{i+1}, \cdots, v_{|V(g)|}\}$ (resp. $\{v_1, v_2, \cdots, v_{i-1}\}$), i.e., $\widehat{g}_i = g[v_i,\cdots,v_{|V(g)|}]$. 


% \smallskip
% \noindent\textbf{Bottom-up Approach for MCE.}
%
% Most of existing solutions adopt a bottom-up approach for MCE, which starts from $S=\emptyset$, $g_C=G$, $g_X=G[\emptyset]$, and recursively branches the search space following Eq.~(\ref{eq:bk-branching}) until no vertex can be included into $S$, i.e., $V(g_C)=\emptyset$. If $V(g_X)$ is also empty, then $S$ is reported as a maximal clique. 
%
% To reduce the number of unnecessary recursive calls, Bron and Kerbosch \cite{bron1973algorithm} introduced a pivoting strategy, in which, instead of considering all candidate vertices in $g_C$, a pivot $u\in V(g_C)$ is first selected. Then only $u$ and its non-neighbors in $g_C$ are needed for branching. Tomita et al. \cite{tomita2006worst} improved the pivot selection by choosing the pivot from $V(g_C)\cup V(g_X)$ that maximizes $|N(u,g_C)|$ to reduce the maximum number of branches. The pseudo-code of this method is shown in Algorithm~\ref{alg:bkpivot}. Some recent studies extended \cite{tomita2006worst} by (1) exploring different vertex orderings for branching, e.g., degeneracy ordering \cite{eppstein2010listing, eppstein2013listing} or degree ordering \cite{xu2014distributed}, and (2) considering other pivot selection strategies for practical speedups \cite{naude2016refined, jin2022fast}. The details of these variants will be provided in the related work (Section~\ref{sec:related}). 


% \begin{algorithm}[t]
% \small
% \caption{Top-down Approach for MCE problem~\cite{li2019fast}}
% \label{alg:bkrcd}
% \KwIn{A graph $G=(V,E)$}
% \KwOut{All maximal cliques within $G$}
% \SetKwFunction{List}{\textsf{BK\_Rcd}}
% \SetKwProg{Fn}{Procedure}{}{}
% % Let $v_1, \cdots, v_n$ be in the degeneracy ordering of $G$\;
% % \For{each $v_i\in V(G)$}{
% % $P_i\gets N(v_i)\cap \{v_1, \cdots, v_{i-1}\}$\;
% % $X_i\gets N(v_i)\cap \{v_{i+1}, \cdots, v_n\}$\;
% % \List{$\{v_i\}, P_i, X_i$}\;
% % }
% \List{$\emptyset, G, G[\emptyset]$}\;
% \Fn{\List{$S, g_C, g_X$}} {
%     \tcc{Termination if $V(g_C)$, $V(g_X)$ are empty}
%     \If{$V(g_C)\cup V(g_X)=\emptyset$}{
%         \textbf{Output} a maximal clique $S$; \Return\;
%     }
%     \tcc{Branching when $P$ is not a clique}
%     \While{$g_C$ is not a clique}{
%         Choose $v$ from $g_C$ that minimizes $|N(u, g_C)|$\;
%         \List{$S\cup \{v\}, P\cap N(v), X\cap N(v)$}\;
%         $P\gets P\setminus \{v\}$\;
%         $X\gets X\cup \{v\}$\;
%     }
%     \tcc{Check maximality}
%     \If{$V(g_C)\neq \emptyset$ and $N(V(g_C), g_X)=\emptyset$}{
%             \textbf{Output} a maximal clique $S\cup V(g_C)$\;
%     }
    
% }
% \end{algorithm}

% \smallskip
% \noindent\textbf{Top-Down Approach for MCE.}
% In \cite{li2019fast}, Li et al. observed that when the candidate subgraph $g_C$ is dense, not all vertices in $g_C$ are needed for branching. Specifically, at the $i$-th branch, if the set of the vertices $\{v_i, v_{i+1}, \cdots, v_{|V(g_C)|}\}$ (i.e., $V(\widehat{g}_{C_i})$) already induces a clique, we can directly report $S\cup V(\widehat{g}_{C_i})$ as a maximal clique if it satisfies the maximality condition. The pseudo-code of this method is shown in Algorithm~\ref{alg:bkrcd}. However, this method has an intrinsic drawback. That is, in the sparse subgraphs, the algorithm would possibly create branches for all vertices in $g_C$. Therefore, its worst-case time complexity is worse than those pivot-based solutions. 


% To sum up, we call the branching step involved in all above methods \emph{vertex-oriented branching} since each sub-branch is formed by including a vertex to the set $S$ (if any). Correspondingly, we denote these vertex-oriented branch-and-bound frameworks for MCE by \texttt{VBBMC}. 
%
% We summarize the existing \texttt{VBBMC} algorithms and their corresponding time complexities in Table~\ref{tab:MCE-complexity}. We note that \texttt{BK\_Rcd} \cite{li2019fast} and \texttt{BK\_Fac} \cite{jin2022fast} do not provide the worst-case time complexities analysis in their paper. We provide such proofs and discussions in the technical report \cite{}. 






\subsection{A New Branch-and-bound Framework: \texttt{EBBMC}}
\label{subsec:EBBMC}


% Inspried by \cite{wang2023efficient}, 
{\chengB We} observe that there exists another {\cheng branching strategy} in which, given a branch $B=(S, g_C, g_X)$, the sub-branches can be created based on the \emph{edges} in $g_C$~\cite{wang2024technical}. We 
% denote 
{\chengc call}
the branching step involved in this approach 
% by 
{\chengc as}
\emph{edge-oriented branching}. Specifically, consider the branching step at $B$ and let $\langle e_1, e_2, \cdots, e_{|E(g_C)|}\rangle$ be an arbitrary edge ordering {\cheng for the edges in} $g_C$. Then the branching step would create $|E(g_C)|$ sub-branches from $B$, where the $i$-th branch, denoted by $B_i=(S_i, g_{C_i}, g_{X_i})$, includes the two vertices incident to the edge $e_i$, i.e., $V(e_i)$, and excludes from $g_C$ those edges in $\{e_1, e_2, \cdots, e_{i-1}\}$.
% (and those vertices that are disconnected from the vertices incident to $e_i$). 
Formally, for $1\le i\le |E(g_C)|$, we have
\begin{equation}
\label{eq:ebb-branching}
\begin{aligned}
    S_i &= S \cup V(e_i),\quad g_{C_i} = G[E(g_C)\setminus\{e_1, e_2, \cdots, e_{i}\}],\\
    g_{X_i} &= G[E(g_X)\cup \{e_1, e_2, \cdots, e_{i-1}\}],
\end{aligned}
\end{equation}
We note that $g_{C_i}$ and $g_{X_i}$ can be further refined by removing those vertices that are not adjacent to $S_i$.
% {\kaixinkdd
% In this case, $S_i$, $V(g'_{C_i})$ and $V(g'_{X_i})$ are also disjoint in \texttt{EBBMC}, where $g'_{C_i}$ (resp. $g'_{X_i}$) is the remaining graph of $g_{C_i}$ (resp. $g_{X_i}$) after refinement.}
% where $\overline{g}_{C_i}$ is a subgraph of $g_C$ induced by the set of edges $\{e_i, e_{i+1}, \cdots, e_{|E(g_C)|}\}$ and $\overline{g}_{X_i}$ is a subgraph of $G$ induced by the set of edges $E(g_X)\cup \{e_1, e_2, \cdots, e_{i-1}\}$. We note that $N(V(e_i),\overline{g}_{C_i})$ and $N(V(e_i),\overline{g}_{X_i})$ are to filter out those vertices that are not adjacent to the two vertices incident to $e_i$ since they cannot form any cliques with $e_i$.
%
% Similar to the vertex-oriented branching, the edge-oriented branching also corresponds to a recursive binary {\cheng partitioning} process: it first splits the current branch $B$ into two sub-branches based on $e_1$, where one includes {\kaixin $V(e_1)$}
% $V(e_i)$ 
% from $g_C$ to $S$ (this is branch $B_1$) and the other excludes the edge $e_1$ from $g_C$ and moves it to $g_X$. Then it recursively splits the latter into two sub-branches based on $e_2$, where one includes $V(e_2)$ from the remaining graph ${g}_{C}$ to $S$ (this is $B_2$) and the other excludes $e_2$ from ${g}_{C}$ and moves it to $g_{X}$. It continues the process until $B_{|E(g_C)|}$ is formed. 
% However,
{\chengB We note that}
given a branch $B$, the branching steps formulated by Eq.~(\ref{eq:ebb-branching}) do not always cover all maximal cliques in $B$ since there may exist some vertices whose degrees are zero in $g_C$ {\chengc (i.e., the vertices can be added to $S$ to form larger cliques, yet this cannot be achieved by expanding $S$ with any edges in $g_C$)}. 
% In other words, these vertices are not incident to any edges in $g_C$. 
%
{\kaixin
For example, when there are isolated vertices in $G$, they are also maximal cliques, i.e., 1-cliques. However, any branch produced by Eq.~(\ref{eq:ebb-branching}) does not cover these maximal cliques. In general, for the maximal cliques with their {\chengB sizes} being odd numbers, each edge-oriented branching step {\cheng would} involve two vertices to $S$ and finally there exists a branch $B=(S,g_C,g_X)$ in which there are isolated vertices in $g_C$.}
%
To enumerate all maximal cliques which include these vertices, we observe that no other vertices can be further added to $S$ after any of these zero-degree vertices is included in $S$. Thus, we can directly output these maximal cliques if they satisfy the maximality condition. 
% it is necessary to create several sub-branches via the vertex-oriented branching on these zero-degree vertices. 
Formally, let $Z(g_C)$ be the set of vertices in $g_C$ whose degrees are zero and let $\langle v_1, v_2, \cdots, v_{|Z(g_C)|} \rangle$ be an arbitrary vertex ordering. We create additional $|Z(g_C)|$ branches. For each entry $1\le j\le |Z(g_C)|$, the branch $B_j=(S_j, g_{C_j}, g_{X_j})$ is represented by
\begin{equation}
\label{eq:zbb-branching}
\begin{aligned}
    S_j &= S\cup \{v_j\}, \quad g_{C_j} = G[\emptyset], \\
    g_{X_j} &= \big(V_{C\cup X} \cup \{v_1, v_2, \cdots, v_{j-1}\}, E_{C\cup X}\big)
\end{aligned}
\end{equation}
We note that (1) $V_{C\cup X}$ (resp. $E_{C\cup X}$) is the vertex (resp. edge) set of the graph $g$, where $g$ is the subgraph of $G$ induced by the edge set $E(g_C)\cup E(g_X)$, (2) we can choose an arbitrary vertex ordering for the vertices in $Z(g_C)$ since the subgraph $g_{C_j}$ has no vertices or edges inside and (3) $g_{X_j}$ can be further refined by removing those vertices that are not adjacent to $S_j$. Then, if the graph $g_{X_j}$ has no vertex inside after refinement, $S_j$ induces a maximal clique; otherwise, $S_j$ is not a maximal clique. 
% $\widetilde{g}_{X_j}$ is a subgraph of $G$ where $V(\widetilde{g}_{X_j}) = V(g_X)\cup (V(g_C)\setminus Z(g_C)) \cup \{v_1, v_2, \cdots, v_{j-1}\}$ and $E(\widetilde{g}_{X_j}) = E(g_X)\cup E(g_C)$. We note that the vertex set $V(g_X)\cup (V(g_C)\setminus Z(g_C))$ (resp. the edge set $E(g_X)\cup E(g_C)$) consists of the vertices (resp. edges) that have been moved from $g_C$ to $g_X$ after the last branch $B_{|E(g_C)|}$ is produced via edge-oriented branching. 
In summary, with Eq.~(\ref{eq:ebb-branching}) and Eq.~(\ref{eq:zbb-branching}), {\chengc $|E(g_C)| + |Z(g_C)|$ branches would be formed, and} all maximal cliques in $B$ would be enumerated exactly once.



% explain these formula as follows. Consider the branching step on the last edge $e_{|E(g_C)|}$ with Eq.~(\ref{eq:ebb-branching}). It produces two sub-branches, where one includes $V(e_{|E(g_C)|})$ from $g_C$ to $S$ (this is the last branch produce by edge-oriented branching) and the other exclude exclues $V(e_{|E(g_C)|})$ from $g_C$ and moves them to $g_X$. Currently, $g_C$ consists of those vertices in $Z(g_C)$ and $g_X$ consists of $g_C$ and $g_X$ excluding those vertices in $Z(g_C)$




\begin{algorithm}[t]
% \small
\caption{The edge-oriented branching-based BB framework for maximal clique enumeration: \texttt{EBBMC}}
\label{alg:EBBMC}
\KwIn{A graph $G=(V,E)$.}
\KwOut{All maximal cliques within $G$.}
\SetKwFunction{List}{\textsf{EBBMC\_Rec}}
\SetKwProg{Fn}{Procedure}{}{}
% Let $v_1, \cdots, v_n$ be in the degeneracy ordering of $G$\;
% \For{each $v_i\in V(G)$}{
% $P_i\gets N(v_i)\cap \{v_1, \cdots, v_{i-1}\}$\;
% $X_i\gets N(v_i)\cap \{v_{i+1}, \cdots, v_n\}$\;
% \List{$\{v_i\}, P_i, X_i$}\;
% }
\List{$\emptyset, G, G[\emptyset]$}\;
\Fn{\List{$S, g_C, g_X$}} {
    % \tcc{Termination 1: $V(g_C)$, $V(g_X)$ are empty}
    \If{$V(g_C) \cup V(g_X)=\emptyset$}{
        \textbf{Output} a maximal clique $S$;
        \Return\;
    }

    % \tcc{Branching on the edges}
    % Choose  $u$ from $V(g_C)\cup V(g_X)$ that maximizes $|N(u, g_C)|$\;
    \For{each $e_i\in E(g_C)$ based on a given edge ordering}{
        Create branch $B_i=(S_i,g_{C_i},g_{X_i})$ based on Eq.~(\ref{eq:ebb-branching})\;
        $g_{C_i}',~g_{X_i}'\gets$ Refine $g_{C_i}$ and $g_{X_i}$ by removing those vertices that are not adjacent to $S_i$\;
        \List{$S_i,g_{C_i}',g_{X_i}'$}\;
        % $P\gets P\setminus \{v\}$\;
        % $X\gets X\cup \{v\}$\;
    }

    % \tcc{Termination 2: zero-degree vertices}
    \For{each $v_j \in Z(g_C)$}{
        Create branch $B_j=(S_j, g_{C_j}, g_{X_j})$ based on Eq.~(\ref{eq:zbb-branching})\;
        $g_{X_j}'\gets$ Refine $g_{X_j}$ by removing those vertices that are not adjacent to $S_j$\;
        \If{$V(g_{X_j}') = \emptyset$}{
            \textbf{Output} a maximal clique $S_j$
        }
    }
}
\end{algorithm}


We call the above branching strategy {\chengc as} \emph{edge-oriented BK branching} {\chengc since} it {\cheng is} mainly based on the edge-oriented branching strategy to {\cheng partition} a search space. 
% Correspondingly, 
We 
% denote 
{\chengc call}
the {\chengB \underline{e}dge-oriented \underline{b}ranch-and-\underline{b}ound framework for \underline{MC}E}
% the edge-oriented branch-and-bound framework for MCE 
% by 
{\chengc as}
\texttt{EBBMC}. The pseudo-code is shown in Algorithm~\ref{alg:EBBMC}. 
%
{\kaixin
Compared with edge-oriented branching strategy for $k$-clique listing problem (i.e., \texttt{EBBkC} framework) \cite{wang2024technical}, both frameworks are associated with a partial clique $S$ and a candidate subgraph, whose definitions are the same with each other.
{\kaixinkdd 
The major difference 
% between \texttt{EBBMC} and \texttt{EBBkC} 
is that in \texttt{EBBMC}, the maximal cliques can have a range of sizes, varying from the smallest one (e.g., a vertex, representing a maximal 1-clique) to the largest one ($\omega$-clique, where $\omega$ denotes the size of the maximum clique) while in \texttt{EBBkC}, all listed cliques are required to possess exactly $k$ vertices inside, with the value of $k$ being a pre-determined input.}
% However, in \texttt{EBBMC}, the maximal cliques can have different sizes, ranging from the smallest one, e.g., a vertex (1-clique) or an edge (2-clique), to the largest one ($\omega$-clique where $\omega$ is the size of a maximum clique) while in \texttt{EBBkC}, all cliques to be listed have exactly $k$ vertices inside, where the value of $k$ is the input and known in advance. 
% Thus, even though the isolated vertices may exist in the candidate subgraph of a branch in \texttt{EBBkC}, the branching step would still be conducted based on the edges if the termination condition is not satisfied (e.g., $|S|+1<k$). 
% This explains why Eq.~(\ref{eq:zbb-branching}) {\cheng applies to} \texttt{EBBMC} {\cheng only}. 
% % but not in \texttt{EBBkC}. 
{\chengB As a result, for \texttt{EBBkC}, the branching step would still be conducted based on the edges as long as $|S|+1<k$, no matter whether there exist isolated vertices in the candidate subgraph of the branch. 
% That is, 
{\chengc Therefore,}
the branching procedure represented in Eq.~(\ref{eq:zbb-branching}) is not necessary for \texttt{EBBkC}.}


% for \texttt{EBBMC}, Eq.~(\ref{eq:ebb-branching}) and Eq.~(\ref{eq:zbb-branching}) ensures the correctness for both even-size and odd-size maximal cliques. 


% However, the main difference is that \texttt{EBBMC} needs a exclusion subgraph $g_X$ for checking the maximality condition while \texttt{EBBkC} uses an integer $l$ to indicate how many remaining vertices should be further added to $S$. This difference further impacts how the algorithms are implemented. For example, in \texttt{EBBMC}, the algorithm terminates and returns when no vertex can be furether added to $S$ (i.e., $g_C$ is empty) while in \texttt{EBBkC}, the algorithm terminates and returns when $l=1$ or $l=2$

}






\noindent
\textbf{Ordering of the edges.} 
%
% Next, we consider the ordering of the edges for edge-oriented branching at a branch $B=(S,g_C,g_X)$. 
For a sub-branch $B_i$ produced from $B$, the size of the graph $g_{C_i}$ after the refinement (i.e., the number of the vertices in $g_{C_i}'$) is equal to the number of common neighbors of vertices in $V(e_i)$ in ${g}_{C_i}$ (line 7 of the Algorithm~\ref{alg:EBBMC}). That is
\begin{equation}
|V(g_{C_i}')| = |N(V(e_i), {g}_{C_i})|    
\end{equation}
where ${g}_{C_i}$ is defined in Eq.~(\ref{eq:ebb-branching}). 
To minimize the size of the graph instances for the sub-branches, as it would reduce the time costs for solving the current branch, we choose the \emph{truss-based edge ordering} \cite{wang2024technical} for branching. Specifically, the truss-based edge ordering can be obtained via a greedy procedure: it iteratively removes from the remaining $g_C$ the edge whose vertices have the smallest number of common neighbors and then adds it to the end of the ordering. By adopting the truss-based edge ordering, the largest size of a graph instance among all sub-branches created during the recursive procedure can be bounded by $\tau$, whose value is strictly smaller than the degeneracy number $\delta$ of the graph $G$ (i.e., $\tau<\delta$) \cite{wang2024technical}. 
% We present the pseudo-codes and the implementation details of \texttt{EBBMC} with truss-based edge ordering in Appendix~\ref{sec:app-bbmc}.
% \subsection{\texttt{EBBMC} with Truss-based Edge Ordering}
% \smallskip\noindent
% \textbf{The \texttt{EBBMC} algorithm.}
% We denote the algorithm of \texttt{HBBMC} with the truss-based edge ordering by \texttt{HBBMC-T}. 
The pseudo-code of \texttt{EBBMC} with truss-based edge ordering is presented in Algorithm~\ref{alg:EBBMC-T}. In particular, we only compute the truss-based edge ordering of $G$ (i.e., $\pi_{\tau}(G)$) for the branching at the initial branch (lines 2-5). Then, for any other branching step at a following branch $B=(S,g_C,g_X)$, edges in $g_C$ adopt the same ordering to those used in $\pi_{\tau}(G)$, which could differ with the truss-based edge ordering of $g_C$. 
Given a branch $B$ other than the initial branch, to create the sub-branches efficiently, we maintain four additional auxiliary sets for each edge in $G$, i.e., $V_+(\cdot)$, $E_+(\cdot)$, $V_-(\cdot)$ and $E_-(\cdot)$ (line 4). The idea is that for an edge $e$, all edges in $E_+(e)$ (resp. $E_-(e)$) are ordered behind (resp. before) $e$ in $\pi_{\tau}$ and the vertices incident to these edges are both connected with those incident to $e$, and $V_+(e)$ (resp. $V_-(e)$) is the set of the vertices in $G[E_+(e)]$ (resp. $G[E_-(e)]$). Therefore, the branching steps can be efficiently conducted via
set intersections (line 9). The correctness of this implementation can be easily verified.



\begin{algorithm}[t]
% \small
\caption{\texttt{EBBMC} with truss-based edge ordering}
\label{alg:EBBMC-T}
\KwIn{A graph $G=(V,E)$.}
\KwOut{All maximal cliques within $G$.}
\SetKwFunction{List}{\textsf{EBBMC-T\_Rec}}
\SetKwProg{Fn}{Procedure}{}{}
% Let $v_1, \cdots, v_n$ be in the degeneracy ordering of $G$\;
% \For{each $v_i\in V(G)$}{
% $P_i\gets N(v_i)\cap \{v_1, \cdots, v_{i-1}\}$\;
% $X_i\gets N(v_i)\cap \{v_{i+1}, \cdots, v_n\}$\;
% \List{$\{v_i\}, P_i, X_i$}\;
% }
% \tcc{Initialize branches from $G$}
$\pi_{\tau}(G)\gets$ the truss-based ordering of edges in $G$\;
\For{each edge $e_i\in E(G)$ following $\pi_{\tau}(G)$}{
    Obtain $S_i$, $g_{C_i}'$ and $g_{X_i}'$ (lines 6-7 of Algorithm~\ref{alg:EBBMC})\;
    % Create branch $B_i=(S_i,g_{C_i},g_{X_i})$ based on Eq.~(\ref{eq:ebb-branching})\;
    % $g_{C_i}',~g_{X_i}'\gets$ Refine $g_{C_i}$ and $g_{X_i}$ by removing those vertices that are not adjacent to $S_i$\;
    Initialize $V_+(e_i)\gets V(g_{C_i}')$, $E_+(e_i)\gets E(g_{C_i}')$, $V_-(e_i)\gets V(g_{X_i}')$ and $E_-(e_i)\gets E(g_{X_i}')$\;
    \List{$S_i,g_{C_i}',g_{X_i}'$}\;
}
Conduct Termination (lines 9-12 of Algorithm~\ref{alg:EBBMC})\;
\Fn{\List{$S, g_C, g_X$}} {
    Conduct Termination (lines 3-4 and 9-12 of Algorithm~\ref{alg:EBBMC});
    
    % \tcc{Branching on the edges}
    \For{each edge $e\in E(g_C)$}{
        $S'\gets S\cup V(e)$,~$g_C'\gets \big(V(g_C)\cap V_+(e), E(g_C)\cap E_+(e)\big)$ and $g_X'\gets \big(V(g_X)\cap V_-(e), E(g_X)\cap E_-(e)\big)$\;
        \List{$S',g_{C}',g_{X}'$}\;
        $E(g_C)\gets E(g_C)\setminus\{e\}$ and $E(g_X)\gets E(g_X)\cup \{e\}$\;
        % $P\gets P\setminus \{v\}$\;
        % $X\gets X\cup \{v\}$\;
    }
}
\end{algorithm}




% \subsection{Proof of Theorem~\ref{theo:ebbmc}}












% There are two benefits of $\pi_{\tau}$. First, given a branch $B=(S,g_C,g_X)$, the largest size of a produced graph instance with the truss-based edge ordering, denoted by $\tau(g_C)$, is strictly smaller than the degeneracy of the graph $\delta(g_C)$, i.e., $\tau(g_C)<\delta(g_C)$ \cite{wang2023efficient}. This would have a significant impact on the time complexity (details can be found in Section~\ref{}). Second, the edge ordering would provide more information of the graph, which provide the opportunity to prune more branches (details can be found in Section~\ref{}). 

% \smallskip\noindent
% \textbf{Complexity.} Given the graph $G=(V,E)$, let $\tau$ be the largest size of a produced graph instance via branching, i.e., $\tau = \max_{e_i\in E} |V(g_{C_i}')|$. Then we have the following theorem. 


\begin{theorem}
\label{theo:ebbmc}
    Given a graph $G=(V,E)$, the time and space complexities of \texttt{EBBMC} with {\cheng the} truss-based edge ordering are $O(\delta m +\tau m \cdot 2^{\tau})$ and $O(m+n)$, respectively.  
\end{theorem}

\begin{proof}
    % Consider the time complexity. 
    \texttt{EBBMC} first needs $O(\delta m)$ time to obtain the truss-based edge ordering \cite{che2020accelerating}. Then it creates $O(m)$ sub-branches from the initial branch $B=(\emptyset, G, G[\emptyset])$. Since (1) the edge-oriented branching corresponds to a recursive binary partitioning process, which implies that each sub-branch would explore $O(2^{\tau})$ branches in the worst case and (2) the size of a maximal clique can be bounded by $\tau$, the worst-case time complexity of \texttt{EBBMC} is $O(\delta m + \tau m \cdot 2^{\tau})$. 
    % Consider the space complexity. \texttt{EBBMC} first needs $O(m+n)$ {\chengc space} to store the whole graph. Then since each produced sub-branch from the initial branch is solved one after another, both $g_C$ and $g_X$ {\cheng would not} exceed the size of the input graph and are much smaller than the graph size in practice. Therefore, the space complexity is $O(m+n)$.
\end{proof}

% \begin{proof}
%     Consider the time complexity. \texttt{EBBMC} first needs $O(\delta m)$ time to obtain the truss-based edge ordering \cite{che2020accelerating}. Then it creates $O(m)$ sub-branches from the initial branch $B=(\emptyset, G, G[\emptyset])$. Since (1) the edge-oriented branching corresponds to a recursive binary partitioning process, which implies that each sub-branch would explore $O(2^{\tau})$ branches in the worst case and (2) the size of a maximal clique can be bounded by $\tau$, the worst-case time complexity of \texttt{EBBMC} is $O(\delta m + \tau m \cdot 2^{\tau})$. Consider the space complexity. \texttt{EBBMC} first needs $O(m+n)$ to store the whole graph. Then since each produced sub-branch from the initial branch is solved one  after another, both $g_C$ and $g_X$ {\cheng would not} exceed the size of the input graph and are much smaller than the graph size in practice. Therefore, the space complexity is $O(m+n)$.
% \end{proof}











\subsection{A Hybrid Branch-and-bound {\cheng Framework}: \texttt{HBBMC}}
\label{subsec:HBBMC}

{\chengc On the one hand,} {\cheng the edge-oriented branching framework with the} truss-based edge ordering can produce much smaller graph {\cheng instances} than those produced by vertex-oriented branching strategy {\cheng since} $\tau<\delta$ \cite{wang2024technical}.
% \texttt{EBBMC} still produces much more branches than necessary. Recall that 
{\chengc On the other hand,}
{\cheng 
% Meanwhile, 
the vertex-oriented branching framework can be improved with the pivoting strategy~\cite{tomita2006worst,naude2016refined}.} 
% some existing studies of \texttt{VBBMC} algorithms \cite{tomita2006worst,naude2016refined} have successfully adopted pivoting strategy for maximal clique enumeration. 
{\chengc Therefore,} 
we propose to integrate the pivoting strategy into the \texttt{EBBMC} framework {\chengc to enjoy the merits of both frameworks}. 
% Specifically, given a branch $B=(S,g_C,g_X)$, instead of producing branches for all vertices in $g_C$, these algorithms first choose a vertex $v\in V(g_C)\cup V(g_X)$, which is called the \emph{pivot vertex}. They then create the branches only for $v$'s non-neighbors in $g_C$ (including $v$ itself if $v\in V(g_C)$), i.e., the branches produced on $v$'s neighbors are pruned. The rationale is that those maximal cliques that have $v$'s neighbors inside either include $v$ (which can be enumerated from the branch produced at $v$) or include at least one $v$'s non-neighbors (which can be enumerated from the branch produced at $v$'s non-neighbors), since otherwise, the clique is not maximal. To reduce the maximum number of sub-branches within a branch, the vertex $v\in V(g_C)\cup V(g_X)$ that has the maximum number of neighbors in $g_C$ is usually selected as the pivot vertex. 
{\chengB Specifically,} we observe that the maximal cliques in $B$ can be enumerated either with \texttt{VBBMC} frameworks (where the branches are produced based on the vertices in $g_C$ according to Eq.~(\ref{eq:vbb-branching})) or with \texttt{EBBMC} framework (where the branches are produced mainly based on the edges in $g_C$ according to Eq.~(\ref{eq:ebb-branching}) and Eq.~(\ref{eq:zbb-branching})). To inherit the benefits from these two frameworks, we first adopt \texttt{EBBMC} {\cheng for the branching at} the initial branch $B=(\emptyset, G, G[\emptyset])$ since the produced candidate graph instance in each sub-branch is bounded by $\tau$; then for each produced sub-branch, {\kaixinC to achieve the best theoretical performance,} we adopt \texttt{VBBMC} with classic pivot selection  \cite{tomita2006worst, eppstein2010listing} to boost the efficiency. 
{\kaixinC Specifically, given a branch $B=(S,g_C,g_X)$, the pivoting strategy always selects a vertex $v^*\in V(g_C)\cup V(g_X)$ such that $v^*$ has the most number of neighbors in $g_C$.}
We call {\chengB this \underline{h}ybrid \underline{b}ranch-and-\underline{b}ound framework for \underline{MC}E} {\chengc as} \texttt{HBBMC}, whose pseudo-code is presented in Algorithm~\ref{alg:HBBMC}. 
%
{\kaixinC We note that \texttt{HBBMC} is the first algorithm that integrates the edge-oriented branching strategy and the vertex-oriented branching strategy 
% together 
for enumeration problem. Besides, with this new hybrid branching strategy, the worst-case time complexity can be theoretically improved when the graph satisfies some condition, which we show in the following theorem as follows.}


% Motivated by this, we apply the pivoting strategy to the \texttt{HBBMC} framework. Formally, consider an arbitrary branch $B=(S, g_C, g_X)$. Let $g$ be a subgraph of $G$ induced by the edges in $g_C$ and $g_X$, i.e., $g = G[E(g_C)\cup E(g_X)]$. We choose a pivot vertex $u\in V(g)$. Then for each vertex $v\in V(g_C)$, we can apply the following pruning rule.

% \begin{itemize}[leftmargin=*]
%     \item \textbf{Rule}: if $(u,v)\in E(g)$, the branch produced on $v$ can be pruned. 
% \end{itemize}

% Although this pruning rule has proven to be effective in existing studies, its benefit is not fully unleashed. To see this, consider the example in Figure~\ref{}. In existing studies, the



% Without loss of generality, we assume that $u_p=u$ is the common end point. Then based on the connectivity of $v_p$ and $v$, there are two sub-cases. 

% \begin{itemize}[leftmargin=*]
%     \item \textbf{Case 1.1: $(v, v_p)\in E(g)$.} The branch produced on $e$ can be pruned. 
%     % The rational is that the vertices $u$ (i.e., $u_p$), $v$ and $v_p$ form a 3-clique. 
%     \item \textbf{Case 1.2: $(v, v_p)\notin E(g)$.} The branch produced on $e$ should be preserved. 
% \end{itemize}


% \noindent\textbf{Case 2: $(u,v)\in E(g)$.} Then the branch produced on $v$ can be pruned. 
% Then based on the connectivity of $u_p$, $v_p$, $u$ and $v$, we have the following two sub-cases. 

% \begin{itemize}[leftmargin=*]
%     \item \textbf{Case 2.1: $\forall e'\in\{(u,u_p), (u, v_p), (v, u_p), (v,v_p)\}, e'\in E(g)$.} The branch produced on $e$ can be pruned. 
%     \item \textbf{Case 2.2: $\exists e'\in\{(u,u_p), (u, v_p), (v, u_p), (v,v_p)\}, e'\notin E(g)$.} The branch produced on $e$ should be preserved. 
% \end{itemize}


% We observe that the maximal cliques in $B$ can be enumerated either with \texttt{VBBMC} frameworks (where the branches are produced based on the vertices in $g_C$ according to Eq.~(\ref{eq:vbb-branching})) or with \texttt{HBBMC} framework (where the branches are produced mainly 
% based on the edges in $g_C$ according to Eq.~(\ref{eq:ebb-branching}) and Eq.~(\ref{eq:zbb-branching})). To inherit the benefits from these two different frameworks, we first adopt \texttt{HBBMC} to branch the initial branch $B=(\emptyset, G, G[\emptyset])$; then for each produced sub-branch, we adopt \texttt{VBBMC} with pivot selection to boost the efficiency. 





\begin{algorithm}[t]
% \small
\caption{The hybrid branching-based BB framework for maximal clique enumeration: \texttt{HBBMC}}
\label{alg:HBBMC}
\KwIn{A graph $G=(V,E)$.}
\KwOut{All maximal cliques within $G$.}
\SetKwFunction{List}{\textsf{VBBMC\_Rec}}
\SetKwProg{Fn}{Procedure}{}{}
% Let $v_1, \cdots, v_n$ be in the degeneracy ordering of $G$\;
% \For{each $v_i\in V(G)$}{
% $P_i\gets N(v_i)\cap \{v_1, \cdots, v_{i-1}\}$\;
% $X_i\gets N(v_i)\cap \{v_{i+1}, \cdots, v_n\}$\;
% \List{$\{v_i\}, P_i, X_i$}\;
% }
% \tcc{Initialize and create branches from $G$}
$\pi_{\tau}(G)\gets$ the truss-based ordering of edges in $G$\;
\For{each edge $e_i\in E(G)$ following $\pi_{\tau}(G)$}{
    Obtain $S_i$, $g_{C_i}'$ and $g_{X_i}'$ (lines 6-7 of Algorithm~\ref{alg:EBBMC})\;
    % Create branch $B_i=(S_i,g_{C_i},g_{X_i})$ based on Eq.~(\ref{eq:ebb-branching})\;
    % $g_{C_i}',~g_{X_i}'\gets$ Refine $g_{C_i}$ and $g_{X_i}$ by removing those vertices that are not adjacent to $S_i$\;
    \List{$S_i,g_{C_i}',g_{X_i}'$}\;
}
Conduct Termination (lines 9-12 of Algorithm~\ref{alg:EBBMC})\;
% \tcc{Initialize and create branches from $G$}
% Conduct Initialization and Termination (lines 1-6 of Algorithm~\ref{alg:HBBMC-T})\;
% \Fn{\List{$S, g_C, g_X$}} {
%     Conduct Termination (lines 3-4 and 9-12 of Algorithm~\ref{alg:HBBMC});
    
%     \tcc{Branching on the edges}
%     $E_c\gets$ \Pivot{$g_C, g_X$}\;
%     \For{each edge $e\in E_c$}{
%         Conduct Branching (lines 10-12 of Algorithm~\ref{alg:HBBMC-T})\; 
%         % $S'\gets S\cup V(e)$,~$g_C'\gets \big(V(g_C)\cap V_+(e), E(g_C)\cap E_+(e)\big)$ and $g_X'\gets \big(V(g_X)\cap V_-(e), E(g_X)\cap E_-(e)\big)$\;
%         % \List{$S',g_{C}',g_{X}'$}\;
%         % $E(g_C)\gets E(g_C)\setminus\{e\}$ and $E(g_X)\gets E(g_X)\cup \{e\}$\;
%         % $P\gets P\setminus \{v\}$\;
%         % $X\gets X\cup \{v\}$\;
%     }
% }
\end{algorithm}




% \if 0

% Motivated by this, we propose to determine a pivoting strategy for the \texttt{EBBMC} framework based on the information of the edges. Consider a branch $B=(S, g_C, g_X)$. Let $g$ be a subgraph of $G$ induced by the edges in $g_C$ and $g_X$, i.e., $g = G[E(g_C)\cup E(g_X)]$. We choose a \emph{pivot edge} $e_p=(u_p,v_p)\in E(g)$. Then for each edge $e=(u,v)\in E(g_C)$, there are two possible cases as follows. 


% \noindent\textbf{Case 1: $e_p$ and $e$ have common end point.} Without loss of generality, we assume that $u_p=u$ is the common end point. Then based on the connectivity of $v_p$ and $v$, there are two sub-cases. 

% \begin{itemize}[leftmargin=*]
%     \item \textbf{Case 1.1: $(v, v_p)\in E(g)$.} The branch produced on $e$ can be pruned. 
%     % The rational is that the vertices $u$ (i.e., $u_p$), $v$ and $v_p$ form a 3-clique. 
%     \item \textbf{Case 1.2: $(v, v_p)\notin E(g)$.} The branch produced on $e$ should be preserved. 
% \end{itemize}

% % If the edge $e$ belongs to this case, it means that both vertices incident to $e$ are the common neighbors of the vertices incident to $e_p$. 

% \noindent\textbf{Case 2: $e_p$ and $e$ have no common end point.} Then based on the connectivity of $u_p$, $v_p$, $u$ and $v$, we have the following two sub-cases. 

% \begin{itemize}[leftmargin=*]
%     \item \textbf{Case 2.1: $\forall e'\in\{(u,u_p), (u, v_p), (v, u_p), (v,v_p)\}, e'\in E(g)$.} The branch produced on $e$ can be pruned. 
%     \item \textbf{Case 2.2: $\exists e'\in\{(u,u_p), (u, v_p), (v, u_p), (v,v_p)\}, e'\notin E(g)$.} The branch produced on $e$ should be preserved. 
% \end{itemize}


% % \noindent\textbf{Case 2 ().} 

% % If the edge $e$ belongs to this case, it means that there exists an least one vertex incident to $e$ that is not the common neighbors of the vertices incident to $e_p$. 


% Let $E_{p}$ be those edges on which the produced branches can be pruned according to Case 1.1 and Case 2.1. We show the rationale of the these two pruning rules in the following lemma. 


% % as follows. Consider , and we denote them by $E_{prune}$. We claim that any clique $C$ that is induced by a subset of edges in $E_{prune}$ cannot be maximal (i.e., if a clique $C$ satisfies $E(C)\subseteq E_{prune}$, then $C$ is not a maximal clique).

% \begin{lemma}
%     If a clique $C$ has $E(C)\subseteq E_{p}$, $C$ is not maximal.
% \end{lemma}
% \begin{proof}
%     We prove the claim by contradiction. Assume that $C$ is maximal. We construct a graph $C'$ as follows. We first let $E(C')=E(C)\cup \{e_p\}$. Then for each edge $e\in E(C)$, it must satisfy either Case 1.1 or Case 2.1. If $e$ satisfies Case 1.1, then we add $(v, v_p)$ into $E(C')$. If $e$ satisfies Case 2.1, then we add $(u,u_p), (u, v_p), (v, u_p), (v, v_p)$ into $E(C')$. Consider the subgraph of $G$ induced by the edge set $E(C')$. We find that $u_p$ and $v_p$ are connected with each other and all vertices in $C$, respectively. Hence, $C'$ is a larger clique that contains $C$, which contradicts to the assumption that $C$ is maximal. 
% \end{proof}



% With this lemma, the maximal cliques in $B$ either include the pivot edge $e_p$ if $e_p\in E(g_C)$ or include an edge that belongs to Case 1.2 or Case 2.2. For the edges that are not pruned based on $e_p$, we can further choose another pivot edge $e_p'\in E(g)\setminus (E_p \cup \{e_p\})$ and prune another set of edges $E_p'$ from $g_C$ based on the above pruning rules. We continue the above process, until all the edges in $g_C$ are either (1) pivot edges or (2) pruned based on some pivot edge. We denote \texttt{HBBMC-T} with the pivoting strategy by \texttt{HBBMC-P} and summarize the above process in Algorithm~\ref{alg:HBBMC-P}. 


% \begin{algorithm}[t]
% \small
% \caption{\texttt{HBBMC-P}: \texttt{HBBMC-T} with pivoting strategy}
% \label{alg:HBBMC-P}
% \KwIn{A graph $G=(V,E)$.}
% \KwOut{All maximal cliques within $G$}
% \SetKwFunction{List}{\textsf{HBBMC-P\_Rec}}
% \SetKwFunction{Pivot}{\textsf{ChoosePivot}}
% \SetKwProg{Fn}{Procedure}{}{}
% % Let $v_1, \cdots, v_n$ be in the degeneracy ordering of $G$\;
% % \For{each $v_i\in V(G)$}{
% % $P_i\gets N(v_i)\cap \{v_1, \cdots, v_{i-1}\}$\;
% % $X_i\gets N(v_i)\cap \{v_{i+1}, \cdots, v_n\}$\;
% % \List{$\{v_i\}, P_i, X_i$}\;
% % }
% \tcc{Initialize and create branches from $G$}
% Conduct Initialization and Termination (lines 1-6 of Algorithm~\ref{alg:HBBMC-T})\;
% \Fn{\List{$S, g_C, g_X$}} {
%     Conduct Termination (lines 3-4 and 9-12 of Algorithm~\ref{alg:HBBMC});
    
%     \tcc{Branching on the edges}
%     $E_c\gets$ \Pivot{$g_C, g_X$}\;
%     \For{each edge $e\in E_c$}{
%         Conduct Branching (lines 10-12 of Algorithm~\ref{alg:HBBMC-T})\; 
%         % $S'\gets S\cup V(e)$,~$g_C'\gets \big(V(g_C)\cap V_+(e), E(g_C)\cap E_+(e)\big)$ and $g_X'\gets \big(V(g_X)\cap V_-(e), E(g_X)\cap E_-(e)\big)$\;
%         % \List{$S',g_{C}',g_{X}'$}\;
%         % $E(g_C)\gets E(g_C)\setminus\{e\}$ and $E(g_X)\gets E(g_X)\cup \{e\}$\;
%         % $P\gets P\setminus \{v\}$\;
%         % $X\gets X\cup \{v\}$\;
%     }
% }
% \Fn{\Pivot{$g_C, g_X$}} {
%  $E_c\gets\emptyset$\;
%  \While{$E(g_C)\neq\emptyset$}{
%    $e_p\gets$ Choose a pivot edge from $E(g_C)\cup E(g_X)$\;
%    $E_p\gets$ Pruned edges based on Case 1.1 and Case 2.1\;
%    $E(g_C)\gets E(g_C)\setminus E_p$\;
%    \If{$e_p\in E(g_C)$}{
%    $E(g_C)\gets E(g_C)\setminus \{e_p\}$\;
%    $E_c\gets E_c\cup \{e_p\}$\;
%    }
%  }
%  \Return{$E_c$}\;
% }
% \end{algorithm}


% \fi

% To see this, 
% Together with the edge $e_p$, these edges can form a set of cliques that include $e_p$. Then if $e_p\in E(g_C)$, the maximal cliques that contain $e_p$ can be enumerated under the branch produced on $e_p$. For other maximal cliques, 





% \smallskip\noindent
% \textbf{Complexity.} Given the graph $G=(V,E)$, let $\tau$ be the largest size of a produced graph instance $g_{C_i}'$ via branching, i.e., $\tau = \max_{e_i\in E} |V(g_{C_i}')|$. Then we have the following analysis. 


\begin{theorem}
\label{theo:hbbmc}
    Given a graph $G=(V,E)$, the time and space complexities of \texttt{HBBMC} are $O(\delta m + \tau m \cdot 3^{\tau/3})$ and $O(m+n)$, respectively.
\end{theorem}



\begin{proof}
    The running time of \texttt{HBBMC} consists of (1) the time of generating the truss-based edge ordering and obtaining the subgraphs (i.e., $g_C$ and $g_X$) for enumeration, which can be done in $O(\delta m)$ time, where $\delta$ is the degeneracy of the graph, and (2) the time of recursive enumeration procedure, which can be done in $O(\tau m \cdot 3^{\tau/3})$ time. Detailed analysis can be found in the Appendix~\ref{app:proof-theorem2}. 
\end{proof}


% \begin{proof}
% {\Revise The running time of \texttt{HBBMC} consists of (1) the time of generating the truss-based edge ordering and obtaining the subgraphs (i.e., $g_C$ and $g_X$) for enumeration, which can be done in $O(\delta m)$ time, where $\delta$ is the degeneracy of the graph, and (2) the time of recursive enumeration procedure.
    
% \underline{Consider the former}. First, the time complexity of generating the truss-based edge ordering is $O(\delta m)$ \cite{wang2024technical}. Besides, the time of getting the subgraphs can also be bounded by $O(\delta m)$. The reason is as follows. First, for all edges $e=(u,v)\in E$, we can compute the set of common neighbors of $u$ and $v$ (i.e., $N(V(e), G)$ for $e\in E$) in $O(\delta m)$ time by any existing triangle listing algorithm \cite{hu2014efficient,chu2011triangle,latapy2008main}. Second, consider an edge $e=(u,v)\in E$. For each $w\in N(V(e), G)$, $w\in V(g_C)$ if both edges $(u, w)$ and $(v, w)$ are ordered after $e$; otherwise, $w\in V(g_X)$. This process can also be done in $O(\delta m)$. To see this, we note that $u$, $v$ and $w$ always form a triangle (i.e., 3-clique), indicating that the time cost for getting all subgraphs for the sub-branches is proportional to the number of triangles in $G$. According to the existing triangle listing algorithms \cite{hu2014efficient,chu2011triangle,latapy2008main}, given a graph with its degeneracy number equal to $\delta$, the number of triangles inside is bounded by $O(\delta m)$. With $V(g_C)$ and $V(g_X)$, it is sufficient to recursively conduct the vertex-oriented branching strategy for the remaining branches. 

% \marginnote{R1O2}

% \underline{Consider the latter}, we analyze the time costs for the recursive process. We first show two lemmas that is necessary for the proof. 

% \begin{lemma}[Theorem 3 of \cite{tomita2006worst}]
% \label{lemma:1}
% Let $F(n)$ be a function which satisfies the following recurrence relation
% \begin{equation}
%     F(n)\le\left\{
% \begin{array}{lr}
%     \max_{k} \{k\cdot F(n-k)\} + O(n^2) & \quad \text{if } n > 0 \\
%      O(1) & \quad \text{if } n=0
% \end{array}
%     \right.
% \end{equation}
% where $n$ and $k$ are positive integers. Then $F(n) = O(3^{n/3})$.
% \end{lemma}

% \begin{lemma}
% \label{lemma:2}
%     Given a graph $G=(V, E)$ with its truss number equal to $\tau$. The number of triangles in $G$ is no more than $m\tau$. 
% \end{lemma}

% \begin{proof}
%     Let $\pi_{\tau}=\langle e_1, e_2, \cdots, e_m \rangle$ be the truss-based edge ordering and $sup(e_i)$ be the number of common neighbors in the subgraph induced by $\{e_i, e_{i+1}, \cdots, e_m\}$. Then, the number of triangles in $G$, denoted by $N$, is bounded by
%     \begin{equation}
%         N =\sum_{i=1}^m sup(e_i) \le \sum_{i=1}^m \tau =m\tau
%     \end{equation}
%     The first equation follows from the fact that each triangle is uniquely associated with the earliest edge in the truss-based ordering of its three constituent edges. The inequality follows from the definition of $\tau$. 
% \end{proof}

% Now, we are ready for the analysis. Consider a branch $B=(S,g_C,g_X)$ produced after the edge-oriented branching strategy, let $T(c,x)$ be the time complexity of solving $B$ with $c=|V(g_C)|$ and $x=|V(g_X)|$. 
% The time cost consists of three components. First, it would take $O(c\cdot (c+x))$ to choose the pivot by checking each vertex in $V(g_C)\cup V(g_X)$ to identify the number of its neighbors in $g_C$. Second, assume that the pivot is $v^*$ and $v^*$ has $k$ ($k\le c$) non-neighbors in $g_C$ (denoted by $u_1, \cdots, u_k$), on which the sub-branches are produced. Correspondingly, for each sub-branch produced on $u_i$, it would take $O(c+x)$ to identify $u_i$'s neighbors in $g_C$ and $g_X$. In total, it would take $O(k\cdot (c+x))$ in total to construct $k$ sub-branches. Third, since $v^*$ is a pivot that has the maximum number of neighbors in $g_C$, i.e., $c-k$ neighbors, for each $u_i\in V(g_C)$, they all have at most $c - k$ neighbors in $g_C$. Thus, we have the following recurrence 
% \begin{equation}
% \label{eq:rec}
% \begin{aligned}
%     T(c,x) &\le \max_k \{k \cdot T(c-k,x)\} + \lambda \cdot c\cdot (c+x) \\
%     &=(c+x) \cdot \Big( \max_k \{k \cdot \frac{T(c-k,x)}{c+x}\} + \lambda \cdot c \Big) \\
%     &\le (c+x) \cdot \Big( \max_k \{k \cdot \frac{T(c-k,x)}{c-k+x}\} + \lambda \cdot c^2 \Big) \\
% \end{aligned}
% \end{equation}
% The first inequality follows by summing up the three components of the time cost, where $\lambda>0$ is a constant. The equality follows by extracting $(c+x)$. To see the third inequality, we first have $\lambda\cdot c\le \lambda \cdot c^2$ since $c\ge 1$. Then, let $k^*$ be value of $k$ such that $k \cdot \frac{T(c-k,x)}{c+x}$ reaches the maximum. We have 
% \begin{equation}
% \begin{aligned}
%     \max_k \{k \cdot \frac{T(c-k,x)}{c+x}\} &= k^* \cdot \frac{T(c-k^*,x)}{c+x} \\
%     &\le k^* \cdot \frac{T(c-k^*,x)}{c-k^*+x} \\
%     &\le  \max_k \{k \cdot \frac{T(c-k,x)}{c-k+x}\}
% \end{aligned}
% \end{equation}
% Let $f(c)=\frac{T(c,x)}{(c+x)}$, we have 
% \begin{equation}
%     f(c)\le \max_k \{k \cdot f(c-k)\} + \lambda \cdot c^2
% \end{equation}
% According to Lemma~\ref{lemma:1}, we have $f(c)=\lambda'\cdot 3^{c/3}$, where $\lambda'>0$ is also a constant. Therefore, $T(c,x)=\lambda'\cdot(c+x)\cdot 3^{c/3}$. To compute the total time complexity, 
% \begin{equation}
% \begin{aligned}
%     \sum_{e\in E} T(c_e, x_e) &=\sum_{e\in E} \lambda' \cdot (c_e + x_e) \cdot 3^{c_e/3}\\
%     &\le \lambda' \cdot 3^{\tau/3} \cdot \sum_{e\in E} (c_e + x_e) \le \lambda'  \cdot 3^{\tau/3} \cdot 3m\tau
% \end{aligned}
% \end{equation}
% The first inequality follows from the fact that $c_e\le \tau$ based on the definition of $\tau$. The second inequality follows from the facts that (1) for an edge $e$, $(c_e+x_e)$ is the number of triangles associated with $e$, and (2) the total number of triangles is no larger than $m\tau$ (Lemma~\ref{lemma:2}). 


% In summary the total time cost of \texttt{HBBMC} is $O(m \delta + m \tau \cdot 3^{\tau/3})$. 
% }
% \end{proof}


% \subsection{Proof of Theorem~\ref{theo:hbbmc}}

% \begin{proof}
%     The running time of \texttt{HBBMC} consists of {\chengc (1)} the time of generating the truss-based edge ordering, which can be done in $O(\delta m)$ {\chengc time}, where $\delta$ is the degeneracy of the graph, and {\chengc (2)} the time of recursive enumeration procedure. Consider the latter. Let $T(n)$ be the total time cost to enumerate all maximal cliques within a branch $B=(S, g_C, g_X)$, where $|V(g_C)|=n$. We have the following recurrence. 
% \begin{equation}
% \label{eq:hbbmc}
% T(n) \le \left\{
% \begin{array}{lr}
%     O(\tau) & g_C = G[\emptyset]\\ 
%     O(\delta m) + \sum_{e\in E} T(\tau) &  g_C = G \\ 
%     \max_k \{k\cdot T(n - k)\} + O(m) & g_C\neq G, G[\emptyset] \\
% \end{array}
% \right.
% \end{equation}
% % where $\Delta$ is the maximum degree of a vertex in $G$. 
% The second inequality derives from facts that (1) the truss-based edge ordering can be obtained in $O(\delta m)$ time \cite{wang2024technical} and (2) for each sub-branch produced by edge-oriented branching, the graph instance is bounded by $\tau$. The third inequality derives from facts that  given a branch $B=(S,g_C,g_X)$ with $|V(g_C)|=n$, (1) the total time to choose the pivot vertex and construct the 
% % graphs 
% {\chengc graph}
% instances for the sub-branches is at most $O(m)$ and (2) with pivoting strategy, the time for recursive enumeration procedure is $\max_{k} \{k\cdot T(c-k, x)\}$ \cite{tomita2006worst, eppstein2010listing}. The reason is briefly explained as follows. First, to choose a pivot vertex $v\in V(g_C)\cup V(g_X)$ that has the maximum number of neighbors in $g_C$, we need to check each vertex in $V(g_C)\cup V(g_X)$ to identify the number of its neighbors in $g_C$, which {\chengc takes} $O(m)$ {\chengc time}. Second, given a branch $B=(X, g_C, g_X)$, to construct the graph instance for a sub-branch produced at $v$, it needs to check all the vertices in $V(g_C)\cup V(g_X)$ such that only $v$'s neighbors are passed to the lower-level recursive calls. Since there are at most $\tau$ sub-branches to produce, the total time {\chengc for constructing} 
% % construct 
% the {\chengc graph} instances for the sub-branches is bounded by $O(m)$. 
% % which needs at most $O(n)$ time. 
% % Since there are at most $\tau$ sub-branches to produce, the total time construct the graphs instances for the sub-branches is bounded by $O(m)$. 
% Third, consider a branch $B=(S,g_C,g_X)$ and a pivot vertex $u$. Assume that $u$ has $k$ non-neighbors in $g_C$, on which the sub-branches are produced. Correspondingly, $u$ has $c-k$ neighbors in $g_C$. Since $u$ is {\chengc a} pivot that has the maximum number of neighbors in $g_C$, for any vertex $v\in V(g_C)$, they all have at most $c - k$ neighbors in $g_C$. Thus, the total time for {\chengc the} recursive calls is bounded by $k\cdot T(c-k, x)$. By solving the recurrence, we {\chengc obtain} the time complexity of \texttt{HBBMC}, {\cheng which} is $O(\delta m + \tau m \cdot 3^{\tau/3})$. 
% \end{proof}

\smallskip\noindent\textbf{{\chengc Differences between \texttt{HBBMC} and \texttt{EBBkC}~\cite{wang2024technical}.}}
{\kaixinC 
% To highlight the our technical contributions on the worst-case time complexity, we clarify the major differences between ours and those in \cite{wang2024technical} as follows. 
In specific, our \texttt{HBBMC} algorithm targets the maximal clique enumeration problem and has the worst-case time complexity of $O(\delta m + \tau m \cdot 3^{\tau/3})$ while \texttt{EBBkC} in \cite{wang2024technical} targets the $k$-clique listing problem and has the worst-case time complexity of $O(\delta m + km \cdot (\tau/2)^{k-2})$. Although these two theoretical results both come from the analysis of the recurrence of the time cost $T(n)$, where $n$ is the size of candidate graph, they follow totally different guidelines and have different forms of the recurrence inequalities (Eq.~(\ref{eq:rec}) of this paper v.s. Eq. (6) in \cite{wang2024technical}). To see this, we explain it from the perspective of the recursion tree (i.e., both algorithms are branch-and-bound algorithms and form a recursion tree with each branch being a tree node).
\begin{itemize}[leftmargin=*]
    \item The depth of the recursion tree formed by \texttt{HBBMC} is bounded by $\tau$ while that formed by \texttt{EBBkC} is bounded by $k$ (note that the partial solution of \texttt{HBBMC} (resp. \texttt{EBBkC}) contains at most $\tau$ (resp. $k$) vertices and we add at least one vertex to the partial set at each branching), where $\tau$ can be much larger than $k$ in practice.
    
    \item The width of the recursion tree formed by \texttt{HBBMC} is different from that of \texttt{EBBkC}. Note that for a branch $B=(S,g_C,g_X)$ in \texttt{HBBMC}, it forms $V(g_C)\setminus N(v^*, g_C)$ sub-branches based on the vertex-oriented branching with pivot selection, where $v^*$ is the pivot vertex, while for a branch $B$ in \texttt{EBBkC}, where $B$ is associated with a partial clique $S$ and a candidate graph $g$, it forms at most $V(g)$ sub-branches based on the vertex-oriented branching. 
\end{itemize}




Due to the above differences, the recursion tree of \texttt{HBBMC} would be narrower but deeper while the recursion tree of \texttt{EBBkC} in \cite{wang2024technical} would be wider but shallower. This also contributes to the different number of branches in the recursion tree. {\chengc Specifically}, the number of branches in the tree of \texttt{HBBMC} could be exponential wrt the size of the input (e.g., $O(3^{n/3})$) while that of \texttt{EBBkC} is polynomial (e.g., $O(n^k)$) wrt the size of the input. Therefore, the problems of solving the recurrence inequalities {\chengc are} largely different from each other. 



Furthermore, the correctness of \texttt{HBBMC} is based on the edge-oriented BK branching, which is a newly introduced branching strategy that is not considered in any existing work, including \cite{wang2024technical}. 
% To eluminate this claim, 
{\chengc Specifically,}
we refer to two formulated branching steps of ours and \cite{wang2024technical} (Eqs.~(\ref{eq:ebb-branching}) and (\ref{eq:zbb-branching}) of this paper v.s. Eq.~(2) of \cite{wang2024technical}), respectively. The differences are in twofold. First, the data structure $g_X$ must be maintained for maximality checking {\chengc for the} maximal clique enumeration problem such that each maximal clique is enumerated only once but $g_X$ is not necessary for the $k$-clique listing problem. Second, Eq. (3) is solely for our problem, for which we have explained in Section~\ref{subsec:EBBMC}. 

Lastly, the term ``hybrid'' refers to different meanings in our paper and in \cite{wang2024technical}, respectively. In our paper, the ``hybrid'' in \texttt{HBBMC} refers to different enumeration frameworks (e.g., the vertex-oriented one and the edge-oriented one) while \cite{wang2024technical} solely utilizes edge-based branching. The achieved theoretical results in this paper (Theorem~\ref{theo:hbbmc}) rely not only on the edge ordering but also on the pivot selection strategy.}



% \begin{proof}
%     The running time of \texttt{HBBMC} consists of the time of generating the truss-based edge ordering, which can be done in $O(\delta m)$, where $\delta$ is the degeneracy of the graph, and the time of recursive enumeration procedure. Consider the latter. Let $T(c,x)$ be the total time cost to enumerate all maximal cliques within a branch $B=(S, g_C, g_X)$, where $|V(g_C)|=c$ and $|V(g_X)|=x$. We have the following recurrence. 
% \begin{equation}
% \label{eq:hbbmc}
% T(c, x) \le \left\{
% \begin{array}{lr}
%     O(\tau) & g_C = G[\emptyset]\\ 
%     O(\delta m) + \sum_{e\in E} T(\tau, \Delta) &  g_C = G \\ 
%     \max_k \{k\cdot T(c - k, x)\} + O(c(c+x)) & g_C\neq G, G[\emptyset] \\
% \end{array}
% \right.
% \end{equation}
% where $\Delta$ is the maximum degree of a vertex in $G$. 
% The second inequality derives from facts that (1) the truss-based edge ordering can be obtained in $O(\delta m)$ time
% % , (2) there are at most $O(n)$ zero-degree vertices in $G$ 
% and (2) for each sub-branch produced by edge-oriented branching, the graph instance is bounded by $\tau$. The third inequality derives from facts that  given a branch $B=(S,g_C,g_X)$ with $|V(g_C)|=c$ and $|V(g_X)|=x$, (1) the total time to choose the pivot vertex and construct the graphs instances for the sub-branches is $O(c(c+x))$ and (2) with pivoting strategy, the time for recursive enumeration procedure is $\max_{k} \{k\cdot T(c-k, x)\}$ \cite{eppstein2010listing, tomita2006worst}. The reason is briefly explained as follows. First, to choose a pivot vertex $v\in V(g_C)\cup V(g_X)$ that has the maximum number of neighbors in $g_C$, we need to check each vertex in $V(g_C)\cup V(g_X)$ to identify the number of its neighbors in $g_C$, which needs $O(c(c+x))$. Second, given a branch $B=(X, g_C, g_X)$, to construct the graph instance for a sub-branch produced at $v$, it needs to check all the vertices in $V(g_C)\cup V(g_X)$ such that only $v$'s neighbors are passed to the lower-level recursive calls, which needs $O(c+x)$ time. Since there are at most $c$ sub-branches to produce, the total time construct the graphs instances for the sub-branches is $O(c(c+x))$. Third, consider a branch $B=(S,g_C,g_X)$ and a pivot vertex $u$. Assume that $u$ has $p$ non-neighbors in $g_C$, on which the sub-branches are produced. Correspondingly, $u$ has $c-p$ neighbors in $g_C$. Since $u$ is pivot that has the maximum number of neighbors in $g_C$, for any vertex $v\in V(g_C)$, they have at most $c - p$ neighbors in $g_C$. Thus, the total time for recursive calls is bounded by $p\cdot T(c-p, x)$. By solving the recurrence, we have the time complexity of \texttt{HBBMC}, {\cheng which} is $O(\delta m + \tau m \cdot 3^{\tau/3})$. 
% \end{proof}


% {\kaixin 
% We note that the running time of \texttt{HBBMC} is nearly worst-case optimal, since (1) there cannot be more than $(m - \frac{\tau(\tau-3)}{2})\cdot 3^{\tau/3}$ maximal cliques in a graph and (2) there exist graph instances that would have exactly $(m - \frac{\tau(\tau-3)}{2})\cdot 3^{\tau/3}$ maximal cliques inside in the worst case and each maximal clique has $O(\tau)$ vertices inside, which we show in the following theorem. 
% }



% % We note that the running time of \texttt{HBBMC} is nearly worst-case optimal, since there exist graph instances that would have $\Theta( (m - \frac{\tau(\tau-3)}{2})\cdot 3^{\tau/3})$ maximal cliques inside in the worst case, which we show in the following theorem. 

% \begin{theorem}
% \label{theo:worst-case}
%     Assume that $\tau>0$ is a multiple of 3. Let $G$ be a large connected graph with $m$ edges ($m\gg \tau$), which satisfies $\tau(G)=\tau$. Then the number of maximal cliques in $G$ is at most $(m - \frac{\tau(\tau - 3)}{2}) \cdot 3^{\tau/3}$. 
% \end{theorem}


% \begin{proof}
%     We give a sketch of the proof and put the details in the appendix. We divide all edges into two parts, i.e., the first $m'$ edges and the last $m-m'$ edges. Then the upper bound of the number of maximal cliques in $G$ can be written by a function of $m'$, i.e., $f(m')$. Finally, we can calculate the optimal value of $m'$, denoted by $m^*$, such that $f(m^*)$ is minimized, which is the upper bound of the number of maximal cliques in $G$. 
% \end{proof}


% % \begin{proof}
% %     % We first analyze the upper bound of the number of the maximal cliques in $G$. 
% %     % First, it is easy to see that the number of the maximal cliques that induced by the single vertex can be bounded by $n$. 
% %     % Then, for the number of maximal cliques that have at least 2 vertices inside, 
% %     We consider the truss-based edge ordering. Based on the definition of $\tau$, for each edge $e\in E$, there are at most $\tau$ vertices that are incident to $V(e)$ in the corresponding sub-branch. Then we consider the first $m-\frac{\tau(\tau+3)}{2}$ edges. For each edge $e$, we apply the Moon-Moser bound \cite{moon1965cliques} to the graph instance of the produced sub-branch, which shows that they can form at most $3^{\tau/3}$ maximal cliques within the sub-branch. Thus, the first $m-\frac{\tau(\tau+3)}{2}$ edges can contribute to at most $(m-\frac{\tau(\tau+3)}{2})\cdot 3^{\tau/3}$ maximal cliques. For the remaining $\frac{\tau(\tau+3)}{2}$ edges, they can form a Moon-Moser graph \cite{moon1965cliques} with $\tau+3$ vertices, which can form at most $3^{(\tau+3)/3}$ maximal cliques. Thus, the total number of the maximal cliques 
% %     % that have at least 2 vertices inside 
% %     can be bounded by $(m-\frac{\tau(\tau+3)}{2})\cdot 3^{\tau/3} + 3^{(\tau+3)/3} < (m-\frac{\tau(\tau-3)}{2})\cdot 3^{\tau/3}$. 
% %     % In summary, we complete the proof. 
% %     % divide all edges into two disjoint sets. One includes $m-\frac{\tau(\tau+3)}{2}$ edges and the other includes the remaining $\frac{\tau(\tau+3)}{2}$ edges. For each edge in the former set, 
% %     % Now, we construct an example graph as illustrated in Figure~\ref{}, which shows the worst case.
% % \end{proof}



% We construct a graph instance such that it has exactly $(m - \frac{\tau(\tau-3)}{2})\cdot 3^{\tau/3}$ maximal cliques inside, which is shown in Figure~\ref{fig:worst-case}. 



{\smallskip\noindent\textbf{Remarks}. 
First, compared with \texttt{VBBMC} algorithms, we define the edge density of the graph as $\rho=\frac{m}{n}$. When $\delta \ge \max\{3, \tau + \frac{3\ln\rho}{\ln 3}\}$, the time complexity of \texttt{HBBMC} (i.e., $O(\delta m + \tau m \cdot 3^{\tau/3})$) {is bounded by} the time complexity of the state-of-the-art \texttt{VBBMC} algorithms (i.e., $O(n\delta \cdot 3^{\delta/3})$). The reason is as follows. {First}, $O(\delta m)$ is bounded by $O(n\delta \cdot 3^{\delta/3})$ when $\delta \ge 3$ since (1) $m \le n\delta$ \cite{lick1970k} and (2) $\delta \le 3^{\delta/3}$ holds for all $\delta$ when $\delta\ge 3$. 
% {Second}, $O(n)$ is bounded by $O(n\delta \cdot 3^{\delta/3})$. 
{Second}, $O(\tau m \cdot 3^{\tau/3})$ is bounded by $O(n\delta \cdot 3^{\delta/3})$ when $\delta \ge \tau + \frac{3\ln\rho}{\ln 3}$. To see this, 
given $\delta \ge \tau + \frac{3 \ln\rho}{\ln 3}$, 
we have $\tau m \cdot 3^{\tau/3} < \delta \cdot n\rho \cdot 3^{\delta/3 - \frac{\ln\rho}{\ln 3} } = \delta  n \cdot 3^{\delta/3}$, where the inequality derives from the facts $\tau < \delta$ \cite{wang2024technical}, $m=n\rho$ and the given condition, and the equation derives from the fact $3^{\frac{\ln \rho}{\ln 3}}=\rho$. We collect the values of $\delta$, $\tau$ and $\rho$ on 139 real-world graphs from \cite{RealGraphs} and 84 real-world graphs from \cite{RealGraphs2}, finding that the condition $\delta \ge \max\{3, \tau + \frac{3 \ln\rho}{\ln 3}\}$ is satisfied for the majority of the graphs (111 {\chengB out} of 139 and 72 {\chengB out} of 84, respectively). 
Second, there are several different \texttt{VBBMC} algorithms in existing studies, which implies that \texttt{HBBMC} can incorporate \texttt{EBBMC} with different \texttt{VBBMC} implementations. We choose the \texttt{VBBMC} with {\kaixinC the pivot selection strategy used in \cite{tomita2006worst, eppstein2010listing}} as the default setting since it achieves the best theorectical results and the relatively good performance in practice (details {\chengB will be presented} in Section~\ref{sec:exp}). 
}




% \begin{theorem}
% \label{theo:compare}
%     Given a graph $G=(V,E)$, we define the edge density of the graph as $\rho=m/n$. When $\delta \ge \max\{3, \tau + \frac{3}{\ln 3}\ln\rho\}$, 
% % which holds for most of the real-world sparse graphs,
% the time complexity of \texttt{HBBMC} (i.e., $O(\delta m + \tau m \cdot 3^{\tau/3})$) {\cheng is bounded by} the time complexity of the state-of-the-art algorithms (i.e., $O(n\delta \cdot 3^{\delta/3})$). 
% \end{theorem}



% \smallskip\noindent\textbf{\texttt{VBBMC} v.s. \texttt{HBBMC} (Time Complexity).} We define the density of the graph $\rho$ as the ratio between the number of edges {\cheng and} the number of vertices, i.e., $\rho=m/n$. 



% \underline{Theoretically}, when $\delta \ge \max\{3, \tau + \frac{3}{\ln 3}\ln\rho\}$, 
% % which holds for most of the real-world sparse graphs,
% the time complexity of \texttt{HBBMC} (i.e., $O(\delta m + \tau m \cdot 3^{\tau/3})$) {\cheng is bounded by} the time complexity of the state-of-the-art algorithms (i.e., $O(n\delta \cdot 3^{\delta/3})$). 
% The explanations are as follows. 
% %
% {First}, $O(\delta m)$ is bounded by $O(n\delta \cdot 3^{\delta/3})$ when $\delta \ge 3$ since (1) $m \le n\delta$ \cite{lick1970k} and (2) $\delta \le 3^{\delta/3}$ holds for all $\delta$ when $\delta\ge 3$. 
% % {Second}, $O(n)$ is bounded by $O(n\delta \cdot 3^{\delta/3})$. 
% {\kaixin
% {Second}, $O(\tau m \cdot 3^{\tau/3})$ is bounded by $O(n\delta \cdot 3^{\delta/3})$ when $\delta \ge \tau + \frac{3}{\ln 3}\ln\rho$. To see this, given the condition $\delta \ge \tau + \frac{3}{\ln 3}\ln\rho$, we have $\tau m \cdot 3^{\tau/3} < \delta \cdot n\rho \cdot 3^{\delta/3 - \frac{1}{\ln 3} \ln\rho} = \delta  n \cdot 3^{\delta/3}$, where the inequality derives from the facts $\tau < \delta$, $m=n\rho$ and the given condition, and the equation derives from the fact $3^{\frac{\ln \rho}{\ln 3}}=\rho$.}
%
% \underline{Practically}, 
% We collect statistics of the values of $\delta$, $\tau$ and $\rho$ on 139 real-world graphs from \cite{RealGraphs} and 84 real-world graphs from \cite{RealGraphs2}, finding that the condition $\delta \ge \max\{3, \tau + \frac{3}{\ln 3}\ln\rho\}$ is satisfied for the majority of the graphs (111 of 139 and 72 of 84). 



% \noindent\textbf{Remarks.} 
%
% (1) We collect the values of $\delta$, $\tau$ and $\rho$ on 139 real-world graphs from \cite{RealGraphs} and 84 real-world graphs from \cite{RealGraphs2}, finding that the condition $\delta \ge \max\{3, \tau + \frac{3}{\ln 3}\ln\rho\}$ is satisfied for the majority of the graphs (111 of 139 and 72 of 84, respectively). (2) As illustrated in Table~\ref{tab:complexity}, there are several designs of \texttt{VBBMC} algorithms in existing studies, which implies that \texttt{HBBMC} can incorporate \texttt{EBBMC} with different \texttt{VBBMC} algorithms. We choose the \texttt{VBBMC} with the classic pivot selection \cite{tomita2006worst, eppstein2010listing} as the default setting since it achieves the best theorectical results and the relatively good performance in practice (details can be found in Section~\ref{sec:exp}). 




% (1) $m \le n\delta$ \cite{lick1970k} and (2) $\tau\cdot 3^{\tau/3} \le 3^{\delta/3}$ when $\delta \ge \tau + \frac{3}{\ln 3}\ln \tau$. In summary, the time complexity of \texttt{HBBMC-P} is better than that of the state-of-the-art algorithms if $\delta \ge \max\{4, \tau + 2.73\ln \tau\}$. We collect the statistics of the values of $\delta$ and $\tau$ of the real-world graphs and we find that the condition $\delta > \tau + 2.73\ln \tau$ holds for the majority of the graphs. 






% \begin{algorithm}[h]
% \small
% \caption{Maximal Clique Enumeration in $t$-plex}
% \label{alg:t-plex}
% \KwIn{A $t$-plex $g$}
% \KwOut{All maximal cliques within $g$}
% \SetKwFunction{List}{\textsf{BKPlex\_Rec}}
% \SetKwProg{Fn}{Procedure}{}{}
% Construct the inverse graph $g_{inv}$ of $g$\;
% $F\gets$ set of vertices in $V(g_{inv})$ that are disconnected with all others\;
% \List{$F, V(g_{inv})\setminus F, \emptyset$}\;
% \Fn{\List{$S, P, X$}} {
%     \tcc{Termination when $P$, $X$ are both empty}
%     \If{$P\cup X=\emptyset$}{
%         \textbf{Output} a maximal clique $S$\;
%     }
%     \tcc{Branching with pivot selection}
%     $u\gets$ an arbitrary vertex in $P\cup X$\;
%     \For{each $v\in N'(u, g_{inv})$}{
%         \List{$S\cup\{v\},P \setminus N'(v, g_{inv}), X \setminus N'(v, g_{inv})$}\;
%         $P\gets P\setminus \{v\}$\;
%         $X\gets X\cup \{v\}$\;
%     }
% }
% \end{algorithm}


==> 4._early-stop.tex <==
\section{Early Termination Technique}
\label{sec:early-termination}


Suppose that we are at a branch $B=(S, g_C, g_X)$, where $g_C$ is dense ({\cheng e.g., it is} a clique or nearly a clique) and {\kaixin $g_X$ is an empty graph}, and we aim to enumerate all maximal cliques within $B$. While the pivot strategy in \texttt{VBBMC} and \texttt{HBBMC} has proven to be effective in practice, it still needs to conduct {\cheng many} set intersections within the vertices in $g_C$,
% than necessary, 
which would be costly. To overcome this issue, we propose an \emph{early-termination} technique, which can directly enumerate the maximal cliques in $B$ with a dense $g_C$ without further {\cheng forming sub-branches on} it. Specifically, we have the following observations. 
%
If $g_C$ is a clique (a.k.a 1-plex), a 2-plex or a 3-plex, we can directly enumerate all maximal cliques within $g_C$ in nearly optimal time. For the first case, {\kaixin since $g_X$ is an empty graph, we can directly include the vertices in $g_C$ to $S$ to form a maximal clique of $G$. 
% by iterating each vertex in $g_X$ to identify whether it is a common neighbor of all vertices in $g_C$. For the latter case, we can do it similarly but in a bit more complex design (details can be found in Section~\ref{subsec:2-plex}).  
For the other two cases, 
% we can also enumerate all maximal cliques with in $g_C$ in nearly optimal time. To achieve this, 
we construct the inverse graph $\overline{g}_C$ of $g_C$. 
% (recall that $\overline{g}_C$ has
% the same set of vertices as $g_C$, with an edge between two vertices
% in $\overline{g}_C$ if and only if they are disconnected from each other in
% $g_C$), 
{An observation is that $\overline{g}_C$} only has several simple paths or cycles. With these additional topological information, we can output all maximal cliques in {\chengc an amount of} time that is proportional to the number of maximal cliques in $g_C$ (details will be discussed in Section~\ref{subsec:2-plex} and Section~\ref{subsec:3-plex}).}
%
% We note that we can determine whether $g_C$ is a $t$-plex for some $t$ by checking the minimum degree of a vertex in $g_C$. If it is no less than $V(g_C) - t$, $g_C$ is a $t$-plex; otherwise, it is not a $t$-plex. This process can be done simultaneously when we select the pivot. 



% \begin{itemize}[leftmargin=*]
    % \item If $g_C$ is a clique or 2-plex, we can directly enumerate all maximal cliques within $g_C$ in nearly optimal time. For the former case, {\color{red} since $g_X$ is an empty graph}, we can directly include the vertices in $g_C$ to $S$ to form a maximal clique of $G$. 
    % by iterating each vertex in $g_X$ to identify whether it is a common neighbor of all vertices in $g_C$. For the latter case, we can do it similarly but in a bit more complex design (details can be found in Section~\ref{subsec:2-plex}).  
    
    % we can directly check the maximality of $g_C$ by iterating each vertex in $g_X$ to identify whether it is a common neighbor of all vertices in $g_C$. For the latter case, we can do it similarly but in a bit more complex design (details can be found in Section~\ref{subsec:2-plex}). 
    
    % \item If $g_C$ is 3-plex, we can also enumerate all maximal cliques with in $g_C$ in nearly optimal time. Since Moon-Moser graph is a special case of 3-plex, there are at most $3^{n/3}$ maximal cliques inside. However, if the number of maximal clique in $G$ is far less than the Moon-Moser bound, we can improve the time complexity from $O(\delta m + n + \tau m \cdot 3^{\tau/3})$ to $O(\delta m + n + \tau \omega + \tau m \cdot 4^{\tau/4})$, where $\omega$ is the number of maximal cliques in $G$ (details can be found in Section~\ref{subsec:3-plex}). 

    % \item If $g_C$ is a $t$-plex with $t \ge 4$, ...
% \end{itemize}


% We note that we can determine whether $g_C$ is a $t$-plex for some $t$ by checking the minimum degree of a vertex in $g_C$. If it is no less than $V(g_C) - t$, $g_C$ is a $t$-plex; otherwise, it is not a $t$-plex. This process can be done simultaneously when we select the pivot. 




\subsection{Enumerating Maximal Cliques from 2-Plex in Nearly Optimal Time}
\label{subsec:2-plex}

\begin{algorithm}[t]
% \small
\caption{Enumerate maximal cliques in a 2-plex}
\label{alg:MC2Plex}
\KwIn{A branch $B=(S,g_C,g_X)$, where $g_C$ is to a 2-plex and $g_X$ is an empty graph.}
\KwOut{All maximal cliques within $B$.}
\SetKwFunction{List}{\textsf{HBBMC-T\_Rec}}
\SetKwProg{Fn}{Procedure}{}{}
Partition $V(g_C)$ into three disjoint sets $F$, $L$ and $R$, such that $L[i]$ disconnects with $R[i]$ in $g_C$ for $1\le i\le |L|$\;
\For{$num=0$ to $2^{|L|}-1$}{
    $S'\gets F$\;
    \For{$i=1$ to $|L|$}{
        \lIf{the $i$-th bit of $num$ is 0}{
            $S'\gets S'\cup \{L[i]\}$
        }
        \lElse {
            $S'\gets S'\cup \{R[i]\}$
        }
    }

    % \If {$N(S\cup S', G)\cap V(g_X) = \emptyset$}{
        \textbf{Output} a maximal clique $S\cup S'$\;
    % }
}
\end{algorithm}



Consider a branch $B=(S, g_C, g_X)$ where $g_C$ is a 2-plex {\kaixin and $g_X$ is an empty graph}. 
% We note that we can directly enumerate all maximal clique in $g_C$ in near optimal time, which we explain as follows. 
We can partition all vertices in $g_C$ into three disjoint sets, namely set $F$, set $L$ and set $R$, each of which induces a clique. This process can be done in two steps. First, we partition $V(g_C)$ into two sets: one containing the vertices that are connected with all the other vertices in $g_C$ (this is $F$) and the other containing the remaining vertices (this is $L\cup R$). For the latter, since each vertex in a 2-plex disconnects with at most 2 vertices (including itself), $L\cup R$ must contain a collection of pairs of vertices $\{u,v\}$ such that $u$ disconnects with $v$ in $g_C$. Thus, we can break each pair of vertices and partition $L\cup R$ into two disjoint sets, where $L$ and $R$ include the first and the second vertices in these pairs, respectively. We note that the {\chengB partitioning} of $L\cup R$ is not unique. Consider an arbitrary one. We observe that the vertex set $F\cup L$ induces a maximal clique in $g_C$. The reason is that if there exists a larger clique $C'$ that is induced by $F\cup L\cup R'$ where $R'\neq \emptyset$, then we must have $R'\subseteq R$. We can find a subset of $L$, denoted by $L'$, such that each vertex in $L'$ disconnects with a vertex in $R'$. In this case, $C'$ is not a clique. Then consider the number of different partitions of $L\cup R$. For each pair of vertices $\{u,v\}$ such that $u$ disconnects with $v$, we can either have (1) $u\in L$ and $v\in R$ or (2) $v\in L$ and $u\in R$. Thus, there are $2^{|L|}$ different partitions of $L\cup R$. 
That is, we have $2^{|L|}$ maximal cliques in $g_C$. We summarize the above procedure in Algorithm~\ref{alg:MC2Plex}. 

% We present the pseudo-code of enumerating maximal cliques in a 2-plex in Algorithm~\ref{alg:MC2Plex}. Specifically, we first partition $V(g_C)$ into three disjoint sets as discussed above. We note that $L$ and $R$ is an arbitrary partition and the $i$-th element of $L$ disconnects with the $i$-th element of $R$ for $1\le i\le |L|$. Let $S'$ be a set that consists of the vertices in a maximal clique in $g_C$ and is initialized as $S'=F$. Then we use an integer $num$ ranging from 0 to $2^{|L|}-1$ to represent each maximal clique in $g_C$. Consider the binary representation of $num$. Since $num$ would use $L$ bits, where each bit is either 0 or 1. We can map each value of $num$ to a maximal clique in $g_C$ by choosing the $i$-th element of $L$ (resp. $R$) if the $i$-th bit of $num$ is 0 (resp. 1). Finally, we output the maximal cliques of $G$ togerther with $S$.  
% if no vertex in $g_X$ is the common neighbor of $S\cup S'$. 


% \begin{algorithm}[t]
% \small
% \caption{{\cheng Enumerating} maximal cliques in a 2-plex}
% \label{alg:MC2Plex}
% \KwIn{A branch $B=(S,g_C,g_X)$, where $g_C$ is to a 2-plex and $g_X$ is an empty graph.}
% \KwOut{All maximal cliques within $B$.}
% \SetKwFunction{List}{\textsf{HBBMC-T\_Rec}}
% \SetKwProg{Fn}{Procedure}{}{}
% Partition $V(g_C)$ into three disjoint sets $F$, $L$ and $R$\;
% \For{$num=0$ to $2^{|L|}-1$}{
%     $S'\gets F$\;
%     \For{$i=1$ to $|L|$}{
%         \uIf{the $i$-th bit of $num$ is 0}{
%             $S'\gets S'\cup \{L[i]\}$\;
%         }
%         \Else {
%             $S'\gets S'\cup \{R[i]\}$\;
%         }
%     }

%     % \If {$N(S\cup S', G)\cap V(g_X) = \emptyset$}{
%         \textbf{Output} a maximal clique $S\cup S'$\;
%     % }
% }
% \end{algorithm}






% \subsection{Enumerating maximal cliques in a 2-plex}

% \begin{figure}[t]
% \centering
% \subfigure[A 2-plex graph $g_C$.]{
%     \label{subfig:2-plex}
%     \includegraphics[width=0.21\textwidth]{figs/plex/plex2.pdf}}
%     \hspace{2mm}
% \subfigure[Inverse graph $\overline{g}_C$ of $g_C$.]{
%     \label{subfig:2-plex-inv}
%     \includegraphics[width=0.21\textwidth]{figs/plex/plex2inv.pdf}}
% % \subfigure[An example 3-plex graph $g$.]{
% %     \label{subfig:3-plex}
% %     \includegraphics[width=0.20\textwidth]{figs/plex/plex3.pdf}}
% % \subfigure[Inverse graph $g_{inv}$ of 3-plex $g$.]{
% %     \label{subfig:3-plex-inv}
% %     \includegraphics[width=0.20\textwidth]{figs/plex/plex3inv.pdf}}
% \caption{{Example of a 2-plex and its inverse graph.}} 
% \label{fig:2-plex}
% \vspace{-5mm}
% \end{figure}

% \smallskip\noindent
% \textbf{Example.}
% %
% Consider the example of a 2-plex and its inverse graph in Figure~\ref{subfig:2-plex}. Based on the definition of $F$, $L$ and $R$ as discussed above, one possible partition is $F=\{v_1, v_2\}$, $L=\{v_3,v_4\}$ and $R=\{v_5,v_6\}$. Given $|L|=2$,  we can directly output 4 maximal cliques as follows, $\{v_1, v_2, v_3, v_4\}$, $\{v_1,v_2,v_3, v_6\}$, $\{v_1, v_2, v_4, v_5\}$ and $\{v_1, v_2, v_5, v_6\}$. 


% \subsection{Proof of Theorem~\ref{theo:complex-within-2plex}}





% \smallskip\noindent
% \textbf{Example.}
% %
% Consider the example of a 2-plex and its inverse graph in Figure~\ref{subfig:2-plex}. Based on the definition of $F$, $L$ and $R$ as discussed above, one possible partition is $F=\{v_1, v_2\}$, $L=\{v_3,v_4\}$ and $R=\{v_5,v_6\}$. Given $|L|=2$,  we can directly output 4 maximal cliques as follows, $\{v_1, v_2, v_3, v_4\}$, $\{v_1,v_2,v_3, v_6\}$, $\{v_1, v_2, v_4, v_5\}$ and $\{v_1, v_2, v_5, v_6\}$. 






% \smallskip
% \noindent\textbf{Complexity.} We analyze the time complexity of Algorithm~\ref{alg:MC2Plex} as follows.

\begin{theorem}
\label{theo:complex-within-2plex}
    Given a branch $B=(S,g_C,g_X)$ with $g_C$ being a 2-plex and $g_X$ being an empty graph, Algorithm~\ref{alg:MC2Plex} enumerates all maximal cliques within $B$ in $O(E(g_C) + \omega(g_C) \cdot c(g_C))$ time, where $\omega(g_C)$ is the size of the largest maximal clique within $B$ and $c(g_C)$ is the number of maximal cliques in $g_C$.
    % and bounded by $2^{|V(g_C)|/2}$.
    % , i.e., $c(g_C) \le 2^{|V(g_C)|/2}$. 
\end{theorem}

\begin{proof}
    First, Algorithm~\ref{alg:MC2Plex} takes $O(E(g_C))$ {\cheng time} for partitioning $V(g_C)$ into three sets (line 1). In each round of lines 2-7,  the algorithm guarantees exactly one maximal clique of $g_C$ to be found. 
    % Besides, the size of $L$ is at most $|V(g_C)|/2$. 
\end{proof}

% \begin{proof}
%     First, Algorithm~\ref{alg:MC2Plex} takes $O(E(g_C))$ {\cheng time} for partitioning $V(g_C)$ into three sets (line 1). In each round of lines 2-9,  the algorithm can guarantee exactly one maximal clique of $g_C$ to be found (lines 3-8). Besides, the size of $L$ is at most $|V(g_C)|/2$. 
% \end{proof}


{\kaixin We note that the above procedure achieves a \emph{nearly optimal} time complexity since $O(\omega(g_C) \cdot c(g_C))$ is the optimal time  and it only takes $O(E(g_C))$ {\chengB extra} time.}





% \begin{figure}[t]
% \subfigure[An example 2-plex graph $g_C$.]{
%     \label{subfig:2-plex}
%     \includegraphics[width=0.20\textwidth]{figs/plex/plex2.pdf}}
% \subfigure[Inverse graph $\overline{g}_C$ of 2-plex $g_C$.]{
%     \label{subfig:2-plex-inv}
%     \includegraphics[width=0.20\textwidth]{figs/plex/plex2inv.pdf}}
% % \subfigure[An example 3-plex graph $g$.]{
% %     \label{subfig:3-plex}
% %     \includegraphics[width=0.20\textwidth]{figs/plex/plex3.pdf}}
% % \subfigure[Inverse graph $g_{inv}$ of 3-plex $g$.]{
% %     \label{subfig:3-plex-inv}
% %     \includegraphics[width=0.20\textwidth]{figs/plex/plex3inv.pdf}}
% \caption{{Example of a 2-plex and its inverse graph.}} 
% \label{fig:2-plex}
% \end{figure}




% \begin{theorem}
% \label{theo:hbbmc-with-2plex}
%     Given a graph $G=(V,E)$, the time complexity of \texttt{HBBMC} with early-termination from 2-plexes is $O(\delta m + \tau m \cdot 3^{\tau/3})$. 
% \end{theorem}

% \begin{proof}
%     Given the facts that (1) Algorithm~\ref{alg:MC2Plex} is nearly optimal and (2) the worst-case time complexity of \texttt{HBBMC} is $O(\delta m + \tau m \cdot 3^{\tau/3})$, the time complexity of \texttt{HBBMC} with early-termination from 2-plex would not be worse than $O(\delta m + \tau m\cdot 3^{\tau/3})$. However, due to fact that the condition for early-termination should satisfy (1) $g_C$ is a 2-plex and (2) $g_X$ is an empty graph, when both conditions are never satisfied simultaneously in the worst case, the recurrence for the time cost reduces to that shown in Eq.~(\ref{eq:hbbmc}). Therefore, the time complexity of \texttt{HBBMC} with early-termination from 2-plexes is $O(\delta m + \tau m \cdot 3^{\tau/3})$. 
% \end{proof}

% We first claim that there are $2^{|L|}$ (i.e., $2^{|R|}$ since $|L|=|R|$) maximal cliques in $g_C$. To see this, we start from a maximal clique which is induced by the vertex set $F\cup L$ and derive all the other maximal cliques in $g_C$. 


\subsection{{\cheng Enumerating} Maximal Cliques from 3-Plex in Nearly Optimal Time}
\label{subsec:3-plex}






Consider a branch $B=(S,g_C, g_X)$ where $g_C$ is 3-plex and $g_X$ is an empty graph. 
% We can also enumerate all maximal cliques in $g_C$ directly in near optimal time. 
% Specifically, consider 
We construct the inverse graph $\overline{g}_C$ of $g_C$. We denote all isolated vertices in $\overline{g}_C$ by $F$ since they connect with all other vertices in $g_C$. Then for each vertex $v\in V(\overline{g}_C)\setminus F$, it belongs to a connected component which can be categorized into two classes: simple paths and simple cycles. The reason is that (1) the maximum degree of a vertex in $\overline{g}_C$ is no greater than two and (2) all connected components of a graph with a maximum degree less than or equal to two consist exclusively of simple paths or simple cycles \cite{west2001introduction}.
% \footnote{https://math.stackexchange.com/questions/2453428/suppose-that-the-maximum-degree-of-a-graph-is-less-or-equal-to-2-then-all-compo}. 
We elaborate on the details of enumerating maximal cliques within these simple paths and simple cycles as follows.

% \smallskip
\noindent\textbf{Category 1 - Paths.}
%
For a path $p=\{v_1, v_2, \cdots, v_{|p|}\}$ in $\overline{g}_C$ ($|p|\ge 2$), the vertices are in the order where $(v_i, v_{i+1})\in E(\overline{g}_C)$. 
% That is, $(v_1, v_2), (v_2, v_3), \cdots, (v_{|p|-1}, v_{|p|})$ are the edges in $\overline{g}_C$. 
Correspondingly, it implies that $v_1$ and $v_{|p|}$ disconnect with only one vertex in $g_C$ (i.e., $v_2$ and $v_{|p|-1}$, respectively), and for any other vertices $v_i$ (if any), it disconnects with two vertices $v_{i-1}$ and $v_{i+1}$ in $g_C$ for $2\le i\le |p|-1$. Next, we present how we can enumerate all maximal cliques in $g_C$ within the vertices of a path $p$ of $\overline{g}_C$. The procedure can be summarized in three steps. 


\begin{itemize}[leftmargin=*]
    \item \textbf{Step 1 - {\chengB Initialization}.}  Let $S_p$ be a subset of $V(p)$ that induces a partial clique of $g_C$. We initialize $S_p=\{v_1\}$ or $S_p=\{v_2\}$. 
    \item \textbf{Step 2 - {\chengB Expansion}.} Let $v_i$ be the last vertex of $S_p$. Then $S_p$ can be either expanded (1) by adding $v_{i+2}$ into $S_p$ (i.e., $S_p = S_p\cup \{v_{i+2}\}$) or (2) by adding $v_{i+3}$ into $S_p$ (i.e., $S_p = S_p\cup \{v_{i+3}\}$). Repeat Step 2 until no vertex can be {\cheng used to expand} $S_p$, i.e., $i+2>|p|$, then go to Step 3. 
    \item \textbf{Step 3 - {\chengB Termination}.} Report $S_p$ as a maximal clique induced within the vertices of the path $p$.
\end{itemize}




\begin{algorithm}[t]
% \small
\caption{Function \textsf{Enum\_from\_Path($p$)}}
\label{alg:enum_path}
\KwIn{A path $p=\{v_1, v_2, \cdots, v_{|p|}\}$ in $\overline{g}_C$.}
\KwOut{All maximal cliques of $g_C$ induced with the vertices in $p$.}
\SetKwFunction{List}{\textsf{Enum\_Rec}}
% \SetKwFunction{ListCycle}{\textsf{Enum\_Rec}}
\SetKwProg{Fn}{Procedure}{}{}
$\mathbb{S}\gets \emptyset$\;
\List{$\mathbb{S}, \{v_1\}, p$}; \List{$\mathbb{S}, \{v_2\}, p$}\;
\Return $\mathbb{S}$\;
\Fn{\List{$\mathbb{S}, S_p, p$}}{
    $v_i\gets$ the last vertex in $S_p$\;
    \If{$i+2>|p|$}{
        $\mathbb{S}\gets \mathbb{S} \cup \{S_p\}$;
        \Return\;
    }
    \List{$\mathbb{S}, S_p\cup\{v_{i+2}\}, p$}\;
    \lIf{$i+3\le|p|$}{
        \List{$\mathbb{S}, S_p\cup\{v_{i+3}\}, p$}
    }
}
\end{algorithm}





\begin{algorithm}[t]
% \small
\caption{Function \textsf{Enum\_from\_Cycle($c$)}}
\label{alg:enum_cycle}
\KwIn{A cycle $c=\{v_1, v_2, \cdots, v_{|c|}\}$ in $\overline{g}_C$.}
\KwOut{All maximal cliques of $g_C$ induced with the vertices in $c$.}
\SetKwFunction{List}{\textsf{Enum\_Rec}}
% \SetKwFunction{ListCycle}{\textsf{Enum\_Rec}}
\SetKwProg{Fn}{Procedure}{}{}
\lIf{$|c|=3$}{\Return $\{\{v_1\},\{v_2\},\{v_3\}\}$}
\lIf{$|c|=4$}{\Return $\{\{v_1,v_3\},\{v_2,v_4\}\}$}
\lIf{$|c|=5$}{\Return $\{\{v_1,v_3\},\{v_1, v_4\},\{v_2,v_4\},\{v_2,v_5\},\{v_3,v_5\}\}$}
\If{$|c|\ge 6$} {
$\mathbb{S}\gets\emptyset$\;
\List{$\mathbb{S}, \{v_1\}, \{v_1, v_2, \cdots, v_{|c|-1}\}$}\;
\List{$\mathbb{S}, \{v_2\}, \{v_2, v_3, \cdots, v_{|c|}\}$}\;
\List{$\mathbb{S}, \{v_{|c|}, v_3\}, \{v_3, v_4, \cdots, v_{|c|-2}\}$}\;
\Return $\mathbb{S}$\;
}
% $\mathbb{S}\gets \emptyset$\;
% \List{$\mathbb{S}, \{v_1\}$}; \List{$\mathbb{S}, \{v_2\}$}\;
% \Return $\mathbb{S}$\;
% \Fn{\List{$\mathbb{S}, S_p$}}{
%     $v_i\gets$ the last vertex in $S_p$\;
%     \If{$i+2>|p|$}{
%         $\mathbb{S}\gets \mathbb{S} \cup S_p$;
%         \Return\;
%     }
%     \List{$\mathbb{S}, S_p\cup\{v_{i+2}\}$}\;
%     \lIf{$i+3\le|p|$}{
%         \List{$\mathbb{S}, S_p\cup\{v_{i+3}\}$}
%     }
% }
\end{algorithm}


\noindent\textbf{{\chengB Correctness}.}
% There are two issues to {\cheng solve} in above design: (1) why do we initialize $S_p$ to $v_1$ or $v_2$ but not some other vertex? (2) why do we expand $S_p$ by just considering $v_{i+2}$ and $v_{i+3}$? The rationale is as follows. For the first question, we note that 
{First}, when both $v_1$ and $v_2$ are not in $S_p$, $S_p$ cannot be maximal since we can add $v_1$ into $S_p$ to form a larger clique. {Second}, it is easy to see that when $v_{i}\in S_p$, $v_{i+1}$ cannot be in $S_p$ since they are disconnected with each other in $g_C$. Thus, one possible choice is to add $v_{i+2}$ to $S_p$. Besides, there exists another choice that we also exclude $v_{i+2}$ from $S_p$ but include $v_{i+3}$ into $S_p$. In this case, adding $v_{i+1}$ or $v_{i+2}$ to $S_p$ cannot form a larger clique since $v_i$ disconnects with $v_{i+1}$ in $g_C$ and $v_{i+2}$ disconnects with $v_{i+3}$ in $g_C$. For other expansion that does not include $v_{i+2}$ and $v_{i+3}$ {\cheng inside}, $S_p$ cannot be maximal since we can add $v_{i+2}$ into $S_p$ to form a larger clique.  
An illustration of enumerating maximal cliques in a given path $p$ is shown in Figure~\ref{fig:path-1} and Figure~\ref{fig:path-2}. The pseudo-codes of function \textsf{Enum\_from\_Path($p$)} is shown in Algorithm~\ref{alg:enum_path}. 
% We provide the illustration and the pseudo-code of the above procedure in \textsf{Enum\_from\_Path($p$)} in Appendix~\ref{sec:app-early}. 
% An illustration is shown in Figure~\ref{fig:path-1} and Figure~\ref{fig:path-2}. We present 
% The  is shown in Algorithm~\ref{alg:enum_path}. 





% \begin{algorithm}[t]
% \small
% \caption{Function \textsf{Enum\_from\_Path($p$)}}
% \label{alg:enum_path}
% \KwIn{A path $p=\{v_1, v_2, \cdots, v_{|p|}\}$ in $\overline{g}_C$.}
% \KwOut{All maximal cliques of $g_C$ induced with the vertices in $p$.}
% \SetKwFunction{List}{\textsf{Enum\_Rec}}
% % \SetKwFunction{ListCycle}{\textsf{Enum\_Rec}}
% \SetKwProg{Fn}{Procedure}{}{}
% $\mathbb{S}\gets \emptyset$\;
% \List{$\mathbb{S}, \{v_1\}, p$}; \List{$\mathbb{S}, \{v_2\}, p$}\;
% \Return $\mathbb{S}$\;
% \Fn{\List{$\mathbb{S}, S_p, p$}}{
%     $v_i\gets$ the last vertex in $S_p$\;
%     \If{$i+2>|p|$}{
%         $\mathbb{S}\gets \mathbb{S} \cup \{S_p\}$;
%         \Return\;
%     }
%     \List{$\mathbb{S}, S_p\cup\{v_{i+2}\}, p$}\;
%     \lIf{$i+3\le|p|$}{
%         \List{$\mathbb{S}, S_p\cup\{v_{i+3}\}, p$}
%     }
% }
% \end{algorithm}


% \begin{algorithm}[t]
% \small
% \caption{Function \textsf{Enum\_from\_Cycle($c$)}}
% \label{alg:enum_cycle}
% \KwIn{A cycle $c=\{v_1, v_2, \cdots, v_{|c|}\}$ in $\overline{g}_C$.}
% \KwOut{All maximal cliques of $g_C$ induced with the vertices in $c$.}
% \SetKwFunction{List}{\textsf{Enum\_Rec}}
% % \SetKwFunction{ListCycle}{\textsf{Enum\_Rec}}
% \SetKwProg{Fn}{Procedure}{}{}
% \lIf{$|c|=3$}{\Return $\{\{v_1\},\{v_2\},\{v_3\}\}$}
% \lIf{$|c|=4$}{\Return $\{\{v_1,v_3\},\{v_2,v_4\}\}$}
% \lIf{$|c|=5$}{\Return $\{\{v_1,v_3\},\{v_1, v_4\},\{v_2,v_4\},\{v_2,v_5\},\{v_3,v_5\}\}$}
% \If{$|c|\ge 6$} {
% $\mathbb{S}\gets\emptyset$\;
% \List{$\mathbb{S}, \{v_1\}, \{v_1, v_2, \cdots, v_{|c|-1}\}$}\;
% \List{$\mathbb{S}, \{v_2\}, \{v_2, v_3, \cdots, v_{|c|}\}$}\;
% \List{$\mathbb{S}, \{v_{|c|}, v_3\}, \{v_3, v_4, \cdots, v_{|c|-2}\}$}\;
% \Return $\mathbb{S}$\;
% }
% % $\mathbb{S}\gets \emptyset$\;
% % \List{$\mathbb{S}, \{v_1\}$}; \List{$\mathbb{S}, \{v_2\}$}\;
% % \Return $\mathbb{S}$\;
% % \Fn{\List{$\mathbb{S}, S_p$}}{
% %     $v_i\gets$ the last vertex in $S_p$\;
% %     \If{$i+2>|p|$}{
% %         $\mathbb{S}\gets \mathbb{S} \cup S_p$;
% %         \Return\;
% %     }
% %     \List{$\mathbb{S}, S_p\cup\{v_{i+2}\}$}\;
% %     \lIf{$i+3\le|p|$}{
% %         \List{$\mathbb{S}, S_p\cup\{v_{i+3}\}$}
% %     }
% % }
% \end{algorithm}








% Given a path $p=\{v_1, v_2, \cdots, v_{|p|}\}$, let $S_p$ be a subset of $V(p)$ that induces a clique of $g_C$. We construct a maximal clique by recursively adding vertices from $V(p)$ to $S_p$ until it is maximal. There are two possible cases: (1) $v_1\in S_p$ and (2) $v_1\notin S_p$ but $v_2\in S_p$. We note that when both $v_1$ and $v_2$ are not in $S_p$, $S_p$ cannot be maximal since we can add at least one vertex $v_1$ into $S_p$ to form a larger clique. 

% \noindent\textbf{Case 1 - $v_1\in S_p$.} Let $v_i$ be the last vertex added into $S_p$. Since $v_{i+1}$ disconnects with $v_i$ in $g_C$, it cannot be added into $S_p$. Then the next vertex that can be added into $S_p$ is $v_{i+2}$. Apart from this 




% \noindent\textbf{Case 2 - $v_2\in S_p$.}


% and $v_{|p|}$ disconnects with $v_2$ and $v_{|p|-1}$ in $g_C$, respectively, and  









% \begin{figure}[t]
% \centering
% \subfigure[Case 1 and 2: $v_1\in S_c$ or $v_2\in S_c$.]{
% \label{fig:cycle-1}
% \includegraphics[width=0.225\textwidth]{figs/path-cycle/cycle-1.pdf}}
% \subfigure[Case 3: $v_1, v_2\notin S_c$.]{
% \label{fig:cycle-2}
% \includegraphics[width=0.23\textwidth]{figs/path-cycle/cycle-2.pdf}}
% \caption{ Three possible cases to enumerate all maximal cliques given a cycle $c$. Note that ``Include'' (resp. ``Exclude'') means that the vertices that are included in (resp. excluded from) a maximal clique. }
% \label{fig:cycle}
% \end{figure}




% \smallskip
\noindent\textbf{Category 2 - Cycles.}
%
For a cycle $c = \{v_1, v_2, \cdots, v_{|c|}\}$ in $\overline{g}_C$ ($|c|\ge 3$), the vertices are in the order where $(v_i, v_{i+1})\in E(\overline{g}_C)$. 
% We note that $(v_1, v_{|c|})$ also is an edge in $\overline{g}_C$. Similarly, it implies that for any vertex $v_i$, it disconnects with two vertices $v_{i-1}$ and $v_{i+1}$ in $g_C$ for $1\le i\le |c|$. We note that $v_0$ and $v_{|c|+1}$ correspond to $v_{|c|}$ and $v_1$, respectively. 
% Next, we will present how we can enumerate all maximal cliques in $g_C$ within the vertices of a cycle $c$ in $\overline{g}_C$. 
% We note that 
When $|c|=3$, $|c|=4$ and $|c|=5$, the maximal cliques are $\{\{v_1\}, \{v_2\}, \{v_3\}\}$, $\{\{v_1, v_3\}, \{v_2, v_4\}\}$ and $\{\{v_1,v_3\},\{v_1, v_4\},\{v_2,v_4\},\{v_2,v_5\},\{v_3,v_5\}\}$, respectively. 
For $|c|\ge 6$, there are three possible cases, each of which can be reduced to enumerate maximal cliques given a simple path in $\overline{g}_C$ as described in Category 1. Let $S_c$ be a subset of $V(c)$ that induces a maximal clique of $g_C$.

\begin{itemize}[leftmargin=*]
    \item \textbf{Case 1 - $v_1\in S_c$.} Consider \emph{path} $p = \{v_1, v_2, \cdots, v_{|c|-1}\}$. All maximal cliques within $c$ can be enumerated by following three steps in Category 1 with initialization $S_p=\{v_1\}$. 
    % (since the initialization $\{v_2\}$ cannot guarantee that $v_1\in S_c$). 
    
    
    \item \textbf{Case 2 - $v_2\in S_c$.} Consider \emph{path} $p=\{v_2, v_3, \cdots, v_{|c|}\}$. All maximal cliques within $c$ can be enumerated by following three steps in Category 1 with initialization $S_p=\{v_2\}$. 
    % (since the initialization $\{v_1\}$ cannot guarantee that $v_2\in S_c$). 


    \item \textbf{Case 3 - $v_1, v_2\notin S_c$.} Consider \emph{path} $p=\{v_3, \cdots, v_{|c|-2}\}$. All maximal cliques within $c$ can be enumerated by following three steps in Category 1 with initialization $S_p=\{v_{|c|}, v_3\}$. 
    % If the path $p$ satisfies $|p|\ge 2$, then for each maximal clique $S_p$ enumerated by the three steps in Category 1 with initialization $\{v_3\}$, we can report a maximal clique $S_c = S_p\cup \{v_{|c|}\}$; otherwise, we directly report $S_c=\{v_3, v_{|c|}\}$. 
    % Let $S_c$ be a subset of $V(c)$ that induces a partial clique of $g_C$. There are three possible choices to initialize $S_c$: (1) $S_c = \{v_1\}$, (2) $S_c = \{v_2\}$ and (3) $S_c = \{v_3, v_{|c|}\}$. 
    % \item \textbf{Step 2 - Expand.} For each initialization $S_c$, we expand it by the following three cases. 
    % \begin{itemize}[leftmargin=*]
    %     \item \textbf{Case $S_c = \{v_1\}$.} We generate a path $p' = \{v_3, v_4, \cdots, v_{|c|-1}\}$ (if any). Then for each maximal clique $S_{p'}$ that can be enumerated within the vertices in $p'$ (e.g., via Algorithm~\ref{alg:enum_path}), $S_c\cup S_{p'}$ is a maximal clique induced by the vertices of $V(c)$.
    %     \item \textbf{Case $S_c = \{v_2\}$.} We generate a path $p''=\{v_4, v_5, \cdots, v_{|c|}\}$ (if any). Then for each maximal clique $S_{p''}$ that can be enumerated with the vertices in $p''$ (e.g., via Algorithm~\ref{alg:enum_path}), $S_c\cup S_{p''}$ is a maximal clique induced by the vertices of $V(c)$.
    %     \item \textbf{Case $S_c = \{v_3, v_{|c|}\}$.} We generate a path $p'''=\{v_5, v_6, \cdots, v_{|c|-2}\}$ (if any). Then for each maximal clique $S_{p'''}$ that can be enumerated with the vertices in $p'''$ (e.g., via Algorithm~\ref{alg:enum_path}), $S_c\cup S_{p'''}$ is a maximal clique induced by the vertices of $V(c)$.
    % \end{itemize}
\end{itemize} 




\begin{figure}[t]
\centering
\subfigure[Expand $S_p$ with $v_{i+2}$.]{
\label{fig:path-1}
\includegraphics[width=0.23\textwidth]{figs/path-cycle/path-1.pdf}}
\subfigure[Expand $S_p$ with $v_{i+3}$.]{
\label{fig:path-2}
\includegraphics[width=0.23\textwidth]{figs/path-cycle/path-2.pdf}}
\subfigure[Case 1 \& 2: $v_1\in S_c$ or $v_2\in S_c$.]{
\label{fig:cycle-1}
\includegraphics[width=0.225\textwidth]{figs/path-cycle/cycle-1.pdf}}
\subfigure[Case 3: $v_1, v_2\notin S_c$.]{
\label{fig:cycle-2}
\includegraphics[width=0.23\textwidth]{figs/path-cycle/cycle-2.pdf}}
\caption{ (a) and (b) show two possible cases to expand a partial maximal clique $S_p$ of a given path $p$ when $v_i\in S_p$ is the last vertex. 
(c) and (d) show three possible cases to enumerate all maximal cliques given a cycle $c$. Note that ``Include'' (resp. ``Exclude'') means that the vertices that are included in (resp. excluded from) a maximal clique. }
\label{fig:cases}
\end{figure}


% \begin{figure}[t]
% \vspace{-4mm}
% \centering
% \subfigure[Expand $S_p$ with $v_{i+2}$.]{
% \label{fig:path-1}
% \includegraphics[width=0.23\textwidth]{figs/path-cycle/path-1.pdf}}
% \subfigure[Expand $S_p$ with $v_{i+3}$.]{
% \label{fig:path-2}
% \includegraphics[width=0.23\textwidth]{figs/path-cycle/path-2.pdf}}
% \subfigure[Case 1 and Case 2: $v_1\in S_c$ or $v_2\in S_c$.]{
% \label{fig:cycle-1}
% \includegraphics[width=0.225\textwidth]{figs/path-cycle/cycle-1.pdf}}
% \subfigure[Case 3: $v_1, v_2\notin S_c$.]{
% \label{fig:cycle-2}
% \includegraphics[width=0.23\textwidth]{figs/path-cycle/cycle-2.pdf}}
% \vspace{-3mm}
% \caption{ (a) and (b) show two possible cases to expand a partial maximal clique $S_p$ of a given path $p$ when $v_i\in S_p$ is the last vertex. 
% (c) and (d) show three possible cases to enumerate all maximal cliques given a cycle $c$. Note that ``Include'' (resp. ``Exclude'') means that the vertices that are included in (resp. excluded from) a maximal clique. }
% \label{fig:cases}
% \vspace{-5mm}
% \end{figure}






\begin{algorithm}[t]
% \small
\caption{{Enumerate} maximal cliques in a 3-plex}
\label{alg:MC3Plex}
\KwIn{A branch $B=(S,g_C,g_X)$ where $g_C$ is to a 3-plex and $g_X$ is an empty graph.}
\KwOut{All maximal cliques within $B$.}
\SetKwFunction{ListPath}{\textsf{Enum\_from\_Path}}
\SetKwFunction{ListCycle}{\textsf{Enum\_from\_Cycle}}
\SetKwProg{Fn}{Procedure}{}{}
Construct the inverse graph $\overline{g}_C$ of $g_C$\;
$F, \mathcal{P}, \mathcal{C}\gets$ set of the isolated vertices, paths and cycles in $\overline{g}_C$\;
\lFor{each path $p_i\in \mathcal{P}$}{
$\mathbb{S}_{p_i}\gets$\ListPath{$p_i$}
}
\lFor{each cycle $c_i\in \mathcal{C}$}{
$\mathbb{S}_{c_i}\gets$\ListCycle{$c_i$}
}

\For{each combination $(S_{p_1},S_{p_2},\cdots,S_{p_{|\mathcal{P}|}})$ where $S_{p_i}\in \mathbb{S}_{p_i}$}{
\For{each combination $(S_{c_1},S_{c_2},\cdots,S_{c_{|\mathcal{C}|}})$ where $S_{c_j}\in \mathbb{S}_{c_j}$}{
    $S'\gets F\cup \Big(\bigcup_{i=1}^{|\mathcal{P}|} S_{p_i}\Big) \cup \Big(\bigcup_{j=1}^{|\mathcal{C}|} S_{c_j}\Big)$\;
    % \If{$N(S\cup S', G)\cap V(g_X)=\emptyset$}{
        \textbf{Output} a maximal clique $S\cup S'$\;
    % }
}
}
\end{algorithm}


% \noindent\textit{Correctness.}
\noindent\textbf{{\chengB Correctness}.}
% The rationale of the above procedure is as follows. 
For Case 1, when $v_1\in S_c$, $v_{|c|}$ must not be in $S_c$ since they are connected in $\overline{g}_C$. It corresponds to finding maximal cliques from the vertices in $\{v_1, v_2, \cdots, v_{|c|-1}\}$ with $v_1$ required to be inside. For Case 2, when $v_2\in S_c$, $v_1$ must not be in $S_c$. It corresponds to finding maximal cliques from the vertices in $\{v_2, \cdots, v_{|c|}\}$ with $v_2$ required to be inside. For Case 3, when $v_1,v_2\notin S_c$, to ensure the maximality of $S_c$, $v_3$ and $v_{|c|}$ must be in $S_c$ since otherwise, we can add $v_1$ or $v_2$ to $S_c$ to form a larger clique. As $v_3$ and $v_{|c|}$ are both in $S_c$, $v_{|c|-1}$ must not be in $S_c$. It corresponds to finding maximal cliques from the vertices in $\{v_3, \cdots, v_{|c|-2}\}$ with $v_3$ required to be inside. 
An illustration of enumerating maximal cliques in a given cycle $c$ is shown in Figure~\ref{fig:cycle-1} and Figure~\ref{fig:cycle-2}. The pseudo-codes of function \textsf{Enum\_from\_Cycle($c$)} is shown in Algorithm~\ref{alg:enum_cycle}. 



% We provide an illustration and the pseudo-code of the above procedure in \textsf{Enum\_from\_Cycle($c$)} in Appendix~\ref{sec:app-early}. 
% An illustration is shown in Figure~\ref{fig:cycle-1} and Figure~\ref{fig:cycle-2}. We present the pseudo-code of the above procedure in \textsf{Enum\_from\_Cycle($c$)} in the appendix. 




% We note that there is no other shape of the connected components in $\overline{g}_C$. 
% We will provide a formal proof of this claim in the appendix. 
Once the maximal cliques within each cycle and path are enumerated, we combine them together to form the maximal cliques in $g_C$. We summarize the procedure in lines {\yui 5-8} of Algorithm~\ref{alg:MC3Plex}. 
% Finally, we check the maximality for each maximal clique in $g_C$. 


% \smallskip
% \noindent\textbf{Example.}
% %
% Consider the example of a 3-plex and its inverse graph in Figure~\ref{fig:3-plex}. Based on the definitions, the inverse graph contains a path $p=\{v_1, v_2, v_3\}$ and a cycle $c=\{v_4, v_5, v_6\}$. Consider the path $p$. It has two partial maximal cliques inside, i.e., $\{v_1,v_3\}$ and $\{v_2\}$. Consider the cycle $c$. It has three partial cliques inside, i.e., $\{v_4\}$, $\{v_5\}$ and $\{v_6\}$. Therefore, there are 6 maximal cliques in $g_C$, i.e., $\{v_1, v_3, v_4\}$, $\{v_1, v_3,v_5\}$, $\{v_1, v_3,v_5\}$, $\{v_2, v_4\}$, $\{v_2,v_5\}$ and $\{v_2, v_6\}$. 



% \begin{figure}[t]
% \subfigure[An example 3-plex graph $g_C$.]{
%     \label{subfig:3-plex}
%     \includegraphics[width=0.20\textwidth]{figs/plex/plex3.pdf}}
% \subfigure[Inverse graph $\overline{g}_C$ of 3-plex $g_C$.]{
%     \label{subfig:3-plex-inv}
%     \includegraphics[width=0.20\textwidth]{figs/plex/plex3inv.pdf}}
% % \subfigure[An example 3-plex graph $g$.]{
% %     \label{subfig:3-plex}
% %     \includegraphics[width=0.20\textwidth]{figs/plex/plex3.pdf}}
% % \subfigure[Inverse graph $g_{inv}$ of 3-plex $g$.]{
% %     \label{subfig:3-plex-inv}
% %     \includegraphics[width=0.20\textwidth]{figs/plex/plex3inv.pdf}}
% \caption{{Example of a 3-plex and its inverse graph.}} 
% \label{fig:3-plex}
% \end{figure}


% \smallskip
% \noindent\textbf{Example.}
% %
% Consider the example of a 3-plex and its inverse graph in Figure~\ref{fig:3-plex}. Based on the definitions, the inverse graph contains a path $p=\{v_1, v_2, v_3\}$ and a cycle $c=\{v_4, v_5, v_6\}$. Consider the path $p$. It has two partial maximal cliques inside, i.e., $\{v_1,v_3\}$ and $\{v_2\}$. Consider the cycle $c$. It has three partial cliques inside, i.e., $\{v_4\}$, $\{v_5\}$ and $\{v_6\}$. Therefore, there are 6 maximal cliques in $g_C$, i.e., $\{v_1, v_3, v_4\}$, $\{v_1, v_3,v_5\}$, $\{v_1, v_3,v_5\}$, $\{v_2, v_4\}$, $\{v_2,v_5\}$ and $\{v_2, v_6\}$. 




% \smallskip
% \noindent\textbf{Complexity.} We analyze the time complexity of Algorithm~\ref{alg:MC3Plex} as follows.

\begin{theorem}
\label{theo:complex-within-3plex}
    Given a branch $B=(S,g_C,g_X)$ with $g_C$ being a 3-plex and $g_X$ {\cheng being} an empty graph, Algorithm~\ref{alg:MC3Plex} enumerates all maximal cliques within $B$ in $O(E(g_C) + \omega(g_C) \cdot c(g_C))$ time, where $\omega(g_C)$ is the size of the largest maximal clique within $B$ and $c(g_C)$ is the number of maximal cliques in $g_C$.
    % and bounded by $3^{|V(g_C)|/3}$, i.e., $c(g_C)\le 3^{|V(g_C)|/3}$. 
\end{theorem}


\begin{proof}
    First, Algorithm~\ref{alg:MC3Plex} takes $O(E(g_C))$ {\cheng time} for partitioning $V(g_C)$ into three sets (line 1). In each round of lines 7-10,  the algorithm guarantees exactly one maximal clique of $g_C$ to be found.
\end{proof}

% \begin{proof}
%     First, Algorithm~\ref{alg:MC3Plex} takes $O(E(g_C))$ {\cheng time} for partitioning $V(g_C)$ into three sets (line 1). In each round of lines 7-10,  the algorithm can guarantee exactly one maximal clique of $g_C$ to be outputted.
% \end{proof}


{\kaixin Similarly, Algorithm~\ref{alg:MC3Plex} also achieves a \emph{nearly optimal} time complexity since $O(\omega(g_C) \cdot c(g_C))$ is the optimal time  and Algorithm~\ref{alg:MC3Plex} only takes $O(E(g_C))$ {\chengB extra} time.}



% \begin{figure}[t]
% \centering
% \subfigure[ 3-plex graph $g_C$.]{
%     \label{subfig:3-plex}
%     \includegraphics[width=0.21\textwidth]{figs/plex/plex3.pdf}}
% \hspace{2mm}
% \subfigure[Inverse graph $\overline{g}_C$ of $g_C$.]{
%     \label{subfig:3-plex-inv}
%     \includegraphics[width=0.21\textwidth]{figs/plex/plex3inv.pdf}}
% % \subfigure[An example 3-plex graph $g$.]{
% %     \label{subfig:3-plex}
% %     \includegraphics[width=0.20\textwidth]{figs/plex/plex3.pdf}}
% % \subfigure[Inverse graph $g_{inv}$ of 3-plex $g$.]{
% %     \label{subfig:3-plex-inv}
% %     \includegraphics[width=0.20\textwidth]{figs/plex/plex3inv.pdf}}
% \caption{{Example of a 3-plex and its inverse graph.}} 
% \label{fig:3-plex}
% \vspace{-3mm}
% \end{figure}

% \smallskip
% \noindent\textbf{Example.}
% %
% Consider the example of a 3-plex and its inverse graph in Figure~\ref{fig:3-plex}. Based on the definitions, the inverse graph contains a path $p=\{v_1, v_2, v_3\}$ and a cycle $c=\{v_4, v_5, v_6\}$. Consider the path $p$. It has two partial maximal cliques inside, i.e., $\{v_1,v_3\}$ and $\{v_2\}$. Consider the cycle $c$. It has three partial cliques inside, i.e., $\{v_4\}$, $\{v_5\}$ and $\{v_6\}$. Therefore, there are 6 maximal cliques in $g_C$, i.e., $\{v_1, v_3, v_4\}$, $\{v_1, v_3,v_5\}$, $\{v_1, v_3,v_5\}$, $\{v_2, v_4\}$, $\{v_2,v_5\}$ and $\{v_2, v_6\}$. 

% \begin{theorem}
% \label{theo:hbbmc-with-3plex}
%     Given a graph $G=(V,E)$, the time complexity of \texttt{HBBMC} with early-termination from 3-plexes is $O(\delta m + \tau m \cdot 3^{\tau/3})$. 
%     % , where $\omega$ is the number of maximal cliques in $G$. 
% \end{theorem}

% \begin{proof}
%     The logic of the proof is similar to that of Theorem~\ref{theo:hbbmc-with-2plex}. Specifically, \texttt{HBBMC} with the early-termination from 3-plex is nearly optimal, and thus its time complexity would not be worse than $O(\delta m + \tau m \cdot 3^{\tau/3})$. Besides, when both conditions for the early-termination are not satisfied simultaneously in any branch in the worst case, the time complexity of \texttt{HBBMC} with early-termination from 3-plexes is $O(\delta m + \tau m \cdot 3^{\tau/3})$.
% \end{proof}


% \smallskip
% \noindent\textbf{Remark.}
% %
% We note that the early-termination technique is  orthogonal to all BB frameworks, including all existing \texttt{VBBMC} algorithms and \texttt{HBBMC} algorithm. With the early-termination technique, the algorithm will retain the same time complexity provided before but run practically much faster as verified in the experiments. 
% %
% Besides, the strategy is supposed to set a small threshold $t$ so as to apply the early-termination from different density of the candidate graphs (i.e., $t$-plexes with different $t$). We vary $t$ in the range $\{0,1,2,3\}$. Note that setting $t=0$ corresponds to the case where the algorithm does not apply the early-termination technique. The results show that $t=3$ runs comparably faster than other choices. 


\begin{table*}[ht]
\vspace{-3mm}
    \begin{minipage}{.46\textwidth}
    \scriptsize
    \centering
    \caption{Dataset Statistics.}
    \vspace{-2mm}
    \label{tab:data}
    \begin{tabular}{r|r|rr|rrr}
    \hline
        \textbf{Graph (Name)} & {Category} & $|V|$ & $|E|$ & $\delta$ & $\tau$ & $\rho$ \\
    \hline
        \textsf{nasasrb (NA)} & {Social Network} & 54,870 & 1,311,227 & 35 & 22 &  23.9 \\ %nasasrb
        \textsf{fbwosn (FB)} & {Social Network} & 63,731 & 817,090 & 52 & 35 &  12.8 \\ %fbwosn
        \textsf{websk (WE)} & {Web Graph} & 121,422 & 334,419 & 81 & 80 &  2.8 \\ %websk
        \textsf{wikitrust (WK)} & {Web Graph} & 138,587 & 715,883  & 64 & 31 & 5.2 \\ %wikitrust
        \textsf{shipsec5 (SH)} & {Social Network} & 179,104 & 2,200,076  & 29 & 22 &  12.3 \\ %shipsec5   
        \textsf{stanford (ST)} & {Social Network} & 281,904 & 1,992,636 & 86 & 61 & 7.1 \\ %stanford
        \textsf{dblp (DB)} & {Collaboration} & 317,080 & 1,049,866 & 113 & 112 & 3.3 \\ %dblp
        \textsf{dielfilter (DE)} & {Other} & 420,408 & 16,232,900 & 56 & 43 & 38.6 \\ % dielfilter
        \textsf{digg (DG)} & {Social Network} & 770,799 & 5,907,132 & 236 & 72 & 7.7  \\ %digg
        \textsf{youtube (YO)} & {Social Network} &1,134,890 & 2,987,624 & 49 & 18 & 2.6 \\ %youtube
        \textsf{pokec (PO)} & {Social Network} & 1,632,803 & 22,301,964 & 47 & 27 & 13.7 \\ %pokec
        \textsf{skitter (SK)} & {Web Graph} & 1,696,415 & 11,095,298 & 111 & 67 & 6.5 \\ %skitter
        \textsf{wikicn (CN)} & {Web Graph} & 1,930,270 & 8,956,902 & 127 & 31 & 4.6 \\ %wikicn
        \textsf{baidu (BA)} & {Web Graph} & 2,140,198 & 17,014,946 & 82 & 29 & 8.0 \\ %baidu
        \textsf{orkut (OR)} & {Social Network} & 2,997,166 & 106,349,209 & 253 & 74 & 35.5 \\ % orkut 
        \textsf{socfba (SO)} & {Social Network} & 3,097,165 &  23,667,394 &  74 & 29 &  7.6 \\ %socfba
        % \textsf{wikipedia (WP)} &  25,921,548 &  543,183,611 &  4M &  1120 &  426 &  21.0 \\
        % \textsf{clueweb (CW)} &  147,925,593 &  446,766,953 & 1M &  192 &  83 &  3.0  \\
    % \hline
         % \textsf{allwebuk (UK)}  &  18,483,186  &  261,787,258 &  3M &  943 &  942 &  14.2  \\   
    \hline
    \end{tabular}
    \end{minipage}
    \hspace{15mm}
\begin{minipage}{.46\textwidth}
\scriptsize
    \centering
    \caption{Comparison with baselines (unit: second).}
\vspace{-2mm}
    \label{tab:real}
    \begin{tabular}{c|rrrrr}
    \hline
         & \texttt{HBBMC++} & \texttt{RRef} & \texttt{RDegen} & \texttt{RRcd} & \texttt{RFac} \\ \hline
\textsf{NA} & \textbf{0.33} & 0.58 & 0.48 & \underline{0.46} & 0.61 \\
\textsf{FB} & \textbf{1.10} & 1.78 & 1.67 & \underline{1.24} & 1.70 \\
\textsf{WE} & \textbf{0.02} & 0.11 & \underline{0.08} & 0.12 & 0.17 \\
\textsf{WK} & \textbf{0.57} & 1.12 & 1.03 & \underline{1.01} & 1.68 \\
\textsf{SH} & \textbf{0.45} & 1.05 & 0.98 & \underline{0.78} & 1.15 \\
\textsf{ST} & \textbf{1.26} & 2.15 & 1.70 & \underline{1.67} & 5.07 \\
\textsf{DB} & \textbf{0.16} & 0.53 & \underline{0.47} & 0.49 & 0.83 \\
\textsf{DE} & \textbf{3.82} & 8.29 & 7.47 & \underline{5.76} & 9.91 \\ 
\textsf{DG} & \textbf{239.58} & 1441.22 & \underline{1046.40} & 1518.36 & 1603.08 \\
\textsf{YO} & \textbf{1.47} & 2.85 & 2.32 & \underline{2.19} & 6.45  \\
\textsf{PO} & \textbf{19.31} & 32.47 & \underline{25.96} & 26.38 & 31.66 \\
\textsf{SK} & \textbf{25.15} & 65.27 & 47.11 & \underline{44.90} & 71.96 \\
\textsf{CN} & \textbf{6.03} & 14.07 & \underline{11.18} & 12.65 & 20.37 \\
\textsf{BA} & \textbf{13.81} & 28.67 & 22.61 & \underline{20.59} & 36.51 \\
\textsf{OR} & \textbf{884.20} & 2297.57 & \underline{2200.54} & 2410.93 & 2749.32 \\
\textsf{SO} & \textbf{21.12} & 40.58 & 39.61 & \underline{37.44} & 42.91 \\
\hline
    \end{tabular}
\end{minipage}
\vspace{-4mm}
\end{table*}



\smallskip
\noindent\textbf{Remarks.}
\underline{First}, the early-termination technique is orthogonal to all BB frameworks, including existing \texttt{VBBMC} algorithms and the \texttt{HBBMC} algorithm. With the early-termination technique, all BB algorithms retain the same time complexities provided before but run significantly faster in practice, as verified in experiments. Additionally, the strategy involves setting a small threshold $t$ to apply early-termination to different densities of candidate graphs (i.e., $t$-plexes with varying $t$). We vary $t\in\{1,2,3\}$ {\chengB in experiments} and the results indicate that $t=3$ achieves higher speedup over other choices.
%
% {\Revise
\underline{Second}, the overhead of checking the early-termination condition is negligible. In the \texttt{HBBMC} framework, the pivoting strategy prunes branches that do not contain any maximal cliques. For a branch $B = (S, g_C, g_X)$, we calculate $d(v, g_C)$, the number of neighbors in $g_C$ for each $v \in V(g_C) \cup V(g_X)$, and select the vertex $v^*$ with the maximum $d(\cdot, g_C)$ as the pivot. The condition for $g_C$ being a 2-plex (or 3-plex) can be checked simultaneously with pivot selection: $g_C$ is a 2-plex (or 3-plex) if the minimum $d(v, g_C)$ for any $v \in V(g_C)$ is at least $|V(g_C)| - 2$ (or $|V(g_C)| - 3$). Let $u_m$ be the vertex with the minimum $d(\cdot, g_C)$. Since $d(u, g_C) \ge d(u_m, g_C) \ge |V(g_C)| - 2$ (or $|V(g_C)| - 3$) for all $u \in V(g_C)$, $g_C$ is confirmed as a 2-plex (or 3-plex). This check only adds $O(|V(g_C)|)$ time per branch, which we consider acceptable.
% }
{\kaixinC \underline{Third}, while the high-level idea of early-termination technique exists for enumeration problem (e.g., \cite{wang2024technical, dai2023hereditary}), our design is different from the existing ones and specific to MCE problem. 
% our proposed method directly outputs all maximal cliques inside without branching, which is not considered in existing studies for MCE problem. Moreover, 
Specifically, for $k$-clique listing problem \cite{wang2024technical}, the design follows a combinatorial manner to find all vertices that are connected with each other; while for MCE problem, our design iteratively adds all possible vertices until no vertex can be added (i.e., adding any vertex {\chengc would} induce a non-clique). For maximal biclique enumeration problem \cite{dai2023hereditary}, the termination is applied when candidate subgraphs have no edges inside; while for MCE problem, the termination is applied for dense candidate subgraphs.
\underline{Fourth}, our design is totally different from simply converting the original recursive procedure into an iterative loop. The reason is as follows. On the one hand, it is hard to convert the original recursive process into a loop since it needs to manually maintain a stack of various variables for conducting the pivot selection and pruning techniques. Thus, existing algorithms including BK and its variants are all implemented in a recursive way. On the other hand, our introduced method takes the advantages of the topological information of the $t$-plexes (with different values of $t$), which can be naturally implemented in an iterative way as shown in Algorithm~\ref{alg:MC2Plex} and Algorithm~\ref{alg:MC3Plex}. This should also be regarded as one of potential benefits of our method. We also provide examples of enumerating maximal cliques from 2-plex and 3-plex in the Appendix~\ref{app:example}.}










==> 5._exp.tex <==

\section{Experiments}
\label{sec:exp}


\subsection{Experimental Setup}
\label{subsec:setup}







% % \begin{figure*}[t]
% % \vspace{-5mm}
% % \subfigure[\textsf{NA}]{
% %     \includegraphics[width=0.24\textwidth]{figs/small/nasasrb.pdf}}
% % \subfigure[\textsf{FB}]{
% %     \includegraphics[width=0.24\textwidth]{figs/small/facebook.pdf}}
% % \subfigure[\textsf{WK}]{
% %     \includegraphics[width=0.24\textwidth]{figs/small/wiki.pdf}}
% % \subfigure[\textsf{SH}]{
% %     \includegraphics[width=0.24\textwidth]{figs/small/shipsec.pdf}}
% % \subfigure[{\kaixinB \textsf{SO}}]{
% % \label{subfig:a}
% %     \includegraphics[width=0.24\textwidth]{figs/small/a.pdf}}
% % \subfigure[\textsf{PO}]{
% %     \includegraphics[width=0.24\textwidth]{figs/small/pokec.pdf}}
% % \subfigure[\textsf{CN}]{
% %     \includegraphics[width=0.24\textwidth]{figs/small/cn.pdf}}
% % \subfigure[\textsf{BA}]{
% %     \includegraphics[width=0.24\textwidth]{figs/small/baidu.pdf}}
% % \vspace{-5mm}
% % \caption{Comparison with baselines on the small-$\omega$ graphs, varying $k$ from 4 to $\omega$.}
% % % \vspace{-2mm}
% % \label{fig:real-small}
% % \end{figure*}


% % \begin{figure*}[t]
% % \vspace{-3mm}
% % \subfigure[\textsf{WE}]{
% %     \includegraphics[width=0.24\textwidth]{figs/large/sk.pdf}}
% % \subfigure[\textsf{CI}]{
% %     \includegraphics[width=0.24\textwidth]{figs/large/citeseer.pdf}}
% % \subfigure[\textsf{ST}]{
% %     \includegraphics[width=0.24\textwidth]{figs/large/stanford.pdf}}
% % \subfigure[\textsf{DB}]{
% %     \includegraphics[width=0.24\textwidth]{figs/large/dblp.pdf}}
% % \subfigure[\textsf{DE}]{
% %     \includegraphics[width=0.24\textwidth]{figs/large/diel.pdf}}
% % \subfigure[\textsf{DG}]{
% %     \includegraphics[width=0.24\textwidth]{figs/large/digg.pdf}}
% % \subfigure[\textsf{SK}]{
% %     \includegraphics[width=0.24\textwidth]{figs/large/skitter.pdf}}
% % \subfigure[\textsf{OR}]{
% %     \includegraphics[width=0.24\textwidth]{figs/large/orkut.pdf}}
% % \vspace{-5mm}
% % \caption{Comparison with baselines on the large-$\omega$ graphs, varying $k$ from 4 to 9 and from $\omega-5$ to $\omega$.}
% % \label{fig:real-large}
% % \vspace{-2mm}
% % \end{figure*}



% % \begin{figure*}[t]
% % \subfigure[\textsf{NA}]{
% %     \includegraphics[width=0.24\textwidth]{figs/nasasrb-effect.pdf}}
% % \subfigure[\textsf{FB}]{
% %     \includegraphics[width=0.24\textwidth]{figs/fbwosn-effect.pdf}}
% % \subfigure[\textsf{WI}]{
% %     \includegraphics[width=0.24\textwidth]{figs/wikitrust-effect.pdf}}
% % \subfigure[\textsf{SH}]{
% %     \includegraphics[width=0.24\textwidth]{figs/shipsec5-effect.pdf}}
% % \subfigure[\textsf{YO}]{
% %     \includegraphics[width=0.24\textwidth]{figs/youtube-effect.pdf}}
% % \subfigure[\textsf{PO}]{
% %     \includegraphics[width=0.24\textwidth]{figs/pokec-effect.pdf}}
% % \subfigure[\textsf{WK}]{
% %     \includegraphics[width=0.24\textwidth]{figs/cn-effect.pdf}}
% % \subfigure[\textsf{BA}]{
% %     \includegraphics[width=0.24\textwidth]{figs/baidu-effect.pdf}}
% % \caption{Comparison among variants on the small-$\omega$ graphs.}
% % \label{fig:real-small-effect}
% % \end{figure*}







% % \begin{figure*}[ht]
% % \subfigure[\textsf{WE} (small $k$)]{
% %     \includegraphics[width=0.24\textwidth]{figs/sk-small-effect.pdf}}
% % \subfigure[\textsf{WE} (large $k$)]{
% %     \includegraphics[width=0.24\textwidth]{figs/sk-large-effect.pdf}}
% % \subfigure[\textsf{CI} (small $k$)]{
% %     \includegraphics[width=0.24\textwidth]{figs/citeceer-small-effect.pdf}}
% % \subfigure[\textsf{CI} (large $k$)]{
% %     \includegraphics[width=0.24\textwidth]{figs/citeceer-large-effect.pdf}}
% % \subfigure[\textsf{ST} (small $k$)]{
% %     \includegraphics[width=0.24\textwidth]{figs/stanford-small-effect.pdf}}
% % \subfigure[\textsf{ST} (large $k$)]{
% %     \includegraphics[width=0.24\textwidth]{figs/stanford-large-effect.pdf}}
% % \subfigure[\textsf{DB} (small $k$)]{
% %     \includegraphics[width=0.24\textwidth]{figs/dblp-small-effect.pdf}}
% % \subfigure[\textsf{DB} (large $k$)]{
% %     \includegraphics[width=0.24\textwidth]{figs/dblp-large-effect.pdf}}
% % \subfigure[\textsf{DE} (small $k$)]{
% %     \includegraphics[width=0.24\textwidth]{figs/diel-small-effect.pdf}}
% % \subfigure[\textsf{DE} (large $k$)]{
% %     \includegraphics[width=0.24\textwidth]{figs/diel-large-effect.pdf}}
% % \subfigure[\textsf{DI} (small $k$)]{
% %     \includegraphics[width=0.24\textwidth]{figs/digg-small-effect.pdf}}
% % \subfigure[\textsf{DI} (large $k$)]{
% %     \includegraphics[width=0.24\textwidth]{figs/digg-large-effect.pdf}}
% % \subfigure[\textsf{SK} (small $k$)]{
% %     \includegraphics[width=0.24\textwidth]{figs/skitter-small-effect.pdf}}
% % \subfigure[\textsf{SK} (large $k$)]{
% %     \includegraphics[width=0.24\textwidth]{figs/skitter-large-effect.pdf}}
% % \subfigure[\textsf{OR} (small $k$)]{
% %     \includegraphics[width=0.24\textwidth]{figs/orkut-small-effect.pdf}}
% % \subfigure[\textsf{OR} (large $k$)]{
% %     \includegraphics[width=0.24\textwidth]{figs/orkut-large-effect.pdf}}
% % \caption{Comparison among variants on the large-$\omega$ graphs, varying $k$ from 3 to 8 and from $\omega-5$ to $\omega$.}
% % \label{fig:real-large-effect}
% % \end{figure*}



\noindent\textbf{Datasets.}
We use both real and synthetic datasets. 
%
The real datasets can be obtained from an open-source network repository \cite{rossi2015network}. For each graph, we follow existing studies \cite{deng2023accelerating, li2019fast} by ignoring directions, weights, and self-loops (if any). 
% Specifically, in some datasets, particularly social networks, self-loops are present due to user self-interactions, such as liking one's own posts. These self-loops were removed, as they do not contribute meaningful information to maximal clique identification and can lead to redundant computations. 
Our approach is naturally extendable to directed or weighted graphs. By first extracting all maximal cliques without considering direction or weight, we can subsequently filter the cliques to include only those that satisfy user-defined directional or weighted conditions.
% at the very beginning. 
We collect the graph statistics and report them in Table~\ref{tab:data}, where $\rho$ represents the edge density of a graph $G=(V,E)$ {\chengB (i.e., $\rho = |E|/|V|$)}, $\delta$ is the graph degeneracy and $\tau$ is the truss related number whose definition can be found in \cite{wang2024technical}. 
% {\Revise Due to the space limit, we provide the descriptions of the synthetic datasets and the corresponding results in the technical report~\cite{TR}.}
The synthetic datasets are generated based on two random graph generators, namely the Erd\"{o}s-R\'{e}yni (ER) graph model \cite{erdds1959random} and the Barab\'{a}si–Albert (BA) graph model \cite{albert2002statistical}. We provide the detailed descriptions of the synthetic datasets and the corresponding results in Appendix~\ref{app:syn}.
% Specifically, in the ER generator, the model first generates $n$ vertices and then randomly chooses $m$ edges between pairs of vertices. In the BA generator, the model adds the vertices to the network one at a time, and each new vertex is connected to a set number of existing vertices based on preferential attachment, i.e., vertices with a higher degree are more likely to receive new links.}
% By default, the number of vertices and edge density are set as  $n=1,000,000$ and $\rho=20$ (i.e., $m=n\rho$) for synthetic datasets, respectively. Due to the random nature of the graph generators, given a setting, we generate 10 graphs and report the mean of the results over these graphs. 
% {\kaixinkdd Due to the space limit, we present how we generate the synthetic datasets, and the corresponding settings and results in Appendix~\ref{sec:app-exp}, respectively.}
% The synthetic datasets are generated based on the Erd\"{o}s-R\'{e}yni (ER) graph model $G(n, m)$ \cite{erdds1959random}. Specifically, the model first generates $n$ vertices and then randomly chooses $m$ edges between pairs of vertices. By default, the number of vertices and edge density are set as  $n=1,000,000$ and $\rho=20$ (i.e., $m=n\rho$) for synthetic datasets, respectively. 





\begin{table*}
\vspace{-5mm}
    \begin{minipage}{.48\textwidth}
\scriptsize
    \centering
    \caption{Ablation studies and effects of different implementations of the hybrid frameworks (unit: second).}
    \vspace{-2mm}
    \label{tab:ablation}
    \begin{tabular}{c|rrr|rrr}
    \hline
      & \texttt{HBBMC++} & \texttt{HBBMC+} & \texttt{RDegen} & \texttt{Ref++} & \texttt{Rcd++} & \texttt{Fac++} \\ \hline
\textsf{NA} & \textbf{0.33} & 0.42 & 0.48 & 0.40 & \underline{0.38} & 0.42 \\
\textsf{FB} & \underline{1.10} & 1.40 & 1.67 & 1.17 & \textbf{0.99} & 1.20 \\
\textsf{WE} & \textbf{0.02} & 0.06 & 0.08 & \underline{0.04} & 0.05 & 0.06 \\
\textsf{WK} & \textbf{0.57} & 0.78 & 1.03 & 0.68 & \underline{0.63} & 0.94  \\
\textsf{SH} & \underline{0.45} & 0.88 & 0.98 & 0.48 & \textbf{0.43} & 0.53  \\
\textsf{ST} & \textbf{1.26} & \underline{1.45} & 1.70 & 1.60 & 1.49 & 3.74  \\
\textsf{DB} & \textbf{0.16} & 0.38 & 0.47 & \underline{0.18} & 0.20 & 0.29  \\
\textsf{DE} & \underline{3.82} & 5.53 & 7.47 & 4.23 & \textbf{3.53} & 5.07  \\
\textsf{DG} & \textbf{239.58} & 521.98 & 1046.40 & 426.28 & \underline{363.25} & 412.58  \\
\textsf{YO} & \textbf{1.47} & 1.92 & 2.32 & 1.80 & \underline{1.66} & 4.08 \\
\textsf{PO} & \textbf{19.31} & \underline{22.33} & 25.96 & 24.15 & 23.54 & 23.55 \\
\textsf{SK} & \textbf{25.15} & 40.81 & 47.11 &  34.85 & \underline{28.78} & 54.45 \\
\textsf{CN} & \textbf{6.03} & \underline{7.50} & 11.18 & 7.59 & 8.19 & 10.88 \\
\textsf{BA} & \textbf{13.81} & 18.73 & 22.61 & 17.51 & \underline{15.09} & 16.89          \\
\textsf{OR} & \textbf{884.20} & 1433.02 & 2200.54 & \underline{923.39} & 1162.74 & 1104.95 \\
\textsf{SO} & \textbf{21.12} & 32.16 & 39.61 & \underline{21.63} & 23.95 & 22.88 \\ \hline
    \end{tabular}
    \end{minipage}
    \hspace{8mm}
    \begin{minipage}{.48\textwidth}
\scriptsize
    \centering
    \caption{Effects of hybrid frameworks, varying the time changing from edge-oriented to vertex-oriented branching strategy.}
    \vspace{-2mm}
    \label{tab:hybrid}
\begin{tabular}{c|rr|rr|rr}
\hline
\multirow{2}{*}{} & \multicolumn{2}{c|}{$d=1$} & \multicolumn{2}{c|}{$d=2$} & \multicolumn{2}{c}{$d=3$}  \\\cline{2-7}
 & Time (s) & \#Calls  & Time (s) & \#Calls & Time (s) & \#Calls \\ \hline
\textsf{NA} & \textbf{0.33} & 365K & 0.99 & 1.57M & 4.99 & 13.3M  \\
\textsf{FB} & \textbf{1.10} & 2.15M & 1.46 & 3.47M & 2.45 & 6.82M \\
\textsf{WE} & \textbf{0.02} & 205K & 0.11 & 467K & 1.29 & 1.45M  \\
\textsf{WK} & \textbf{0.57} & 1.76M & 1.04 & 2.91M & 2.35 & 5.83M  \\
\textsf{SH} & \textbf{0.45} & 1.57M & 0.72 & 3.27M & 1.91 & 10.6M \\
\textsf{ST} & \textbf{1.26} & 1.69M & 1.83 & 3.56M & 11.12 & 14.7M \\
\textsf{DB} & \textbf{0.16} & 537K & 0.27 & 1.43M & 3.05 & 3.61M \\
\textsf{DE} & \textbf{3.82} & 1.29M & 33.28 & 17.4M & 313.02 & 279.1M  \\
\textsf{DG} & \textbf{239.58} & 1.54B & 583.76 & 1.89B & 798.05 & 2.07B  \\
\textsf{YO} & \textbf{1.47} & 3.97M & 1.58 & 6.25M & 1.75 & 8.24M  \\
\textsf{PO} & \textbf{19.31} & 27.9M & 21.48 & 39.0M & 25.48 & 65.1M \\
\textsf{SK} & \textbf{25.15} & 53.8M & 30.86 & 76.8M & 59.09 & 104.5M \\
\textsf{CN} & \textbf{6.03} & 16.6M & 13.57 & 24.9M & 16.57 & 39.8M \\
\textsf{BA} & \textbf{13.81} & 25.1M & 25.18 & 35.4M & 26.43 & 53.5M \\
\textsf{OR} & \textbf{884.20} & 5.58B & 1391.90 & 6.11B & 1829.41 & 6.70B \\
\textsf{SO} & \textbf{21.12} & 42.5M & 28.51 & 61.3M & 38.23 & 108.8M \\ \hline
\end{tabular}
\end{minipage}
\vspace{-5mm}
\end{table*}



\smallskip
\noindent\textbf{Baselines, Metrics and Settings.} 
%
We choose \texttt{HBBMC} as the default branching-based BB framework for comparison. Besides, we apply two techniques to enhance the performance of \texttt{HBBMC}. One is the early-termination technique (\texttt{ET} for short) as introduced in Section~\ref{sec:early-termination}. We set the the parameter $t=3$ by default {\chengB for the early-termination technique.}
% (i.e., early-termination from $t$-plexes). 
The other is the graph reduction technique (\texttt{GR} for short) proposed in \cite{deng2023accelerating}, which is to eliminate the branches that are created {\cheng based on} some small-degree vertices and report the maximal cliques that {\cheng involve} these vertices directly during the recursive procedure. Note that \texttt{GR} is also orthogonal to frameworks and can be easily adopted to our algorithm. We denote our algorithm with the above two techniques by \texttt{HBBMC++}. We compare our algorithm \texttt{HBBMC++} with four state-of-the-art algorithms proposed in \cite{deng2023accelerating}, namely \texttt{RRef} , \texttt{RDegen}, \texttt{RRcd} and \texttt{RFac} in terms of running time. Specifically, each of these four algorithms can be viewed as the original \texttt{VBBMC} algorithms, i.e., \texttt{BK\_Ref} \cite{naude2016refined}, \texttt{BK\_Degen} \cite{eppstein2010listing}, \texttt{BK\_Rcd} \cite{li2019fast}, \texttt{BK\_Fac} \cite{jin2022fast}, with {\cheng the} graph reduction technique. 
% (e.g., \texttt{RDegen} corresponds to the \texttt{BK\_Degen} algorithm with \texttt{GR}). 
The running time of all algorithms reported in our paper includes the time costs of (1) generating the orderings of vertices or edges (if any) and (2) enumerating maximal cliques via recursive procedures. The source codes of all algorithms are written in C++ and the experiments are conducted on a Linux machine with a 2.10GHz Intel CPU and 128GB memory. 
{\kaixinC The codes are available at \url{https://github.com/wangkaixin219/HBBMC}.}
% employs the edge-oriented branching-based BB framework with hybrid edge ordering, and applies the early-termination technique. 
% %
%  The running times of all algorithms reported in our paper include the time costs of (1) conducting the pre-processing techniques (if any) and (2) generating orderings of vertices. For our early termination technique, we set the parameter $t=2$ when $k\le \tau/2$ and $t=3$ when $\tau/2<k\le \omega$ for early-termination.}\marginpar{R4O1(7)}
% %
% All baselines are the state-of-the-art algorithms for $k$-cliques listing with vertex-oriented {\chengB branching-based} BB framework. 
% % consider two variants of \texttt{EBBkC} algorithm, namely \texttt{EBBkC+} and \texttt{EBBkC++}, where \texttt{EBBkC+} adopts both edge-oriented and vertex-oriented branching strategies as introduced in Section~\ref{subsec:EBBkC+}, and \texttt{EBBkC++} is the improved algorithm of \texttt{EBBkC+} with early-termination. Note that we choose the best possible $t$ (in $t$-plex) for early-termination. In addition, we also compare our algorithms
% % We compared our algorithm \texttt{RL-ETC}, which involves all techniques we propose in this paper, 
% % with four existing algorithms. namely \texttt{DDegCol} \cite{li2020ordering}, \texttt{DDegree} \cite{li2020ordering}, \texttt{SDegree} \cite{yuan2022efficient} and \texttt{BitCol} \cite{yuan2022efficient} in terms of running time. 
% %
% % All methods for comparison are implemented in C++. Note that for \texttt{DESCol}, we first implement and train it using Pytorch (Python 3.8). Then we use the model to generate the orderings of vertices. Finally, we list $k$-cliques in C++ using the above ordering to improve the efficiency. 
% % Since the early-termination technique can also be applied to all existing algorithms, we denote the corresponding algorithms with early-termination by \texttt{DDegCol++}, \texttt{DDegree++}, \texttt{SDegree++} and \texttt{BitCol++}, respectively. 
% {\kaixin Following the existing study \cite{li2020ordering}, we vary $k$ from 4 since $k$-clique listing problem reduces to triangle listing problem when $k=3$ and there are efficient algorithms \cite{latapy2008main,ortmann2014triangle} for triangle listing which run in polynomial time.}
% % {\yuiR
% % We measure all algorithms by reporting the running times that include the time costs of (1) conducting the pre-processing (if possible), (2) generating orderings and (3) listing $k$-cliques via BB. 
% % }

% %For a fair comparison, we only collect the time of listing $k$-clique {\kaixinB (including generating vertex/edge orderings)} and omit the time of reading the graph from the disk. 

% % Besides, we generate the possible orderings (of vertices or edges) in advance for all algorithms. 
% %
% % In addition, all existing methods can also exploit our truss decomposition index process to prune some unpromising search paths. Therefore, we run all algorithms on the pruned graphs for fairness. 
% %



% \begin{table}[t]
%     \centering
%     \caption{Effects of different hybrid frameworks.}
%     \label{tab:frame}
%     \begin{tabular}{c|C{1cm}C{1cm}C{1cm}C{1cm}C{1cm}}
%     \hline
%   (\texttt{+ETGR}) & \texttt{HBBMC} & \texttt{EBBMC} & \texttt{HRef} & \texttt{HRcd} & \texttt{HFac} \\ \hline
% \textsf{NA} &       &       &      &      &      \\
% \textsf{FB} &       &       &      &      &      \\
% \textsf{WE} &       &       &      &      &      \\
% \textsf{WK} &       &       &      &      &      \\
% \textsf{SH} &       &       &      &      &      \\
% \textsf{ST} &       &       &      &      &      \\
% \textsf{DB} &       &       &      &      &      \\
% \textsf{DE} &       &       &      &      &      \\
% \textsf{DG} &       &       &      &      &      \\
% \textsf{YO} &       &       &      &      &      \\
% \textsf{PO} &       &       &      &      &      \\
% \textsf{SK} &       &       &      &      &      \\
% \textsf{CN} &       &       &      &      &      \\
% \textsf{BA} &       &       &      &      &      \\
% \textsf{OR} &       &       &      &      &      \\
% \textsf{SO} &       &       &      &      &     \\ \hline
%     \end{tabular}
% \end{table}





% \smallskip\noindent
% \textbf{Settings.}
% The source codes of all algorithms are written in C++ and the experiments are conducted on a Linux machine with a 2.10GHz Intel CPU and 128GB memory. 
% % We note that we do not use SIMD instructions for data-level parallelism in our implementation although it can further accelerate our algorithm. 
% {\cheng We note that we have not utilized SIMD instructions for data-level parallelism in our implementation, despite the potential to further enhance the acceleration of our algorithm.}
% We set the time limit as 3 hours (i.e., 10,800 seconds) and the running time of any algorithm that exceeds the time limit is recorded with ``{-}''. 
% For the experiments on synthetic datasets, due to the random nature of the graph generator (i.e., Erd\"{o}s-R\'{e}yni (ER) graph model), given a setting, we generate 10 graphs and report the mean of the results over these graphs.
% Implementation codes and datasets can be found via this link \url{https://anonymous.4open.science/r/HBBMC}. 
% ***. 


% We consider three instances of \texttt{DESCol}, which adopt different color orderings (line 15 of Algorithm~\ref{alg:clique}). The first one uses the learned ordering via reinforcement learning, which we denote by \texttt{DESCol-L}. The second one uses the inverse degree ordering \cite{yuan2017effective}, which we denote by \texttt{DESCol-D}. The third one uses the inverse degeneracy ordering \cite{hasenplaugh2014ordering}, which we denote by \texttt{DESCol-G}. Besides, we also compare our algorithm with three existing algorithms, namely \texttt{DDegCol} \cite{li2020ordering} and \texttt{DDegree} \cite{li2020ordering} and \texttt{BitCol} \cite{yuan2022efficient} in terms of running time. 






% \smallskip\noindent
% \textbf{Hyperparameter Setting and Policy Learning.}
% There are two neural networks in \texttt{DESCol} method. The actor network $\mu(\cdot|s; \theta)$ involves one input layer, one hidden layer and one output layer, where the hidden layer involves 32 neurons and uses tanh function as the activation function. 
% %
% The critic network $V(s; \omega)$ involves one input layer, one hidden layer and one output layer, where the hidden layer involves 32 neurons and uses tanh as the activation function. 
% %
% The output layer involves $K$ neurons and $K$ is set as 10 by default. 
% %
% For the training, we generate the training data, validation data and testing data as follows. For each graph, we first generate a DAG $\overrightarrow{G}$ by degeneracy ordering, and decompose the graph $\overrightarrow{G}$ into $n$ subgraphs, which are induced by $N_u^+(\overrightarrow{G})$ for all $u\in \overrightarrow{G}$. Then we choose 40\% and 20\% of these $n$ subgraphs as training data and validation data, respectively. Finally, we test the model by applying it to the whole graph. 
% %
% It is a straight forward idea to train a model for each $k\in[3,\omega]$ with which we can find optimal orderings for every $k$. However, it would take a long time to train the model when $k$ increases, and it doesn't robust. Therefore, we choose $k=5$ to train the model based on the empirical results. 
% %
% For the reward coefficient parameters, we set $\beta_{col}=\beta_{deg}=1$. For the reward discount $\gamma$, we set it as 0.99. We train the networks for 500 epochs, using the Adam stochastic gradient descent with the learning rate of 0.001. For other parameters involved in PPO policy learning process, we set them as the default values provided in \cite{schulman2017proximal}. 


% \if 0
% \begin{figure*}[ht]
% \subfigure[$n=250,000$]{
%     \includegraphics[width=0.24\textwidth]{figs/synn25.pdf}}
% \subfigure[$n=500,000$ (default)]{
%     \includegraphics[width=0.24\textwidth]{figs/synn50.pdf}}
% \subfigure[$n=750,000$]{
%     \includegraphics[width=0.24\textwidth]{figs/synn75.pdf}}
% \subfigure[$n=1,000,000$]{
%     \includegraphics[width=0.24\textwidth]{figs/synn100.pdf}}
% \caption{Results on varying $n$ (synthetic dataset).}
% \label{fig:vary-n}
% \end{figure*}


% \begin{figure*}[ht]
% \subfigure[$p=0.37$]{
%     \includegraphics[width=0.24\textwidth]{figs/synp37.pdf}}
% \subfigure[$p=0.40$ (default)]{
%     \includegraphics[width=0.24\textwidth]{figs/synp40.pdf}}
% \subfigure[$p=0.43$]{
%     \includegraphics[width=0.24\textwidth]{figs/synp43.pdf}}
% \subfigure[$p=0.45$]{
%     \includegraphics[width=0.24\textwidth]{figs/synp45.pdf}}
% \caption{Results on varying $p$ (synthetic dataset).}
% \label{fig:vary-p}
% \end{figure*}
% \fi

% \begin{figure*}[ht]
% \subfigure[\textsf{sc-nasasrb}]{
%     \includegraphics[width=0.24\textwidth]{figs/empty.png}}
% \subfigure[\textsf{com-youtube}]{
%     \includegraphics[width=0.24\textwidth]{figs/empty.png}}
% \subfigure[\textsf{web-baiduBK}]{
%     \includegraphics[width=0.24\textwidth]{figs/empty.png}}
% \subfigure[\textsf{soc-facebook}]{
%     \includegraphics[width=0.24\textwidth]{figs/empty.png}}
% \caption{Results on varying $K$.}
% \label{fig:vary-k-small-phi}
% \end{figure*}
















\subsection{Experimental Results on Real Datasets}
\label{subsec:real-result}


\noindent
\textbf{(1) Comparison among algorithms.}
Table~\ref{tab:real} shows the results of the running time of different algorithms for maximal clique enumeration on all datasets. We observe that our algorithm \texttt{HBBMC++} runs faster than all baselines on all datasets. For most of the datasets that satisfy the condition $\delta \ge \tau+\frac{3}{\ln 3}\ln\rho$, the results are consistent with our theoretical analysis that the time complexity of \texttt{HBBMC++} is better than those of the baseline algorithms. For example, on \textsf{DG}, \textsf{CN} and \textsf{OR}, the values of $\tau$ are far smaller than the values of $\delta$. As a result, \texttt{HBBMC++} can run up to 4.38x faster than the state-of-the-art algorithms. For the others (e.g., \textsf{WE} and \textsf{DB}), the speedups are also significant, i.e., \texttt{HBBMC++} achieves 4.0x and 2.94x speedups on \textsf{WE} and \textsf{DB}, respectively. There are two possible reasons. First, while the \texttt{HBBMC} would {\chengB produce} more branches than the \texttt{VBBMC} algorithms from the initial branch (i.e., $m$ branches v.s. $n$ branches), the sizes of the branches are typically much smaller, which rarely reaches the worst case. Second, the early-termination technique \texttt{ET} also {\cheng helps} quickly enumerate those maximal cliques in a dense subgraph instead of making branches for the search space, which dramatically reduces the running time.
\texttt{RRcd} and \texttt{RDegen} also perform well in practice. Both are BK branching-based algorithms, where the former follows \texttt{BK\_Rcd} framework while the latter follows \texttt{BK\_Degen} framework. The main difference between \texttt{BK\_Rcd} and \texttt{BK\_Degen} is that \texttt{BK\_Rcd} adopts a \emph{top-to-down} approach that starts from a subgraph and iteratively removes vertices from the subgraph until the subgraph becomes a clique, while \texttt{BK\_Degen}, in essence, adopts a \emph{bottom-to-up} approach that starts from an individual vertex, adds only one vertex into the result set with one independent recursive call, and discovers a maximal clique utill all its vertices are added into the result set. When $g_C$ is already a clique or a near-clique (e.g., a clique with only a few edges missing), \texttt{BK\_Rcd} would create less branches than that of \texttt{BK\_Degen}. This would help explain why \texttt{BK\_Rcd} sometimes performs better than \texttt{BK\_Degen} in practice. 


% {\Revise \texttt{RRcd} and \texttt{RDegen} \marginnote{R1O4} also perform very well in practice. \texttt{RRcd} follows \texttt{BK\_Rcd} \cite{li2019fast} framework, which adopts the Bron-Kerbosch (BK) branching and creates the branches via Eq.~(\ref{eq:vbb-branching}). The main difference between \texttt{BK\_Rcd} and other BK branching based algorithms (e.g., \texttt{BK\_Degen}) is that \texttt{BK\_Rcd} does not equip pivoting strategy to prune unpromising branches during the recursive process. Specficically, given a branch $B=(S,g_C,g_X)$, it repeatedly conducts branching at the vertex with the smallest degree in $g_C$ until $g_C$ becomes a clique. Due to the lack of pivoting strategy, \texttt{BK\_Rcd} would produce $O(2^n)$ branches at the worst case if $g_C$ contains $n$ vertices inside, which makes \texttt{BK\_Rcd} have worse theoretical result than that of \texttt{BK\_Degen}. However, real-world graphs are usually globally sparse but locally dense. When $g_C$ is already a near-clique, \texttt{BK\_Rcd} would create much less branches than that of \texttt{BK\_Degen}. This would help explain why \texttt{BK\_Rcd} performs very well in practice. 
% }

\smallskip\noindent
\textbf{(2) Ablation studies.}
We compare two variants of our methods, namely \texttt{HBBMC++} (the full version) and \texttt{HBBMC+} (the full version without the early-termination \texttt{ET}), with the state-of-the-art \texttt{VBBMC} algorithm \texttt{RDegen}. 
We note that it is not fair to compare \texttt{HBBMC} with other \texttt{VBBMC} algorithm (e.g., \texttt{RRcd}) since the former applies the classic pivot selection introduced in \cite{tomita2006worst} while the latter does not. 
% We note that while \texttt{RDegen} and \texttt{RFac} do not have the best theorectical results compared to the other two \texttt{VBBMC} algorithms, their practical performance is much better (see details in Figure~\ref{fig:real}, \cite{li2019fast} and \cite{jin2022fast}). 
We report the results in the columns 1-3 of Table~\ref{tab:ablation} and have the following observations. 
\underline{First}, \texttt{HBBMC+} runs consistently and clearly faster than \texttt{RDegen}, which demonstrates the contribution of the hybrid frameworks of \texttt{HBBMC} since \texttt{HBBMC+} and \texttt{RDegen} only differ in their frameworks (note that the graph reduction technique \texttt{GR} is employed in \texttt{RDegen}). 
\underline{Second}, \texttt{HBBMC++} runs faster than \texttt{HBBMC+}, which demonstrates the contribution of the early-termination technique \texttt{ET}. 
%
For example, on \textsf{OR}, the hybrid framework and early-termination technique contribute 41.7\% and 58.3\% to the efficiency improvements over \texttt{RDegen}, respectively. 


% \smallskip\noindent
% \textbf{(3) Comparison between \texttt{HBBMC-T} and \texttt{HBBMC-P} (real datasets).}





















\begin{table*}[t]
\vspace{-5mm}
% \footnotesize
    \centering
    \caption{Effects of early-termination technique, where ``Ratio'' is the ratio between the number of branches that can be early-terminated (i.e., $g_C$ is $t$-plex and $g_X$ is an empty graph) and the number of all branches where the condition that $g_C$ is a $t$-plex is satisfied.}
    \vspace{-2mm}
    \label{tab:early}
\begin{tabular}{c|R{1.1cm}R{1.1cm}|R{1.1cm}R{1.1cm}R{1.1cm}|R{1.1cm}R{1.1cm}R{1.1cm}|R{1.1cm}R{1.1cm}R{1.1cm}}
\hline
\multirow{2}{*}{} & \multicolumn{2}{c|}{$t=0$} & \multicolumn{3}{c|}{$t=1$} & \multicolumn{3}{c|}{$t=2$} & \multicolumn{3}{c}{$t=3$} \\\cline{2-12}
 & Time (s) & \#Calls  & Time (s) & \#Calls & Ratio & Time (s) & \#Calls & Ratio & Time (s) & \#Calls & Ratio \\ \hline
\textsf{NA} & 0.42 & 552K & 0.38 & 374K & 19.47\% & {0.34} & 366K & 19.83\% & {0.33} & 365K & 19.72\% \\
\textsf{FB} & 1.40 & 4.08M & 1.33 & 3.45M & 75.47\% & {1.25} & 2.77M & 74.90\% & {1.10} & 2.15M & 65.92\% \\
\textsf{WE} & 0.06 & 321K & 0.04 & 217K & 59.14\% & {0.03} & 206K & 59.23\% & {0.02} & 205K & 57.39\% \\
\textsf{WK} & 0.78 & 3.36M & 0.64 & 2.76M & 84.72\% & {0.60} & 2.20M & 83.06\% & {0.57} & 1.76M & 76.35\% \\
\textsf{SH} & 0.88 & 2.31M & 0.66 & 1.72M & 53.98\% & {0.52} & 1.66M & 52.91\% & {0.45} & 1.57M & 49.47\% \\
\textsf{ST} & 1.45 & 2.61M & 1.36 & 1.99M & 64.94\% & {1.29} & 1.76M & 60.98\% & {1.26} & 1.69M & 57.17\% \\
\textsf{DB} & 0.38 & 993K & 0.29 & 571K & 57.71\% & {0.22} & 550K & 55.92\% & {0.16} & 537K & 52.47\% \\
\textsf{DE} & 5.53 & 2.26M & 4.94 & 1.30M & 4.23\% & {4.02} & 1.29M & 4.63\% & {3.82} & 1.29M & 4.63\% \\
\textsf{DG} & 521.98 & 2.36B & 419.62 & 2.06B & 73.76\% & {347.80} & 1.78B & 71.38\% & {239.58} & 1.54B & 64.50\% \\
\textsf{YO} & 1.92 & 6.30M & 1.74 & 5.00M & 82.16\% & {1.57} & 4.37M & 78.91\% & {1.47} & 3.97M  & 74.79\% \\
\textsf{PO} & 22.33 & 38.6M & 21.20 & 33.4M & 63.58\% & {20.03} & 30.2M & 61.97\% & {19.31} & 27.9M & 57.25\% \\
\textsf{SK} & 40.81 & 102M & 35.83 & 82.3M & 82.65\% & {30.45} & 69.1M & 83.11\% & {25.15} & 53.8M & 77.81\% \\
\textsf{CN} & 7.50 & 25.1M & 6.86 & 20.6M & 78.74\% & {6.57} & 18.2M & 76.07\% & {6.03} & 16.6M & 71.92\% \\
\textsf{BA} & 18.73 & 36.4M & 15.49 & 31.1M & 73.33\% & {14.39} & 27.6M & 71.19\% & {13.81} & 25.1M & 66.88\% \\
\textsf{OR} & 1433.02 & 8.99B & 1034.83 & 7.73B & 69.29\% & {966.22} & 6.78B & 67.12\% & {884.20} & 5.58B & 62.90\%\\
\textsf{SO} & 32.16 & 63.9M & 26.03 & 53.2M & 71.11\% & {18.22} & 47.0M & 68.45\% & {21.12} & 42.5M & 62.69\% \\ \hline
\end{tabular}
\vspace{-4mm}
\end{table*}







\begin{table}[t]
\vspace{-2mm}
\scriptsize
    \centering
    \caption{Effects of truss-based edge ordering \\(unit: second).}
\vspace{-2mm}
    \label{tab:revise1}
    \begin{tabular}{c|rrrrr}
    \hline
    & \texttt{HBBMC++} & \texttt{VBBMC-dgn} & \texttt{HBBMC-dgn} & \texttt{HBBMC-mdg} \\ \hline
\textsf{NA} & \textbf{0.33}     & 0.44 & 0.45 & \underline{0.37}   \\
\textsf{FB} & \textbf{1.10}     & 1.42 & 1.43 & \underline{1.26}   \\
\textsf{WE} & \textbf{0.02}     & \underline{0.04} & 0.04 & 0.05   \\
\textsf{WK} & \textbf{0.57}     & 0.76 & 0.77 & \underline{0.73}   \\
\textsf{SH} & \textbf{0.45}     & 0.66 & 0.68 & \underline{0.55}   \\
\textsf{ST} & \textbf{1.26}     & 1.81 & 1.89 & \underline{1.57}   \\
\textsf{DB} & \textbf{0.16}     & 0.27 & 0.28 & \underline{0.23}   \\
\textsf{DE} & \textbf{3.82}     & 6.81 & 6.96 & \underline{5.13}   \\ 
\textsf{DG} & \textbf{239.58}   & 594.27 & 596.55 & \underline{486.02}   \\
\textsf{YO} & \textbf{1.47}     & \underline{2.42} & 2.51 & 2.53   \\
\textsf{PO} & \textbf{19.31}    & 25.99 & 26.58 & \underline{20.64}   \\
\textsf{SK} & \textbf{25.15}    & 37.58 & 38.71 & \underline{32.30}   \\
\textsf{CN} & \textbf{6.03}     & 11.91 & 12.36 & \underline{7.83}  \\
\textsf{BA} & \textbf{13.81}    & 16.78 & 17.19 & \underline{16.58}  \\
\textsf{OR} & \textbf{884.20}   & 1505.95 & 1550.6 & \underline{1204.22}   \\
\textsf{SO} & \textbf{21.12}    & 36.03 & 37.33 & \underline{27.66}  \\
\hline
    \end{tabular}
\vspace{-4mm}
\end{table}






\smallskip\noindent
\textbf{(3) Effects of hybrid frameworks (varying vertex-oriented branching framework).}
Recall that in Section~\ref{subsec:HBBMC}, there are several combinations of \texttt{EBBMC} and \texttt{VBBMC} to implement the hybrid framework (i.e., using different \texttt{VBBMC} frameworks). Therefore, we first study the effect of these combinations by making comparison among these implementations. We denote the algorithms for comparison by \texttt{HBBMC++} (the full version), \texttt{Ref++}, \texttt{Rcd++} and \texttt{Fac++}. We note that each of the last three algorithms corresponds to an enumeration procedure in which {\cheng we} (1) use the edge-oriented BB framework with truss-based edge ordering {\cheng for the partitioning at} the initial branch, (2) use the corresponding \texttt{VBBMC} algorithm (e.g., \texttt{BK\_Ref}, \texttt{BK\_Rcd} or \texttt{BK\_Fac}) to produce the remaining branches and (3) use \texttt{ET} (with $t=3$) and \texttt{GR} to boost the performance. We report the results in columns 4-6 of Table~\ref{tab:ablation}. Compared among the algorithms with different \texttt{VBBMC} frameworks,  \texttt{HBBMC++} runs the fastest on the majority of the datasets. While \texttt{Rcd++} runs faster on some datasets (e.g., \textsf{FB}, \textsf{SH} and \textsf{DE}), the differences are marginal. 



\smallskip\noindent
\textbf{(4) Effects of hybrid frameworks (varying the time when \texttt{HBBMC++} changes from edge-oriented to vertex-oriented branching strategy).}
We also explore alternative hybrid strategies by investigating the use of the edge-oriented branching strategy at varying depths within the recursion tree. Specifically, we applied the edge-oriented branching strategy at the early stages of the tree, up to a depth threshold $d\ge 1$, beyond which we switched to the pivot-based vertex-oriented branching strategy. By varying $d$ within the range $d\in\{1,2,3\}$, we aimed to identify the optimal balance between the effectiveness of edge-oriented branching and the more granular control provided by vertex-oriented branching at deeper levels. We note that the case $d=1$ corresponds to the branching strategy employed in \texttt{HBBMC++}.
Table \ref{tab:hybrid} shows that increasing $d$ typically results in more branching calls and longer runtimes, due to the lack of pivot-based pruning in edge-oriented branching. However, edge-oriented branching is still effective for rapid pruning at the initial stages, and adjusting $d$ allows us to fine-tune when to leverage the strengths of each strategy. The results suggest that carefully choosing the threshold $d$ (i.e., $d=1$) is crucial for optimizing the performance of the hybrid framework, ensuring that the transition between branching strategies is both timely and effective.


\smallskip\noindent
\textbf{(5) Effects of early-termination technique.}
We study the effects by choosing different parameter $t$ (in $t$-plex) for early-termination. We vary $t$ in the range $\{0, 1, 2, 3\}$ and report the corresponding running time of \texttt{HBBMC++} under different values of $t$. We note that when $t=0$, \texttt{HBBMC++} is equivalent to \texttt{HBBMC+} (the full version without early-termination technique). The results are shown in Table~\ref{tab:early}. We observe that the running time of \texttt{HBBMC++} decreases as the value of $t$ increases. The reason is that 
% while we can list all maximal cliques inside a $t$-plex in optimal time when $t=1, 2, 3$, 
we can early-terminate the recursion in an earlier phase when $t$ has a larger value as $t$-plex must be a $t'$-plex if $t<t'$ but not vice versa. We collect the statistics of the number of recursive function calls of \textsf{VBBMC\_Rec} in \texttt{HBBMC}, showing that the numbers drop steadily from $t=0$ to $t=3$, which explains the contribution of the efficiency improvement with different values of $t$. 
%
Besides, there is another factor that affects the power of the early-termination. That is the ratio between the number of branches that can be early-terminated (i.e., $g_C$ is $t$-plex and $g_X$ is an empty graph), which we denote by $b_0$, {\cheng and} the number of all branches where the condition that $g_C$ is a $t$-plex is satisfied, which we denote by $b$. The closer the ratio is to 1, the more potent the early-termination becomes. We also report this ratio in Table~\ref{tab:early}. We have the following observations. First, the ratio is over 60\% with different settings of $t$ on most of datasets, which indicates that the early-termination truly helps \texttt{HBBMC} accelerate the enumeration in such dense subgraphs. For the datasets such as \textsf{NA} and \textsf{DE} in which the ratio is relatively small, the possible reason is that these two graphs are dense (i.e., $\rho > 20$) but have too few maximal cliques inside (i.e., there are only 28,154 and 24,012 maximal cliques in \textsf{NA} and \textsf{DE}, respectively). As a result, the value of $b$ is much larger than $b_0$ on these two graphs. Second, it shows a trend that the ratio decreases as the value of $t$ increases. We collect the values of $b_0$ and $b$ and find that while $b_0$ and $b$ both increase as $t$ increases, the increase rate of $b$ is larger than that of $b_0$. The possible reason is that the requirement that $g_C$ is $t$-plex is much easier to be satisfied as the value of $t$ increases but $g_X$ is not always an empty graph. 



% \begin{table}[t]
%     \centering
%     \caption{Effects of early-termination technique (varying $t$).}
%     \label{tab:early}
%     \begin{tabular}{c|C{1.2cm}C{1.2cm}C{1.2cm}C{1.2cm}}
%     \hline
%    & $t=0$ & $t=1$ & $t=2$ & $t=3$  \\ \hline
% \textsf{NA} & 0.42 & 0.38 & \underline{0.34} & \textbf{0.33} \\
% \textsf{FB} & 1.40 & 1.33 & \underline{1.25} & \textbf{1.10} \\
% \textsf{WE} & 0.06 & 0.04 & \underline{0.03} & \textbf{0.02} \\
% \textsf{WK} & 0.78 & 0.64 & \underline{0.60} & \textbf{0.57} \\
% \textsf{SH} & 0.88 & 0.66 & \underline{0.52} & \textbf{0.45} \\
% \textsf{ST} & 1.45 & 1.36 & \underline{1.29} & \textbf{1.26} \\
% \textsf{DB} & 0.38 & 0.29 & \underline{0.22} & \textbf{0.16} \\
% \textsf{DE} & 5.53 & 4.94 & \underline{4.42} & \textbf{3.82} \\
% \textsf{DG} & 521.98 & 419.62 & \underline{347.80} & \textbf{239.58} \\
% \textsf{YO} & 1.92 & 1.74 & \underline{1.57} & \textbf{1.47} \\
% \textsf{PO} & 22.33 & 21.20 & \underline{20.03} & \textbf{19.31} \\
% \textsf{SK} & 40.81 & 35.83 & \underline{30.45} & \textbf{25.15} \\
% \textsf{CN} & 7.50 & 6.86 & \underline{6.57} & \textbf{6.03} \\
% \textsf{BA} & 18.73 & 15.49 & \underline{14.39} & \textbf{13.81} \\
% \textsf{OR} & 1433.02 & 1034.83 & \underline{966.22} & \textbf{884.20} \\
% \textsf{SO} & 32.16 & 26.03 & \underline{18.22} & \textbf{21.12} \\ \hline
%     \end{tabular}
% \end{table}






\smallskip\noindent
\textbf{(6) Effects of truss-based edge ordering.}
We compare the performance of \texttt{HBBMC++} with three new baselines that only differ in their branching strategies for the initial branch. \texttt{VBBMC-dgn} uses a vertex-oriented branching strategy based on degeneracy ordering. \texttt{HBBMC-dgn} adopts an edge-oriented branching strategy where edges are ordered alphabetically based on the degeneracy ordering of their endpoints. \texttt{HBBMC-mdg} also uses an edge-oriented branching strategy, but the edge ordering is based on a non-decreasing order of an upper bound derived from the minimum degree of their endpoints.
The results are shown in Table~\ref{tab:revise1}. We have the following observations. \underline{First}, \texttt{HBBMC++} (with the proposed hybrid branching) outperforms \texttt{VBBMC-dgn} (with the existing vertex-oriented branching) across all datasets, with significant improvements particularly on larger datasets. This demonstrates the superiority of the porposed hybrid branching, particularly the edge-oriented branching, and is well aligned with the theoritical results in Theorem~\ref{theo:hbbmc}. \underline{Second}, \texttt{HBBMC++} consistently outperforms both \texttt{HBBMC-dgn} and \texttt{HBBMC-mdg}, which verifies the effectiveness of truss-based edge ordering towards reducing computational overhead. We remark that, without adopting the truss-based edge ordering, \texttt{HBBMC-dgn} and \texttt{HBBMC-mdg} cannot acheive the same time complexity as \texttt{HBBMC++} does.
% Compare \texttt{HBBMC++} with \texttt{VBBMC-dgn}. \texttt{HBBMC++} consistently achieves better performance due to the use of truss-based edge ordering, which is obtained through a greedy procedure that iteratively removes the edge whose vertices have the smallest number of common neighbors. It effectively reduces the size of intermediate graph instances due to the fact $\tau < \delta$, thereby decreasing the search space and computation time. The results show that \texttt{HBBMC++} outperforms \texttt{VBBMC-dgn} across all datasets, with significant improvements particularly on larger datasets.
% %
% Compare \texttt{HBBMC++} with \texttt{HBBMC-dgn} and \texttt{HBBMC-mdg}, they all use the edge-oriented branching strategy but differ in what edge ordering is applied. The results demonstrate that \texttt{HBBMC++} consistently outperforms both \texttt{HBBMC-dgn} and \texttt{HBBMC-mdg}, illustrating the efficiency of truss-based edge ordering in reducing computational overhead.



% \subsection{Experimental Results on Synthetic Datasets}
% \label{subsec:syn-result}




% % \smallskip\noindent
% % \textbf{(5) Scalability test (varying $n$, synthetic datasets).}
% First, we vary the number of vertices in the range $n\in\{100\text{K}, 500\text{K}, 1\text{M}, 5\text{M}, 10\text{M}\}$ and set $\rho=20$ {\cheng by} default. {\Revise The results for the graphs generated using the ER model and the BA model are presented in Figure~\ref{fig:scale-er} and Figure~\ref{fig:scale-ba}, respectively. Under all settings, \texttt{HBBMC++} consistently outperforms all baselines, achieving remarkable speedups compared to the second-best algorithm \texttt{RRcd}, with average speedups of 1.84x and 1.94x (up to 2.84x and 2.26x) on the graphs generated by the ER and BA models, respectively.
% %
% \marginnote{R1O3}
% % 1.84x speedups on average (up to ) over the second best algorithm \texttt{RRcd}. 
% Additionally, we report the degeneracy number $\delta$ and the truss-related number $\tau$ under different settings. In the graphs generated by the ER model, these values are $\delta=\{8, 14, 28, 43, 58\}$ and $\tau=\{0, 1, 3, 5, 7\}$ for different values of $n$. In contrast, for the graphs generated by the BA model, the values remain approximately $\delta\approx 42$ and $\tau\approx 25$ across all $n$. 
% %
% This interesting phenomenon can be explained by the distinct mechanisms of edge formation in the two models. In the ER model, edges are uniformly distributed, which facilitates the formation of larger  $k$-cores as the number of vertices $n$ increases, leading to an increase in degeneracy. Conversely, in the BA model, the preferential attachment mechanism concentrates edges around a few high-degree hubs, stabilizing the graph’s core structure and maintaining a nearly constant degeneracy, irrespective of the growth in $n$.}
% %
% Finally, we note that all above results are well aligned with our theoretical analysis, i.e., the worst-case time complexity of \texttt{HBBMC++} is better than that of our algorithms when $\delta\ge \tau +\frac{3}{\ln 3}\ln \rho$. 




% \begin{figure}[t]
% \centering
% \subfigure[Scalability test (ER model).]{
% \label{fig:scale-er}
% \includegraphics[width=0.23\textwidth]{figs/exp/scale-er.pdf}}
% \subfigure[Scalability test (BA model).]{
% \label{fig:scale-ba}
% \includegraphics[width=0.23\textwidth]{figs/exp/scale-ba.pdf}}
% \subfigure[Results on varying $\rho$ (ER model).]{
% \label{fig:density-er}
% \includegraphics[width=0.23\textwidth]{figs/exp/density-er.pdf}}
% \subfigure[Results on varying $\rho$ (BA model).]{
% \label{fig:density-ba}
% \includegraphics[width=0.23\textwidth]{figs/exp/density-ba.pdf}}
% \caption{ Results on synthetic datasets. }
% \vspace{-5mm}
% \end{figure}


% % \smallskip\noindent
% % \textbf{(6) Effects of edge density (varying $\rho$, synthetic datasets).}
% Second, we vary the edge density in the range $\rho\in\{5,10,20,30,40\}$ and set $n=1\text{M}$ {\cheng by} default. {\Revise The results for the graphs generated using the ER and BA models are presented in Figure~\ref{fig:density-er} and Figure~\ref{fig:density-ba}, respectively. 
% %
% \marginnote{R1O3}
% %
% On average, \texttt{HBBMC++} achieves speedups of 1.65x and 1.88x (with maximum speedups of 1.89x and 3.17x) on the graphs generated by the ER and BA models, respectively, compared to the second-best algorithm \texttt{RRcd}.} We also observe that the speedup decreases as the graph $\rho$ increases. The possible reason is that when $\rho$ increases, the graph becomes denser. Therefore, the differences between $\delta$ and $\tau$ becomes {\cheng narrower}. 




% {\Revise \marginnote{R1O3}
% Notably, we observe that when comparing the results under identical parameter settings but using the ER model, the computation time is longer for graphs generated by the BA model. The possible reason is that the graphs following a power-law distribution typically contain larger sizes of maximal cliques. For example, under the default setting (i.e., $n=1\text{M}$ and $\rho=20$), the largest clique in the ER graph is a 5-clique, while for the BA graph, this value is a 28-clique.}


==> 6._related.tex <==

% \clearpage

\section{Related Work}
\label{sec:related}

% \smallskip\noindent
% \textbf{Maximal Clique Enumeration in a Serial Processing Setting.}
%
Sequential algorithms for maximal clique enumeration (MCE) problem 
% under serial processing setting 
can be classified into two categories: branch-and-bound based algorithms \cite{bron1973algorithm, tomita2006worst, eppstein2010listing, eppstein2013listing, li2019fast, naude2016refined} and reverse-search based algorithms \cite{johnson1988generating, chang2013fast, conte2016sublinear, tsukiyama1977new, chiba1985arboricity, makino2004new, comin2018improved}. 
%
% {\chengB \underline{For the former}}, 
{\chengc For the former,}
% branch-and-bound based algorithms,
Bron-Kerbosch (\texttt{BK}) algorithm \cite{bron1973algorithm} is the first practical algorithm for MCE, in which each branch is represented by three vertex sets $S$, $C$ and $X$ ({\cheng correspondingly,} $g_C=G[C]$ and $g_X=G[X]$ are the candidate and {\kaixin exclusion}
% forbidden 
subgraphs,
% as introduced in Section~\ref{sec:BBMC}, 
respectively). \texttt{BK\_Pivot} \cite{tomita2006worst} improves \texttt{BK} {\cheng with} the pivoting strategy, which selects a vertex $u\in C\cup X$ that maximizes $|N(u,G)\cap C|$ as the pivot in each branch. It has been {\cheng proved} that the worst-case time complexity of \texttt{BK\_Pivot} is $O(n\cdot 3^{n/3})$, which is worst-case optimal since the Moon-Moser graph \cite{moon1965cliques} truly has $3^{n/3}$ maximal cliques inside. \texttt{BK\_Ref} \cite{naude2016refined} refines and accelerates \texttt{BK\_Pivot} by considering some special cases during the pivot selection {\cheng process} but retains the same worst-case time complexity as that of \texttt{BK\_Pivot}. Recently, different vertex orderings are adopted to improve \texttt{BK\_Pivot} on sparse graphs. Specifically, \texttt{BK\_Degen} \cite{eppstein2010listing, eppstein2013listing} uses the degeneracy ordering {\cheng for the branching at the initial branch} $B=(\emptyset, G, G[\emptyset])$ such that for each produced sub-branch, there are at most $\delta$ vertices in the candidate subgraph $g_C$, where $\delta$ is the degeneracy of the graph, and correspondingly, the worst-case time complexity improves to $O(n\delta\cdot 3^{\delta/3})$. Similarly, \texttt{BK\_Degree} \cite{xu2014distributed} uses the degree ordering to branch the initial search space. In this case, there are at most $h$ vertices in the candidate subgraph $g_C$, where $h$ is the $h$-index of graph, and the worst-case time complexity is $O(nh\cdot 3^{h/3})$. \texttt{BK\_Rcd} \cite{li2019fast} extends \texttt{BK\_Degen} {\cheng with} a top-to-down approach, {\chengB which} repeatedly conducts branching at the vertex with the smallest degree in $g_C$ until $g_C$ {\cheng becomes} a clique. \texttt{BK\_Fac} \cite{jin2022fast} aims to choose the pivot efficiently. Given a branch $B$, instead of finding an optimal pivot vertex that could minimize the number of produced sub-branches before the branching steps, \texttt{BK\_Fac} first {\cheng initializes} an arbitrary vertex in $g_C$ as pivot and iteratively changes to a new one if branching on it would produce fewer branches. However, given a branch $B=(S,g_C,g_X)$, \texttt{BK\_Rcd} and \texttt{BK\_Fac} would produce $2^{|V(g_C)|}$ sub-branches in total in the worst-case, the time complexities of these two algorithms are $O(n\delta \cdot 2^{\delta})$. In \cite{deng2023accelerating}, several graph reduction rules are proposed to improve the performance pratically. We note that these rules are orthogonal to frameworks. 
%

% {\chengB \underline{For the latter}}, 
{\chengc For the latter,}
they can be viewed as different instances of the general reverse-search enumeration framework \cite{avis1996reverse}. {\cheng It} traverses from one solution to another solution following a depth-first search (DFS) procedure on an implicit connected solution graph. 
% has an implicit connected solution graph,  where each vertex corresponds to a solution and each edge corresponds to the traversal from one solution to another, and finds all solutions in the solution graph by a depth-first search (DFS) procedure. 
%
Although reverse-search based algorithms can guarantee that the time cost between two consecutive outputs is bounded by a polynomial function of the input size (i.e., polynomial delay), which implies that the time complexity of these algorithm is proportional to the number of maximal cliques within the input graph (i.e., output-sensitive), their performances on real-world graphs are not as {\cheng competitive} as those of branch-and-bound based algorithms \cite{das2018shared}. 
%

There are also numerous studies that develop parallel algorithms for MCE \cite{han2018speeding, inoue2014faster, wu2009distributed, schmidt2009scalable, lu2010dmaximalcliques, xu2015distributed, abu2017genome, lessley2017maximal, du2006parallel, cheng2012fast, blanuvsa2020manycore, das2020shared, brighen2019listing, chen2016parallelizing, hou2016efficient, svendsen2015mining}.
% \cite{wu2009distributed, schmidt2009scalable, lu2010dmaximalcliques, svendsen2015mining, xu2015distributed, abu2017genome, lessley2017maximal, du2006parallel, cheng2012fast, blanuvsa2020manycore, das2020shared, han2018speeding, brighen2019listing, chen2016parallelizing, hou2016efficient, inoue2014faster}, 
% {\cheng among} which \cite{han2018speeding, inoue2014faster} target the data-level parallelization with SIMD instructions, 
% \cite{wu2009distributed, schmidt2009scalable, lu2010dmaximalcliques, xu2015distributed, abu2017genome, lessley2017maximal, du2006parallel, cheng2012fast, blanuvsa2020manycore, das2020shared} target the task-level parallelization with shared-memory setting and 
% \cite{brighen2019listing, chen2016parallelizing, hou2016efficient, svendsen2015mining} target the task-level parallelization with distributed-memory setting. 
These algorithms extend the techniques that are originally proposed for sequential algorithms and aim to balance and reduce the computation overheads to achieve higher degrees of parallelism. Besides, there are also several related studies that (1) solve {\cheng the} MCE problem on other graph types, such as uncertain graphs \cite{dai2022fast, mukherjee2015mining}, temporal graphs \cite{himmel2016enumerating}, attributed graphs \cite{pan2022fairness, zhang2023fairness} and graph streams \cite{das2019incremental, sun2017mining}, and (2) solve MCE's counterpart problem, such as maximal biclique enumeration on bipartite graph \cite{chen2022efficient, abidi2020pivot} and other maximal subgraph enumeration problems \cite{yu2023fast}. We note that the techniques proposed for these problems are not suitable for general MCE problem. 







% \smallskip\noindent
% \textbf{Listing $k$-cliques for arbitrary $k$ values.} 
% Existing exact $k$-clique listing algorithms for arbitrary $k$ values can be classified into two categories: backtracking based algorithms \cite{chiba1985arboricity} and branch-and-bound based algorithms \cite{yuan2017effective, li2020ordering, yuan2022efficient}.
% Specifically, the algorithm \texttt{Arbo} \cite{chiba1985arboricity} is the first practical algorithm for listing all $k$-cliques, whose time complexity ({\cheng we focus on the worst-case time complexies in this paper}) is $O(km\alpha^{k-2})$, where $m$ and $\alpha$ are the number of edges and the arboricity of the graph, respectively. However, {\cheng it is difficult to paralleize} \texttt{Arbo} 
% % is hard to be parallelized 
% since it involves a depth-first backtracking procedure. 
% %
% To solve this issue, several (vertex-oriented {\chengB branching-based}) branch-and-bound (BB) based algorithms are proposed, 
% % e.g., 
% {\cheng including}
% \texttt{Degree} \cite{ortmann2014triangle, finocchi2015clique}, \texttt{Degen} \cite{danisch2018listing}, \texttt{DegenCol} \cite{li2020ordering}, \texttt{DegCol} \cite{li2020ordering}, \texttt{DDegCol} \cite{li2020ordering}, \texttt{DDegree} \cite{li2020ordering}, \texttt{SDegree} \cite{yuan2022efficient} and \texttt{BitCol} \cite{yuan2022efficient}. As introduced in Section~\ref{sec:vbbkc}, these algorithms follow the 
% % similar 
% {\cheng same}
% {\chengB framework} but differ in how the vertex orderings are adopted {\cheng and some implementation details}.
% %
% Specifically, \texttt{Degree} uses a global degree ordering, with which {\cheng the size of} the largest problem instance produced 
% % by \texttt{Degree} 
% can be bounded by $\eta$ (i.e., the $h$-index of the graph).
% % thus it 
% \texttt{Degree} has a time complexity of $O(km(\eta/2)^{k-2})$. \texttt{Degen} uses a global degeneracy ordering, with which {\cheng the size of} the largest problem instance produced 
% % by \texttt{Degen} 
% can be bounded by $\delta$ (i.e., the degeneracy of the graph).
% % , thus it 
% \texttt{Degen} has a time complexity of $O(km(\delta/2)^{k-2})$. Since it has been proven that $\delta\le 2\alpha-1$ \cite{zhou1994edge}, \texttt{Degen} is the first algorithm that outperforms \texttt{Arbo} theoretically and practically. However, \texttt{Degen} suffers from the issue that it cannot list the clique whose size is near $\omega$ (i.e., the size of a maximum clique). 
% %
% To solve this issue, the authors in \cite{li2020ordering} propose several {\cheng algorithms, which are based on} {\chengB color-based vertex orderings}. \texttt{DegCol} and \texttt{DegenCol} first color the graph with some graph coloring algorithms (e.g., inverse degree based \cite{yuan2017effective} and inverse degeneracy based \cite{hasenplaugh2014ordering}) and generate the an ordering of vertices {\cheng based on the color values of the vertices}.
% % , which we call color ordering}. 
% {\cheng While the color values} of the vertices can significantly prune the unpromising search paths and make the algorithm efficient to list near-$\omega$ cliques, \texttt{DegCol} and \texttt{DegenCol} both {\cheng have} the time complexity of $O(km(\Delta/2)^{k-2})$, where $\Delta$ is the maximum degree of a vertex in the graph since the {\chengB color-based} ordering cannot guarantee a tighter size bound for the produced problem instance. 
% %
% To overcome this limitation, \texttt{DDegCol} adopts a hybrid ordering, where it first uses degeneracy ordering to branch the universal search space such that the size of each produced problem instance is bounded by $\delta$, then it uses {\chengB color-based} orderings to branch each produced sub-branch. Following a similar procedure, \texttt{DDegree} also combines degeneracy ordering and degree ordering to branch the universal search space and the sub-spaces, respectively. In this way, \texttt{DDegCol} and \texttt{DDegree} have the 
% % state-of-the-art 
% time complexity of $O(km(\delta/2)^{k-2})$. 
% %
% \texttt{BitCol} and \texttt{SDegree} implement \texttt{DDegCol} and \texttt{DDegree} in a more efficient way with SIMD instructions, respectively, 
% % but 
% {\cheng and}
% retain the same time complexity as that of \texttt{DDegCol} and \texttt{DDegree}. 
% %
% {\cheng In contrast, our \texttt{EBBkC} algorithm is an edge-oriented {\chengB branching-based BB} algorithm based on edge orderings and has its time complexity (i.e., $O(km(\tau/2)^{k-2})$) better than 
% % (if not the same as) 
% that of the state-of-the-art algorithms including \texttt{DDegCol}, \texttt{DDegree}, \texttt{BitCol} and \texttt{SDegree} (i.e., $O(km(\delta/2)^{k-2})$), where $\tau$ is strictly smaller than $\delta$. 
% % the truss number of the graph and we have $\tau < \delta$.
% }

 


% % which are originally designed for listing triangles an undirected graphs \cite{ortmann2014triangle}, are also applied to list cliques. 
% % The $k$-clique listing algorithms based on degree ordering \cite{finocchi2015clique} and degeneracy ordering \cite{danisch2018listing}, denoted by \texttt{Degree} and \texttt{Degen}, has a time complexity of $O(km{(\eta/2)}^{k-2})$ and $O(km{(\delta/2)}^{k-2})$, where $\eta$ and $\delta$ are the $h$-index and the degeneracy of the graph, respectively. Recently, the $k$-clique listing algorithms with color ordering further reduce the search space. The algorithm using inverse degree based \cite{yuan2017effective} and inverse degeneracy based \cite{hasenplaugh2014ordering} coloring, denoted by \texttt{DegCol} and \texttt{DegenCol}, runs much faster than \texttt{Degree} and \texttt{Degen}, but both have the same time complexity as \texttt{Degen}. As explained in Section~\ref{sec:intro}, these existing studies all generate the ordering by some heuristic policies, whose running time is far from the optimum as shown in our experiments in Section~\ref{sec:exp}. In addition, there are some other related studies on the problem of listing $k$-clique densest subgraphs \cite{sun2020kclist++, tsourakakis2015k}, listing maximal cliques \cite{makino2004new} and listing maximal quasi-cliques \cite{khalil2021parallel, guo2020scalable}, which either cannot adapt to $k$-clique listing problem setting \cite{sun2020kclist++, tsourakakis2015k, khalil2021parallel, guo2020scalable} or will result in higher time complexity after adaption \cite{makino2004new}. 



% Some other algorithms, e.g., \texttt{MACE} \cite{makino2004new}, 
% % that are originally targeted 
% {\cheng which are originally designed for}
% the maximal clique enumeration problem, can also be adapted to listing $k$-cliques problem \cite{makino2004new, schmidt2009scalable, takeaki2012implementation}. These adapted algorithms are mainly based on the well-known Bron-Kerbosch (BK) algorithm \cite{bron1973algorithm} with some size constraints to ensure that each clique to be outputted has exactly $k$ vertices. However, these adapted algorithm are even less efficient than \texttt{Arbo} theoretically and practically, e.g., \texttt{MACE} has a time complexity of $O(kmn\alpha^{k-2})$ \cite{schmidt2009scalable, li2020ordering}, 
% % which makes them hard to 
% {\cheng and cannot}
% handle large real graphs. 

% \noindent
% \textbf{Listing $k$-cliques for special $k$ values.} There are two special cases for $k$-clique listing problem: when $k=3$ and when $k=\omega$. When $k=3$, the problem reduces to triangle listing problem \cite{chiba1985arboricity, latapy2008main, ortmann2014triangle}. The state-of-the-art algorithm for triangle listing problem 
% % also 
% follows a vertex ordering based framework \cite{ortmann2014triangle}, whose time complexity is $O(m\alpha)$, where $\alpha$ is the arboricity of the graph. When $k=\omega$, the problem reduces to maximum clique search problem \cite{ostergaard2002fast, pattabiraman2015fast, lu2017finding, chang2019efficient}. The state-of-the-art algorithm for maximum clique search problem first transforms the maximum clique problem to a set of clique finding sub-problems, then it conducts a branch-and-bound framework to iteratively check whether a clique of a certain size can be found in the sub-problem \cite{chang2019efficient}, whose time complexity is $O(n 2^n)$. 
% % Although the triangle listing problem and the maximum clique search problem can be efficiently solved by existing studies, the algorithm cannot solve the $k$-clique listing problem since we do not know the value of $k$ in advance. 
% {\cheng We note that these existing algorithms cannot solve the $k$-clique listing problem for arbitrary $k$'s.}






% \noindent
% \textbf{Learning-based methods on graph problems.} 
% In recent years, many traditional graph problems, especially those in NP-complete, such as travelling salesman problem (TSP), minimum vertex cover (MVC) and subgraph isomorphism (SI), have attracted researchers to employ learning-based frameworks to solve them \cite{vinyals2015pointer, li2018combinatorial, khalil2017learning}. Generally speaking, these learning based methods first encode the input graph into some high dimension vectors then decode the vectors to generate feasible results. For the encoding network, it is a common practice to use a sequence model, such as LSTM \cite{hochreiter1997long} and Transformer \cite{vaswani2017attention}, or a graph neural network, such as GCN \cite{defferrard2016convolutional} and structure2vec \cite{dai2016discriminative}, to extract the representations of the graph. For the decoding network, its design depends mainly on the specific problem. For example, it is reasonable to use a sequence model for TSP \cite{vinyals2015pointer, khalil2017learning} while for MVC and SI, directly using a fully connect network to output how much probability each vertex belongs to the result set is a better choice \cite{li2018combinatorial}. Interested readers are referred to two surveys \cite{bengio2021machine, yow2022learning} for more details on this topic. However, all above mentioned models can only handle some small graphs with hundreds of nodes. As shown in \cite{li2018combinatorial}, the learning-based algorithms perform even worse than some classic heuristics when the graph size is larger than 10,000 nodes, while for $k$-clique listing problem, the graphs often contains millions of nodes. 



% \noindent
% \textbf{Reinforcement learning. }
% The goal of the reinforcement learning is to guide the agents in an unknown environment on how to map its situation to actions so as to maximize its accumulative rewards. The environment is generally formulated as a Markov Decision Process (MDP) \cite{puterman2014markov}. In this paper, we model the process of sequentially deciding which vertex is to color as an MDP and adopt a policy gradient method, namely proximal policy optimization (PPO) \cite{schulman2017proximal}, to solve the MDP. Recently, RL has been successfully applied to some graph optimization problems. For example, Khalil et al. \cite{khalil2017learning} and Bello et al. \cite{bello2016neural} use RL model to optimize TSP. Wang et al. \cite{wang2021adaptive} designs effective RL model for bipartite matching. The most related study that also uses RL for vertex ordering is \cite{wang2022reinforcement}. However, \cite{wang2022reinforcement} differs from this study in that it targets subgraph matching problem, where only the vertices in the query graphs (less than 50 nodes) need to be ordered. 



==> 7._conclusion.tex <==
% \vspace{-4mm}
\section{Conclusion}
\label{sec:conclusion}


In this paper, we study the maximal clique enumeration (MCE) problem. 
% Existing algorithms, mostly utilizing the vertex-oriented Bron-Kerbosch (BK) branching in a branch-and-bound (BB) framework, have been effective but face challenges. Inspired by edge-oriented branching techniques from related problems, 
We propose a hybrid branch-and-bound (BB) algorithm, \texttt{HBBMC}, integrating both vertex-oriented and edge-oriented branching strategies, achieving a time complexity 
% of $O(\delta m + \tau m \cdot 3^{\tau/3})$. 
{\chengc which is better than the best-known one under a condition that holds for the majority of real-world grpahs.}
To further boost efficiency, we introduce an early termination technique, {\chengB which is} applicable across BB frameworks. Extensive experiments demonstrate the efficiency of our algorithms and the effectiveness
of proposed techniques.



\smallskip
\noindent\textbf{Acknowledgments.}
This research is supported by the Ministry of Education, Singapore, under its Academic Research Fund (Tier 2 Award MOE-T2EP20221-0013, Tier 2 Award MOE-T2EP20220-0011, and Tier 1 Award (RG20/24)). Any opinions, findings and conclusions or recommendations expressed in this material are those of the author(s) and do not reflect the views of the Ministry of Education, Singapore.

==> EBBkC.tex <==
% {\cheng\section{A New Branch-and-Bound Framework: \texttt{EBBkC}}}
\section{A New Branch-and-Bound Framework: \texttt{EBBkC}}

\label{sec:edge-oriented-bb-framework}

% \subsection{A New Branch-and-Bound Framework: \texttt{EBBkC}}

\subsection{{\cheng Motivation and Overview of \texttt{EBBkC}}}
\label{subsec:motivation}

Recall that for a branch $B = (S, g, l)$, the vertex-oriented branching forms a sub-branch by moving one vertex $v_i$ from $g$ to $S$. To improve the performance, existing studies consider the information of each vertex in $g$ towards pruning more sub-branches and/or forming sub-branches with smaller graph instances. Specifically, with the newly added vertex $v_i$, the produced sub-branch $B_i$ can shrink the graph instance $g$ as a smaller one induced by the neighbors of $v_i$ (e.g., removing those vertices that are not adjacent to $v_i$). As a result, one can prune the branch $B_i$ if $v_i$ has less than $(l-1)$ neighbors in $g$. In addition, one can produce a group of sub-branches with small graph instances by specifying the ordering of vertices in $g$ for branching.

% One interesting attempt is to 
In this paper, we propose to form a branch by \emph{moving two vertices that connect with each other} (correspondingly, an edge) from $g$ to $S$ at the same time. Note that the two vertices are required to be connected since otherwise they will not form a larger partial $k$-clique with $S$. 
% One desired property 
{\cheng The intuition} is that it {\cheng would allow} us to consider more information (i.e., an edge {\cheng or two vertices instead of a single vertex}) towards pruning more sub-branches and/or forming sub-branches with smaller graph instances. Specifically, with the newly added edge, the produced branch can shrink the graph instance as the one induced by the common neighbors of two vertices of the edge, which is smaller than that produced by the vertex-oriented branching (details {\chengB can be found} in Section~\ref{subsec:EBBkC-T}).
%
% As a result, we can explore different 
% {\cheng In fact, we explore an ordering of edges based on truss decomposition \cite{wang2012truss}, which we call \emph{truss-based edge ordering}, which helps to form} sub-branches with smaller graph instances (details find in Section~\ref{subsec:EBBkC-T}). 
{\cheng In addition}, we can prune more branches {\cheng based on} the information of {\cheng the added edge}, e.g., a produced branch can be pruned if the vertices in the newly added edge have less than $(l-2)$ common neighbors in $g$ (details {\chengB can be found} in Section~\ref{subsec:EBBkC-C}).
%
We call the above branching strategy \emph{edge-oriented branching}, which we introduce as follows. 
% We remark that \texttt{VBBkC} cannot incorporate the newly proposed branching strategy. 
% Below, we introduce an \emph{\underline{e}dge-oriented \underline{b}ranch-and-\underline{b}ound} framework for \underline{$k$}-\underline{c}lique listing called \texttt{EBBkC}.
% a new BB framework {\cheng based on the edge-oriented branching strategy for listing $k$-cliques, which we call \texttt{EBBkC}}.


\if 0
Consider the recursive process of \texttt{VBBkC} that starts from a branch $B=(S,g,l)$. Suppose we take each branch as a node and create directed links from a branch 
% $B'$
to {\kaixin{its produced sub-branches}}
% branch $B''$ if $B''$ is produced from $B'$ 
based on Eq.~(\ref{eq:vertex-oriented-branching}). Then, we obtain a \emph{recursion tree} rooted at $B$. The directed links from node $B$ correspond to the vertex-oriented branching at branch $B$; it iteratively includes to the partial clique $S$ \emph{each vertex} in $g$ based on an ordering of vertices which can be \emph{arbitrary}. 
%
%
We further review the recursion tree by aggregating every twice recursive branching at a branch as a unit. An illustration is shown in Figure~\ref{subfig:vbbkc}. We obtain the following observations regarding the branch $B$ and the group of sub-branches {\kaixin{rooted at $B_i$.}} 
% $\{B_{i,j} \mid 1\leq i\leq |V(g)|\ \text{and}\   1\leq j \leq |V(g_i)|\}$ within the same unit. 
\underline{First}, each {\kaixin{sub-branch rooted at $B_i$}}
% branch $B_{i,j}$ 
is produced by including to $S$ two \emph{connected} vertices in $g$. 
% , i.e., $S_{i,j}=S\cup\{v_i,u_{i,j}\}$ and $(v_i,u_{i,j})\in E(g)$. 
\underline{Second}, there would be $|E(g)|$ branches in total
% in the group 
and each of which 
% $B_{i,j}$ 
corresponds to including two end points of a distinct edge 
% $(v_i,u_{i,j})$ 
in $g$. Hence, one unit at branch $B$ can be regarded as a branching which we call \emph{vertex-oriented twice-branching}; it produces $|E(g)|$ sub-branches via iteratively including to the partial clique $S$ \emph{each edge} (i.e., pair of connected vertices) in $g$ based on \emph{certain} ordering of edges $\langle e_1, e_2, \cdots, e_{|E(g)|} \rangle$ in $g$; the edge ordering is determined by the given orderings of vertices (for vertex-oriented branching) at branches $B$ and $B_1, B_2, \cdots, B_{|V(g)|}$. Consequently, the recursion tree (i.e., execution of \texttt{VBBkC}) can also be interpreted as a series of recursive calls of vertex-oriented twice-branching.
  
Consider the vertex-oriented twice-branching at a branch $B=(S,g,l)$. We observe that \emph{though the orderings of vertices can be set arbitrarily, the resulting ordering of edges cannot be an arbitrary one.} 
%We observe that \emph{the ordering of edges cannot be an arbitrary one} since it is determined by the given orderings of vertices for vertex-oriented branching at branches $B$ and $B_1$, $B_2$, \cdots, $B_{|V(g)|}$. Specifically, given an ordering of vertices $\langle v_1, v_2,\cdots, v_{|V(g)|} \rangle$ (which can be arbitrary) for the vertex-oriented branching at $B$, we can thus partition the sequence   
%
This is because once the ordering of vertices $\langle v_1,v_2,\cdots,v_{|V(g)|} \rangle$ at $B$ is given, the resulting edge ordering $\langle e_1,e_2,\cdots,e_{|E(g)|}\rangle$ can be partitioned into $|V(g)|$ groups, {\kaixin{and the $i$-th group contains $|V(g_i)|$ edges. An illustration is shown in Figure~\ref{subfig:vbbkc}.}} Then the edges in the $i$-th group must include $v_i$ (for those edges in the $i$-th group, the ordering can be arbitrary by varying vertex ordering at $B_i$).
%
% Formally, it needs to satisfy the following constraint.
% \begin{equation}
%     v_i \in e_t \text{ where } 1\leq i\leq |V(g)| \text{ and } \sum_{j=1}^{i-1}|V(g_j)|+1 \leq t \leq \sum_{j=1}^{i} |V(g_j)|.\nonumber
% \end{equation}
Therefore, there exists some ordering of edges that always cannot be adopted by \texttt{VBBkC}.
%
%For example, two edges that share no common endpoint cannot appear in the same sub-sequence for any possible vertex ordering at $B$.
%
This would limit existing studies which adopt \texttt{VBBkC} and mainly focus on optimizing the ordering of vertices for branching.

\fi

\begin{algorithm}[t]
\small
\caption{The edge-oriented {\chengB branching-based} BB framework: \texttt{EBBkC}}
\label{alg:EBBkC}
\KwIn{A graph $G=(V,E)$ and an integer $k\geq 3$}
\KwOut{All $k$-cliques within $G$}
\SetKwFunction{List}{\textsf{EBBkC\_Rec}}
\SetKwProg{Fn}{Procedure}{}{}
\List{$\emptyset, G, k$}\;
\Fn{\List{$S, g, l$}} {
    \tcc{Pruning}
    \lIf{$|V(g)|<l$}{\textbf{return}}
    \tcc{Termination when $l=1$ or $l=2$}
    \uIf{$l=1$}{
       \lFor{each vertex $v$ in $g$}{
                \textbf{Output} a $k$-clique $S\cup\{v\}$
       }
       \textbf{return}\;
    }\ElseIf{$l=2$}{
       \lFor{each edge $(u,v)$ in $g$}{
                \textbf{Output} a $k$-clique $S\cup\{u,v\}$
       }
       \textbf{return}\;
    }
    \tcc{Branching when $l\geq 3$}
    \For{each edge $e_i\in E(g)$ based on a given edge ordering}{
        Create branch $B_i=(S_i,g_i,l_i)$ based on Eq.~(\ref{eq:edge-oriented-branching})\;
        \List{$S_i, g_i, l_i$}\;
    }
}
\end{algorithm}

% We propose an \emph{\underline{e}dge-oriented \underline{b}ranch-and-\underline{b}ound} framework for \underline{$k$}-\underline{c}lique listing called \texttt{EBBkC}. 
% Specifically, \texttt{EBBkC} starts from the initial branch $(\emptyset,G,k)$ and recursively partitions a branch into new sub-branches via the newly proposed {edge-oriented branching}. 
Consider the branching step at a branch $B=(S,g,l)$. Let $\langle e_1,e_2,\cdots,e_{|E(g)|} \rangle$ be an \emph{arbitrary} ordering of edges in $g$. Then, the branching step would produce $|E(g)|$ new sub-branches from $B$. The $i$-{th} branch, denoted by $B_i=(S_i,g_i,l_i)$, includes to $S$ 
{\kaixin{{\chengB the two vertices incident to} the edge $e_i$, i.e., $V(e_i)$,}} 
% connected by $e_1$ 
and excludes from $g$ those edges in $\{e_1,e_2,\cdots,e_{i-1}\}$ (and those vertices that {\Revise are disconnected from}\marginpar{R4D3} the vertices incident to $e_i$). Formally, for $1\leq i \leq |E(g)|$, we have
%
\begin{equation}
\label{eq:edge-oriented-branching}
   % S_i=S\cup V(e_i),\ g_i=g[N(V(e_i),g[e_i,\cdots,e_{|E(g)|}])],\ l_i=l-2.
    S_i=S\cup V(e_i),\quad     g_i=\overline{g}_i[N(V(e_i),\overline{g}_{i})],\quad l_i=l-2,
\end{equation}
% where $\overline{g}_{i}=g[e_i,\cdots,e_{|E(g)|}]$ is a subgraph of induced by the set of edges 
{\cheng where $\overline{g}_{i}$ is a subgraph of $g$ induced by the set of edges $\{e_i, e_{i+1}, \cdots, e_{|E(g)|}\}$, i.e., $\overline{g}_{i} = g[e_i,\cdots,e_{|E(g)|}]$.}
{\kaixin 
% based on an ordering of the edges, which is to ensure that each $k$-clique will be listed exactly once. 
We note that (1) $N(V(e_i),\overline{g}_{i})$ is to filter out those vertices that are not adjacent to
% the end points of 
{\chengB the two vertices incident to}
$e_i$ since they cannot form any $k$-cliques with $e_i$ and (2) $\overline{g}_i[N(V(e_i),\overline{g}_{i})]$ is the graph instance for the sub-branch induced by the vertex set $N(V(e_i),\overline{g}_{i})$ in $\overline{g}_{i}$. }


%
% Similarly, the branching 
% also 
The edge-oriented branching also corresponds to a recursive binary partition process, as illustrated in Figure~\ref{subfig:ebbkc}. Specifically, it first divides branch $B$ into two sub-branches based on $e_1$: one moves $e_1$ from $g$ to $S$ (this is the branch $B_1$ which will list those $k$-cliques in $B$ that include edge $e_1$), and the other removes $e_1$ from $g$
% and thus excludes $e_1$ from being added to $S$ 
% (this is $(S,\overline{g}_2,l)$ which 
(so that it will list others that exclude $e_1$). For branch $B_1$, it also removes from $g$ those vertices that are not adjacent to the vertices in $V(e_1)$ (i.e., $g_1=\overline{g}_1[N(V(e_1),\overline{g}_{1})]$) since they cannot form any $k$-clique with $e_1$. Then, it recursively divides the latter into two new sub-branches: one moves $e_2$ from $\overline{g}_2$ to $S$ (this the branch $B_2$ which will list those $k$-cliques in $B$ that exclude $e_1$ and include $e_2$), and the other removes $e_2$ from $\overline{g}_2$ 
% (this is $(S,\overline{g}_3,l)$ which 
(so that it will list others that exclude $\{e_1,e_2\}$). It continues the process, until the last branch $B_{|E(g)|}$ is formed. 
% We note that branch $B_i$ will list those $k$-cliques in $B$ that include $e_i$ and exclude $\{e_1,\cdots,e_{i-1}\}$. Consequently, all $k$-cliques in $B$ will be listed exactly once after the branching.

% We call the above branching \emph{edge-oriented branching} since it branches based on edges in $g$. 
{\cheng We call the \emph{\underline{e}dge-oriented branching-based \underline{BB} framework for \underline{$k$}-\underline{c}lique listing \texttt{EBBkC}.}}
We present in Algorithm~\ref{alg:EBBkC} the pseudo-code of \texttt{EBBkC}, which differs with \texttt{VBBkC} mainly in the branching step (lines {\cheng 10-}11). 
% In particular, the edge-oriented branching employed in \texttt{EBBkC} allows an arbitrary ordering of edges for branching while the vertex-oriented twice-branching in \texttt{VBBkC} cannot do so. 
{\cheng
% \smallskip 
% \noindent\textbf{Remark.} 
{\chengB We note that while} a branching step in our edge-oriented branching (i.e., including an edge) can be treated as two branching steps in the existing vertex-oriented branching (i.e., including two vertices of an edge via two steps), our \texttt{EBBkC} has a major difference from \texttt{VBBkC} as follows. For the former, we can explore \emph{arbitrary} edge orderings for each branching step while for the latter, the underlying edge orderings are \emph{constrained} by the adopted vertex ordering. For example, once a vertex ordering is decided for vertex-oriented branching with vertex $v_i$ appearing before $v_j$, then the edges that are incident to $v_i$ would appear before those that are incident to $v_j$ for the corresponding edge-oriented branching. For this reason, the existing \texttt{VBBkC} framework is covered by our \texttt{EBBkC} framework, i.e., for any instance of \texttt{VBBkC} with a vertex ordering, there exists an edge ordering such that the corresponding \texttt{EBBkC} instance is equivalent to the \texttt{VBBkC} instance, \emph{but not vice versa}. This explains why the time complexity of \texttt{EBBkC} based on some edge ordering is better than that of \texttt{VBBkC} (details can be found in Section~\ref{subsec:EBBkC-T}).
}

In the sequel, we explore different {\cheng orderings} of edges in \texttt{EBBkC}.
% to boost the performance. In fact, 
{\chengB Specifically, with the proposed truss-based edge ordering}, \texttt{EBBkC} would have the worst-case time complexity of $O(k m  (\tau/2)^{k-2})$ with $\tau < \delta$, {\cheng i.e., the time complexity is strictly better than that of the state-of-the-art \texttt{VBBkC} algorithms (which is $O(k m  (\delta/2)^{k-2})$)} 
% which is strictly smaller than that of the \texttt{VBBkC} algorithm based on vertex-oriented branching 
(Section~\ref{subsec:EBBkC-T}). 
{\chengB With the proposed color-based edge ordering}, \texttt{EBBkC} can apply some pruning rules to improve the efficiency in practice (Section~\ref{subsec:EBBkC-C}). Finally, with the proposed hybrid {\chengB edge} ordering, \texttt{EBBkC} would inherit both the above theoretical {\chengB result} and practical {\chengB performance} (Section~\ref{subsec:EBBkC-H}). 
% In summary, they demonstrate the benefits of our framework \texttt{EBBkC} compared to \texttt{VBBkC}.




\begin{algorithm}[t]
\small
% \caption{The edge-oriented BB framework: \texttt{EBBkC-T}}
\caption{{\cheng \texttt{EBBkC} with truss-based edge ordering}: \texttt{EBBkC-T}}
\label{alg:EBBkC-T}
\KwIn{A graph $G=(V,E)$ and an integer $k\geq 3$}
\KwOut{All $k$-cliques within $G$}
\SetKwFunction{List}{\textsf{EBBkC-T\_Rec}}
\SetKwProg{Fn}{Procedure}{}{}
\tcc{Initialization and branching at $(\emptyset,G,k)$}
$\pi_\tau(G)\leftarrow$ the truss-based ordering of edges in $G$\;
\For{{\kaixin each edge $e_i\in E(G)$ following $\pi_\tau(G)$}}{
    {\kaixin Obtain $S_i$ and $g_i$ according to Eq.~(\ref{eq:edge-oriented-branching})}\;
    {\Revise Initialize $VSet(e_i)\leftarrow V(g_i)$ and $ESet(e_i)\leftarrow E(g_i)$}\;
    % $S_i\leftarrow V(e_i)$ and $g\leftarrow (V[e],E[e])$ according to Eq.~(\ref{eq:edge-oriented-branching})\;
    \List{$S_i, g_i, k-2$}\;
}
% \tcc{Edge-oriented branching at $(\emptyset,G,k)$}
% \For{each edge $e$ in $E(G)$}{
%     $S\leftarrow V(e)$ and $g\leftarrow (V[e],E[e])$ according to Eq.~(\ref{eq:edge-oriented-branching})\;
%     \List{$S, g, k-2$}\;    
% }
\Fn{\List{$S, g, l$}} {
    Conduct Pruning and Termination (lines 3-9 of Algorithm~\ref{alg:EBBkC})\; 
    \tcc{Branching when $l\geq 3$}
    \For{each edge $e$ in $E(g)$}{
    % \For{each edge $e\in E(g)$ {\cheng following $\pi_\tau(G)$}}{
        {\Revise $S'\leftarrow S\cup V(e)$, $g'\leftarrow (V(g)\cap VSet(e), E(g)\cap ESet(e))$}\;
        \List{$S', g', l-2$}\;
    }
}
\end{algorithm}



\subsection{\texttt{EBBkC-T}: {\cheng \texttt{EBBkC} with the} Truss-based Edge Ordering}
\label{subsec:EBBkC-T}

Consider the edge-oriented branching at $B=(S,g,l)$ based on an ordering of edges $\langle e_1,e_2,\cdots,e_{|E(g)|}\rangle$. For a {\chengB sub-branch} $B_i$ ($1\leq i \leq |E(g)|$) produced from $B$, we observe that the size of graph instance $g_i$ {\cheng (i.e., the number of vertices in $g_i$)}\marginpar{R4D5}
% corresponds to 
{\chengB is equal to}
the number of common neighbors of vertices in $V(e_i)$ {\chengB in $\overline{g}_i$}, which depends on the ordering of edges. Formally, we have 
\begin{equation}
|V(g_i)|=|N(V(e_i),\overline{g}_i)|,\ \text{where}\ \overline{g}_i=g[e_i,\cdots,e_{|E(g)|}].    
\end{equation}
%
Recall that the smaller a graph instance is, the faster the corresponding branch can be solved. %
Therefore, to reduce the time costs, we {\cheng aim} to minimize the {\cheng sizes} of graph instances by determining the ordering of edges via the following greedy procedure.

\smallskip
\noindent\textbf{Truss-based edge ordering.} We determine the ordering of edges by an iterative process. Specifically, it iteratively removes from $g$ the edge whose vertices have the smallest number of common {\Revise neighbors}\marginpar{R4D9} (correspondingly, the smallest size of a graph instance), and then adds it to the end of the ordering. {\chengB Consequently}, for the $i$-th edge $e_i$ in the produced ordering ($1\leq i\leq |E(g)|$), we have
\begin{equation}
\label{eq:truss-based-edge}
    e_i = \min_{e\in E(g)\setminus \{e_1,\cdots,e_{i-1}\}} |N(V(e_i), g[E(g)\setminus \{e_1,\cdots,e_{i-1}\}])|.
\end{equation}
We call the above ordering \emph{truss-based edge ordering} of $g$ and denote it by $\pi_\tau(g)$ since the corresponding iterative process is the same to the \emph{truss decomposition}~\cite{che2020accelerating,wang2012truss,cohen2008trusses}, which can be done in $O(|E(g)|^{1.5})$ {\chengB time}. 

\smallskip
\noindent\textbf{The \texttt{EBBkC-T} algorithm.} 
% With the truss-based ordering, we design a new algorithm called \texttt{EBBkC-T}. 
{\cheng When the truss-based edge ordering is adopted in \texttt{EBBkC}, we call the resulting algorithm \texttt{EBBkC-T}.}
The pseudo-code of \texttt{EBBkC-T} is presented in Algorithm~\ref{alg:EBBkC-T}. 
%
In particular, it only computes the truss-based edge ordering of $G$ (i.e., $\pi_{\tau}(G)$) for the branching at the initial branch $(\emptyset,G,k)$ (lines 2-5). Then, for any other branching step at a following branch $(S,g,l)$, edges in $\langle e_1,e_2,\cdots,e_{|E(g)|} \rangle$ adopt the same ordering to those used in $\pi_{\tau}(G)$, which could differ with the truss-based edge ordering of $g$. Formally, $e_i$ comes before $e_j$ in $\langle e_1,e_2,\cdots,e_{|E(g)|} \rangle$ (i.e., $i<j$) if and only if it does so in $\pi_{\tau}(G)$. 
%
To implement this efficiently, it maintains two additional auxiliary sets, i.e., {\Revise $VSet(\cdot)$ and $ESet(\cdot)$}\marginpar{R4D5} (lines 2-4). The idea is that for an edge $e$, all edges in {\Revise $ESet(e)$ } are ordered behind $e$ in $\pi_{\tau}$ and the vertices incident to these edges are both connected with those incident to $e$. Therefore, the branching steps (with the introduced edge ordering) can be efficiently conducted via set intersections (line 9) for those branches following $(\emptyset,G,k)$. The correctness of this implementation can be easily verified. 
% (details of the proof find in the technical report).  



\smallskip
\noindent\textbf{Complexity.} 
% When applying the truss-based ordering $\pi_\tau(g)$ at branch $(S,g,l)$, one benefit is that the largest size of produce graph instance is \emph{strictly bounded} by the degeneracy of $g$. 
% Formally, we define by $\tau(g)$ the largest size of produced graph instance, 
{\cheng Given a branch $B=(S,g,l)$, let $\tau(g)$ be the largest size of a produced graph instance, i.e., }
\begin{equation}
\label{eq:tau}
    \tau(g) = \max_{e_i\in E(g)} |V(g_i)|.
    %\coloneq |N(V(e_i),\overline{g}_i)|\ \text{where}\ \overline{g}_i=g[e_i,\cdots,e_{|E(g)|}].\nonumber
\end{equation}
% We summarize the above observation in the following lemma.
{\cheng We have the following observation.}
\begin{lemma}
\label{lemma:comparison}
    When applying the truss-based {\chengB edge} ordering $\pi_\tau(g)$ at $(S,g,l)$, we have $\tau(g)<\delta(g)$, where $\delta(g)$ is the degeneracy of $g$.
\end{lemma}
\begin{proof}
    We prove by contradiction. Suppose that $\tau\ge \delta$. Since $\delta$ is defined as the largest value of $k$ such that the $k$-core of $g$ is non-empty, there must not have a $(\delta+1)$-core in $g$, i.e., $V(C_{\delta+1})=\emptyset$. {\chengB Here, $C_k$ refers to a $k$-core.}
    Consider the branching step at such an edge $e_i\in E(g)$ that produces the largest size of graph instance, i.e., $|V(g_i)|=\tau$. According to Eq.~(\ref{eq:truss-based-edge}), $e_i$ has the minimum number of common neighbors of its end points in the graph $\overline{g}_i=g[e_{i},\cdots, e_{|E(g)|}]$. This means for each edge $e\in E(\overline{g}_i)$, the number of common neighbors of the end points of $e$ is no less than $\tau$, i.e., $|N(V(e), \overline{g}_i)| \ge \tau$,
    % where $G_{{i}}$ is the subgraph of $G$ induced by  $\{e_{i},\cdots, e_{|E|}\}$. 
    Obviously, $\overline{g}_{i}$ is non-empty, i.e., $V(\overline{g}_{i})\neq \emptyset$. 
    Then for each vertex $v\in V(\overline{g}_{i})$, the number of its neighbors is at least $\tau+1$, i.e., $|N(v,\overline{g}_{i})|\ge \tau+1$. Therefore, $\overline{g}_{i}$ is a subgraph of $(\tau+1)$-core, i.e., $V(\overline{g}_{i})\subseteq V(C_{\tau+1})$. According to the hereditary property of $k$-core\footnote{{\kaixin The hereditary property claims that given a graph $G$ and two integers $k$ and $k'$ with $k\le k'$, then the $k'$-core of $G$ is a subgraph of the $k$-core of $G$ \cite{batagelj2003m}.}} and the hypothesis $\tau\ge\delta$, we have $V(C_{\tau+1}) \subseteq V(C_{\delta+1})$, which leads to a contradiction that $V(\overline{g}_{i})\subseteq V(C_{\tau+1})\subseteq V(C_{\delta+1})= \emptyset$. 
\end{proof}






%
{\cheng Based on the above result, we derive that}
the time complexity of \texttt{EBBkC-T} is strictly smaller than that of the state-of-the-art {\chengB algorithms}, i.e., $O(k m  (\delta/2)^{k-2})$, which we show in the following theorem.\marginpar{R4O2(3)}

\begin{theorem}
\label{theo:ebbkc-t}
     Given a graph $G=(V,E)$ and an integer $k\geq 3$, the time and {\Revise space complexities of \texttt{EBBkC-T} are} $O(k m  (\tau/2)^{k-2})$ and {\Revise $O(m+n)$}, respectively, where $\tau=\tau(G)$ and it is strictly smaller than the degeneracy $\delta$ of $G$.
\end{theorem}


\begin{proof}
    We give a sketch of the proof and put the details in the technical report \cite{wang2024technical}. The running time of \texttt{EBBkC-T} is dominated by the recursive listing procedure (lines 6-10 of Algorithm~\ref{alg:EBBkC-T}). 
    Given a branch $B=(S, g, l)$, we denote by $T(g, l)$ the upper bound of time cost of listing $l$-cliques under such a branch. When $k\ge 3$, with different values of $l$, we have the following recurrences. 
\begin{equation}
\label{eq:ebbkc-recurrence-main}
T(g, l) \le \left\{
\begin{array}{lc}
    O(k\cdot |V(g)|) & l = 1\\ 
    O(k\cdot |E(g)|) &  l = 2 \\ 
    \sum_{e\in E(g)} \Big( T(g', l-2) + T'(g') \Big) & 3\le l\le k-2 \\
\end{array}
\right.
\end{equation}
where $T'(g')$ is the time for constructing $g'$ given $B=(S, g, l)$ (line 9 {\chengB of Algorithm~\ref{alg:EBBkC-T}}). We show that with different values of $l$, $T'(g')$ satisfies the following equation. 
\begin{equation}
\label{eq:close-T-prime-main}
    \sum_{e\in E(g)} T'(g') = \left\{
\begin{array}{lc}
    O(\tau \cdot |E(g)|) & l = 3 \\
    O(\tau^2 \cdot |E(g)|) & l > 3 \\
\end{array}
\right.
\end{equation}
The reason is as follows. When given a branch $B=(S,g,l)$ with $l=3$, for each edge, we just need to compute $V(g')$ for the sub-branch (since the termination when $l=1$ only cares about the vertices in $g'$), which can be done in $O(\tau)$. When given a branch $B=(S,g,l)$ with $l>3$, for each edge, we need to construct both $V(g')$ and $E(g')$, which can be done in $O(\tau^2)$ since there are at most $\tau(\tau-1)/2$ edges in $g$. Besides, we show that given a branch $B=(S,g,l)$ and the sub-branches $B'=(S',g',l')$ produced at $B$, we have
\begin{equation}
    \sum_{e\in E(g)} |E(g')| < \left \{
    \begin{array}{lc}
      \frac{\tau^2}{4} \cdot |E(g)|   &  l < k \\
       \frac{\tau^2}{2} \cdot |E(g)|  & l = k
    \end{array}
\right.
\end{equation}
This inequality is proven by a lemma in the technical report \cite{wang2024technical}. With above inequalities, we can prove the theorem by induction on $l$. 
\end{proof}


\marginpar{R2O2\\ R3O3\\ R4O2(1)}
{\Revise 
\smallskip
\noindent\textbf{Discussion on $\tau$.}
By definition, $\tau$ of a graph $G$, i.e., $\tau(G)$, corresponds to the largest integer such that there exists a non-empty subgraph where the two vertices of each edge have at least $\tau$ common neighbors.
%
Similar to the degeneracy $\delta$ of the graph, $\tau$ also measures the density of a graph, say, the larger the value of $\tau$, the denser the graph. However, $\tau$ is always smaller than $\delta$ as it imposes stricter constraint on connections (i.e., the two vertices of every edge have at least $\tau$ common neighbors v.s. every vertex has at least $\delta$ neighbors). 
%
\underline{Theoretically}, for a graph with $n$ vertices, the gap between $\delta$ and $\tau$ can be as large as $n/2$.
% , which can be infinity. 
To see this, consider a complete bipartite graph with $p$ vertices on each side, where $p$ is a positive integer. For this graph, we have $\delta = p$ since each vertex has exactly $p$ neighbors and $\tau = 0$ since the two vertices of each edge have no common neighbors.
\underline{Practically}, the ratio $\tau/\delta$ is below 0.8 for many real-world graphs. For example, we have collected the statistics of $\tau/\delta$ on 139 more real-world graphs \cite{RealGraphs} and found that the ratio is below 0.8 for the majority of the graphs (105 out of 139). 
Since our algorithms runs ${(\delta/\tau)}^{k-2}$ times faster than the state-of-the-art (i.e., $O(km(\tau/2)^{k-2})$ vs. $O(km(\delta/2)^{k-2})$), when $\tau/\delta$ is at most 0.8 and $k=12$, the speedup of our algorithm would be at least $1.25^{10} = 9.31$, which is already about an order of magnitude.
}






\smallskip
\noindent\textbf{Remark.} 
{\Revise (1) We note that given an integer $k\ge 3$, the time cost of generating the truss-based edge ordering, which is $O(m^{1.5})$, is dominated by the cost of the recursive listing procedure, which is $O(km(\tau/2)^{k-2})$, under the worst case. This is because $\tau$ is tightly bounded by $\delta$ (e.g., in a complete graph, $\tau = \delta - 1$) and $\delta$ is tightly bounded by $O(\sqrt{m})$ according to the results in~\cite{barenboim2008sublogarithmic, lin2012arboricity}.}\marginpar{R4O2(2)}
% {\yuiR The time of generating the truss-based edge ordering is $O(m^{1.5})$, which is dominated by $O(km(\tau/2)^{k-2})$ when $k\ge 3$ since $\tau <\delta$ (Lemma~\ref{lemma:comparison}) and $ \delta< 2\sqrt{m}$~\cite{barenboim2008sublogarithmic,lin2012arboricity}.}
(2) We note that another option of designing \texttt{EBBkC-T} is to 
{\chengB compute the truss-based edge ordering for each individual branch and use it for branching at the branch.}
% apply the truss-based edge ordering for all branching steps. 
However, it {\chengB would} introduce additional time cost 
{\chengB without achieving} better theoretical time complexity. Thus, we {\chengB choose not to adopt this option.} 
% implement \texttt{EBBkC-T} in such way. 
{\kaixin
(3) It is worthy noting that for a truss-based edge ordering, {\chengB there} does not always exist a vertex ordering such that the instance of \texttt{VBBkC} {\chengB with the vertex ordering} is equivalent to the instance of \texttt{EBBkC-T}. {\chengB We include a counter-example in the technical report~\cite{wang2024technical} for illustration.}
}

% the resulting algorithm is not efficient in practice since computing the truss-based ordering for every branch is costly (which will be verified in our experiments) and cannot achieve better theoretical time complexity.


\begin{algorithm}[t]
\small
% \caption{The edge-oriented BB framework: \texttt{EBBkC-C}}
\caption{{\cheng \texttt{EBBkC} with color-based edge ordering}: \texttt{EBBkC-C}}
\label{alg:EBBkC-C}
\KwIn{A graph $G=(V,E)$ and an integer $k\geq 3$}
\KwOut{All $k$-cliques within $G$}
\SetKwFunction{List}{\textsf{EBBkC-C\_Rec}}
\SetKwProg{Fn}{Procedure}{}{}
Conduct vertex coloring on $G$ and get $id(v)$ for each vertex in $V$\;
$\overrightarrow{G}\leftarrow (V,\overrightarrow{E})$ where $\overrightarrow{E}=\{u\rightarrow v \mid (u,v)\in E \land id(u)<id(v)\}$\;
\List{$\emptyset,\overrightarrow{G}, k$}\;

\Fn{\List{$S, \overrightarrow{g}, l$}} {
    Conduct Pruning and Termination (line 3-9 of Algorithm~\ref{alg:EBBkC})\; 
    \tcc{Branching when $l\geq 3$}
    \For{each edge $u\rightarrow v$ in $E(\overrightarrow{g})$}
    % \For{each edge $u\rightarrow v$ in $E(\overrightarrow{g})$ {\cheng following the color-based ordering}}
    {
        $S'\leftarrow S\cup \{u,v\}$ and $\overrightarrow{g}'\leftarrow \overrightarrow{g}[N^+(\{u,v\},\overrightarrow{g})]$\;
        % \lIf{one of pruning conditions is satisfied}{\textbf{continue}}
        \lIf{either of the rules of pruning applies}{\textbf{continue}}
        \List{$S', \overrightarrow{g}', l-2$}\;
    }
}
\end{algorithm}


\subsection{\texttt{EBBkC-C}: {\cheng \texttt{EBBkC} with the} Color-based Edge Ordering}
\label{subsec:EBBkC-C}


{\kaixin 
{\cheng While the truss-based edge ordering helps to form sub-branches with small sizes at a branch, it does not offer much power to prune the formed sub-branches - all we can leverage for pruning are some size constraints (line 3 of Algorithm~\ref{alg:EBBkC}). On the other hand, some existing studies of \texttt{VBBkC} have successfully adopted color-based \emph{vertex} ordering for effective pruning~\cite{hasenplaugh2014ordering, yuan2017effective}. Specifically, consider a branch $B=(S,g,l)$. They first color the vertices in $g$ by iteratively assigning to an uncolored vertex $v$ the smallest color value taken from $\{1,2,\cdots\}$ that has not been assigned to $v$'s neighbours. {\chengB Let $c$ be the number of color values used by the coloring procedure.} They then obtain a vertex orderng by sorting the vertices in a non-increasing order based on the color values $\langle v_1,v_2,\cdots,v_{|V(g)|} \rangle$ (with ties broken by node ID), i.e., for $v_i$ and $v_j$ with $i<j$, we have $col(v_i)\geq col(v_j)$, where $col(\cdot)$ is the color value of a vertex. As a result, they prune the sub-branch $B_i=(S_i, g_i, l_i)$, which includes $v_i$ to $S$, if $col(v_i)<l$.}
% The main limitation of \texttt{EBBkC-T} is that it is unable to prune some unpromising search paths where no $k$-clique can be found inside since its pruning technique only relies on some size constraints (line 3 of Algorithm~\ref{alg:EBBkC}). 
% To overcome this limitation, we observe that existing studies for \texttt{VBBkC} utilize the graph coloring technique~\cite{hasenplaugh2014ordering, yuan2017effective} and obtain some color ordering of vertices, which can significantly reduce the search space and sharply improve the efficiency \cite{li2020ordering}. Specifically, consider a branch $B=(S,g,l)$, assume that $g$ can be colored with $c$ colors. Existing studies first color the vertices in $g$ by iteratively assigning to an uncolored vertex $v$ the smallest color value taking from $\{1,2,\cdots, c\}$ that has not been assigned to $v$'s neighbours, such that no two adjacent vertices have the same color value. 
%
% Then the color-based vertex ordering is obtained by sorting the vertices in a non-increasing ordering of color value $\langle v_1,v_2,\cdots,v_{|V(g)|} \rangle$ (break ties by node ID), i.e., $col(v_i)\geq col(v_j)$ for $i<j$, where $col(\cdot)$ is the color value of a vertex. Consider a branching step at $v_i$ from $B=(S,g,l)$. With the color-based vertex ordering, the sub-branch $B_i=(S_i, g_i, l_i)$ produced at $v_i$ can be pruned if $col(v_i)<l$. 
The rationale is that since all vertices in $g_i$ have their color values strictly smaller than $col(v_i)$ (according to Eq.~(\ref{eq:vertex-oriented-branching}) and the definition of the color-based vertex ordering), they do not have $l-1$ different color values, indicating $g_i$ does not contain any $(l-1)$-cliques, {\cheng and therefore} $B_i$ can be pruned.



% We observe that \emph{there would be no $k$-clique to be listed within $B$ if the vertices in $g$ have less than $l$ distinct colors}, which can be safely pruned. The reason is that every two vertices in a clique are connected with an edge and they must have different colors after coloring. 



% The rationale is \emph{there would be no $k$-clique to be listed within $B$ if the vertices in $g$ have less than $l$ distinct colors}. 

Recall that in Section~\ref{subsec:motivation}, for an instance of \texttt{VBBkC} with a vertex ordering, there {\cheng would} exist an edge ordering such that the corresponding \texttt{EBBkC} instance {\cheng based on the edge ordering} is equivalent to the \texttt{VBBkC} instance. 
% This motivates us to think of whether we can first transform a color-based vertex ordering to its corresponding color-based edge ordering and use the information of two end points of an edges to conduct more powerful pruning. Our design is as follows. 
{\cheng Motivated by this, we propose to adopt the edge ordering that corresponds to the color-based vertex ordering, which we call \emph{color-based edge ordering}, for our \texttt{EBBkC}. One immediate benefit is that it would naturally inherit the pruning power of the color-based vertex ordering, which has been demonstrated for \texttt{VBBkC}~\cite{hasenplaugh2014ordering, yuan2017effective}. Furthermore, it would introduce new opportunities for pruning, compared with existing \texttt{VBBkC} with the color-based vertex ordering, since it can leverage the two {\chengB vertices incident to} an edge collectively (instead of a single vertex twice as in \texttt{VBBkC}) for designing new pruning rules, which we explain next.}

% design our color-based edge ordering and the corresponding pruning rules. 

}


\if 0
{\cheng \textbf{***Since the color ordering has been used for VBBkC, we'd better start with color ordering for VBBkC, then discuss the adaption for EBBkC, and then present why and how we can do better for VBBkC. Currently, we directly present our techniques - in fact the intuition presented in the first paragraph should not be presented as a new result.***}}
Consider a branch $B=(S,g,l)$, we can color the vertices of graph instance $g$ such that no two adjacent vertices are of the same color, which corresponds to the \emph{vertex coloring} problem. We observe that \emph{there would be no $k$-clique to be listed within $B$ if the vertices in $g$ have less than $l$ distinct colors}, which can be safely pruned. The reason is that every two vertices in a clique are connected with an edge and they must have different colors after coloring. 
% and thus there is no $l$-clique in $g$. 
% Consequently, branch $B$ can be pruned. 
%
To prune as many branches as possible, we design a color-based edge ordering and some additional pruning rules.
\fi


\begin{figure}[t]
\vspace{-6mm}
\subfigure[An example graph $G$.]{
    \label{subfig:g2}
    \includegraphics[width=0.23\textwidth]{figs/example/exp_graph2.pdf}}
\subfigure[The DAG built upon $G$ {\chengB (the numbers inside circles are the color values)}.]{
    \label{subfig:color-dag}
    \includegraphics[width=0.23\textwidth]{figs/example/exp_DAG2.pdf}}
\vspace{-5mm}
\caption{Color-based edge ordering and pruning rules.}
\label{fig:example2}
\vspace{-6mm}
\end{figure}


\smallskip
\noindent\textbf{Color-based edge ordering and pruning rules.} 
Consider the branch $B=(S,g,l)$. 
% Similar to the existing studies, 
We first color the graph $g$ {\cheng using} the graph coloring technique~\cite{hasenplaugh2014ordering, yuan2017effective} and obtain the color-based vertex ordering $\langle v_1,v_2,\cdots,v_{|V(g)|} \rangle$ such that $col(v_i)\geq col(v_j)$ for $i<j$. 
% Assume that $G$ can be colored using $c$ colors. We assign each vertex an integer color value taken from $\{1,2,\cdots,c\}$ using any greedy coloring algorithm~\cite{hasenplaugh2014ordering, yuan2017effective} such that no two adjacent vertices have the same color value. Specifically, the coloring step iteratively assigns to an uncolored vertex $v$ the smallest color value that has not been assigned to $v$'s neighbours. 
% {\color{blue} An illustration is shown in Figure~\ref{fig:example2}.}
%
% We denote by $col(u)$ the color value of a vertex $u$, and sort the vertices in {\cheng a} non-increasing ordering of color value $\langle v_1,v_2,\cdots,v_{|V|} \rangle$ ({\cheng we} break ties by node ID), i.e., $col(v_i)\geq col(v_j)$ for $i<j$. 
Then for each vertex $u\in V(g)$, let $id(u)$ be the position of a vertex $u$ in the ordering. 
{\kaixin{For each edge $e=(u,v)\in E(g)$ {\cheng with $id(u)<id(v)$}, we define $str(e)$ 
% (where $e=(u,v)$ with $id(u)<id(v)$) 
as a string,
% by concatenating 
{\cheng which is the concatenation of}
$id(u)$ and $id(v)$ (i.e., $str(e)=$`$id(u)$+$id(v)$').}} 
%
Finally, we {\cheng define} the color-based edge ordering 
% by 
% sorting each edge $e$ in $g$ 
% following 
{\cheng as}
the alphabetical ordering {\cheng based on} $str(e)$ for {\cheng edges} $e\in E(g)$. {\cheng That is}, one edge $e = (u,v)$ 
{\cheng with $id(u)<id(v)$}
% (where $e=(u,v)$ with $id(u)<id(v)$) 
comes before {\chengB another edge} $e' = (u', v')$ {\cheng with $id(u')<id(v')$}
% (where $e'=(u',v')$ with $id(u')<id(v')$) 
if (1) $id(u)<id(u')$ or (2) $id(u)=id(u')$ and $id(v)<id(v')$.
%

% When applying the color-based edge ordering, it allows us to prune more branches, which we summarize in the following two rules. 
Consider a branch $B=(S,g,l)$ and 
% the branching step at an edge $e$ (where $e=(u,v)$ with $col(u)>col(v)$). 
{\cheng and a sub-branch $B_i$ that includes edge $e_i=(u,v)$ with $col(u)>col(v)$ to $S$.}
We can apply the following two pruning rules.
% We can safely prune the sub-branch if either of the following rules is satisfied:
% by adding an edge $e_i$ if either of the following conditions is satisfied, 
% which we summarize in the following lemma. 
% \begin{lemma}
% \label{lemma:prune}
%     {\cheng Consider} a branch $B=(S,g,l)$ and the branching step at an edge $e=(u,v)$. We can safely prune the produced sub-branch if either of the following rules is satisfied: (1) $\min\{col(u), col(v)\}<l-1$ or (2) the vertices in produced sub-branch have less than $l-2$ distinct color values. 
% \end{lemma}
%
\begin{itemize}[leftmargin=*]
    \item {\cheng \textbf{Rule (1).}} If $col(u)<l$ or $col(v)<l-1$, we prune sub-branch $B_i$;  
    \item {\cheng \textbf{Rule (2).}} If the vertices in produced sub-branch have less than $l-2$ distinct color values, we prune sub-branch $B_i$.  
\end{itemize}
%

{\kaixin 
We note that Rule (1) is 
{\cheng equivalent to the pruning that \texttt{VBBkC} with the color-based vertex ordering conducts at two branching steps of including $u$ and $v$~\cite{li2020ordering}.
% adapted from the color-based pruning technique (for vertex-oriented branching) proposed in~\cite{li2020ordering}, which can be easily verified. 
% Besides, 
% The Rule (2) is a new rule which is more powerful than the Rule (1). 
Rule (2) is a new one, which applies only in our \texttt{EBBkC} framework with the color-based edge ordering. In addition, Rule (2) is more powerful than Rule (1) in the sense that if Rule (2) applies, then Rule (1) applies, but not vice versa.}
}
{\kaixin The reason is that the color values of $u$ and $v$ are sometimes much larger than the number of distinct color values in the sub-branch since both color values consider the information of their own neighbors instead of their common neighbors. 
% Rule (1) must be violated (i.e., $\min\{col(u), col(v)\}\ge l-1$) if Rule (2) is violated (i.e., the vertices in produced sub-branch at least $l-2$ distinct color values) but not vice versa.} 
{\cheng For illustration}, consider the example in Figure~\ref{fig:example2} and assume that we aim to list 4-cliques (i.e., $k=4$). We focus on the edge ${EH}$. It is easy to check that 
{\cheng Rule (1) does not apply, but Rule (2) applies since the vertices in the produced sub-branch, i.e., $F$ and $G$, have only one color value.
Given that it takes $O(1)$ time to check if Rule (1) applies and $O(|V(g_i)|)$ time to check if Rule (2) applies, our strategy is to check Rule (1) first, and if it does not apply, we further check Rule (2).}
}
{\Revise
We remark that Rule (2) can be adapted to some \texttt{VBBkC} based algorithms including \texttt{DDegCol}~\cite{li2020ordering} and \texttt{BitCol}~\cite{yuan2022efficient}, that is, we prune sub-branch $B_i$, if the vertices inside have less than $l-1$ distinct color values.
}\marginpar{R4D6}
% the edge $EH$ satisfies the rule (1) but the vertices in the produced sub-branch, i.e., $F$ and $G$, have only one color value, which violates the rule (2). 
% though rule (2) needs additional time cost $O(|V(g_i)|)$. 


% \begin{enumerate}[leftmargin=*]
%     \item $\min\{col(u), col(v)\}<l-1$ where $e=(u,v)$.
%     \item Vertices in $g_i$ have less than $l-2$ distinct color values. 
% \end{enumerate}
%
% For Rule (1), it is because all vertices in $g_i$ have their color values no larger than $\min\{col(u),col(v)\}$ (since otherwise, assume that $col(u)\geq col(v)$, $id(u)<id(v)$ and there is a vertex $w\in V(g_i)$ such that $col(w)>col(u)$; we have $id(w)<id(u)<id(v)$ based on the definition and $(u,w)\in E(g_i)$ since $u\in S_i$ connects all vertices in $V(g_i)$; we thus derive that edge $(u,w)$ comes before $(u,v)$ in the color-based ordering, which contradicts to the fact that $(u,v)$ comes before every edge in $g_i$). Therefore, vertices in $g_i$ have at most $l-3$ distinct color values smaller than $col(u)$ and thus $g_i$ holds on $l_i$-clique. For Rule (2), the correctness can be easily verified.


\smallskip
\noindent\textbf{The \texttt{EBBkC-C} algorithm.} 
% With the color-based ordering, we design a new algorithm called \texttt{EBBkC-C}. 
{\cheng When the color-based edge ordering is adopted in \texttt{EBBkC}, we call the resulting algorithm \texttt{EBBkC-C}.}
The pseudo-code of \texttt{EBBkC-C} is presented in Algorithm~\ref{alg:EBBkC-C}. {With the color-based edge ordering, a directed acyclic graph (DAG), denoted by $\overrightarrow{G}$, is built for efficiently conducting the branching steps \cite{li2020ordering, yuan2022efficient}. Specifically, $\overrightarrow{G}$ is built upon $G$ by orienting each edge $(u,v)$ in $E$ with $id(u)<id(v)$ 
{\cheng from $u$ to $v$}
% a direction $u\rightarrow v$ 
(line 2). 
{\chengB For illustration, consider Figure~\ref{fig:example2}.}
Given $V_{sub}\subseteq V$, let $N^+(V_{sub},\overrightarrow{g})$ be the common out-neighbours of the vertices in $V_{sub}$ in $\overrightarrow{g}$. Then, given a branch $B=(S,\overrightarrow{g},l)$\footnote{Note that $\overrightarrow{g}$ is a subgraph of $\overrightarrow{G}$, whose edge {\chengB orientations are the same as those} of $\overrightarrow{G}$.}, the edge-oriented branching at a branch with the color-based ordering can be easily conducted by calculating the common out-neighbors of the {\chengB vertices incident to} an edge in $\overrightarrow{g}$ (line 7). Then, we will prune the produced branch if either of the above two 
% conditions is satisfied 
{\cheng rules applies}
(line 8). 
}


% In particular, we prune a branch when either of the above two conditions is satisfied (line 8), and maintain an directed graph, denoted by $\overrightarrow{G}$, for efficiently conducting the branching steps. Specifically, $\overrightarrow{G}$ is built upon $G$ by orienting each edge $(u,v)$ in $E$ with $id(u)<id(v)$ a direction $u\rightarrow v$ (line 2). Besides, given $u\in V$, let $N^+(u,\overrightarrow{G})$ denote the out-neighbours of $u$ in $\overrightarrow{G}$. The edge-oriented branching at a branch with the color-based ordering can be equivalently conducted at line 7, which is adapted from  \cite{danisch2018listing, li2020ordering, yuan2022efficient}. 
% We leave the proof of correctness in the technical report.


\smallskip
\noindent\textbf{Complexity.} The time cost of \texttt{EBBkC-C} is $O(k m  (\Delta/2)^{k-2})$, {\cheng which is worse than that of \texttt{EBBkC-T} (i.e., $O(k m  (\tau/2)^{k-2})$)} though \texttt{EBBkC-C} runs faster in practice. \marginpar{R4O2(3)}

\begin{theorem}
\label{theo:ebbkc-c}
    Given a graph $G=(V,E)$ and an integer $k\geq 3$, the time and {\Revise space complexities of \texttt{EBBkC-C} are} $O(k m  (\Delta/2)^{k-2})$ and {\Revise $O(m+n)$}, respectively, where $\Delta$ is the maximum degree of $G$.
\end{theorem}

\begin{proof}
The proof is similar to that of Theorem~\ref{theo:ebbkc-t}. The difference is that the largest size of the produced graph instance in \texttt{EBBkC-C} can only be bounded by $\Delta$. 
\end{proof}



% \smallskip
% \noindent\textbf{Remark.} The rule (1) (which is conducted on the edge-oriented branching) is adapted from the one (which is conducted on the vertex-oriented branching) proposed in~\cite{li2020ordering}. Besides, the rule (2) is more powerful compared to the rule (1), though rule (2) needs additional time cost $O(|V(g_i)|)$. 
% This means that the rule (2) can be satisfied when the rule (1) does not, which can be easily verified.  


\subsection{\texttt{EBBkC-H}: {\cheng \texttt{EBBkC} with} Hybrid Edge Ordering}
\label{subsec:EBBkC-H}

% We observe that the \texttt{EBBkC-T} and \texttt{EBBkC-C} algorithms can be naturally combined. 
Among \texttt{EBBkC-T} and \texttt{EBBkC-C}, the former has a better theoretical time complexity and the latter enables effective pruning in practice. 
{\Revise
Inspired by the hybrid vertex ordering used for \texttt{DDegCol}~\cite{li2020ordering} and \texttt{BitCol}~\cite{yuan2022efficient}, we aim to achieve the merits of both algorithms by adopting both the truss-based edge ordering (used by \texttt{EBBkC-T}) and the color-based edge ordering (used by \texttt{EBBkC-C}) in the \texttt{EBBkC} framework.}\marginpar{R4D2}
%To achieve the merits of both algorithms, we observe that existing studies of \texttt{VBBkC} \cite{li2020ordering, yuan2022efficient} naturally use \emph{hybrid} vertex orderings at different branching steps to retain both theoretical and practical advantages. For example, \texttt{DDegCol} \cite{li2020ordering} and \texttt{BitCol} \cite{yuan2022efficient} first use degeneracy ordering to branch the universal search space such that the size of each produced problem instance is bounded by the degeneracy $\delta$, then they use color orderings to branch each produced sub-branches. 
%
%Inspired by this idea, we adopt both the truss-based edge ordering (used by \texttt{EBBkC-T}) and the color-based edge ordering (used by \texttt{EBBkC-C}) in the \texttt{EBBkC} framework.
%
%
Specifically, we first apply the truss-based edge ordering for the branching step at the initial branch $(\emptyset,G,k)$. Then, for the following branches, we adopt the color-based ordering for their branching steps. We call this algorithm based on the hybrid edge ordering \texttt{EBBkC-H}. The pseudo-code of \texttt{EBBkC-H} is presented in Algorithm~\ref{alg:EBBkC-H} and the implementations of branching steps are similar to those in \texttt{EBBkC-T} and \texttt{EBBkC-C}. 
% We remark that \texttt{EBBkC-H} inherits the benefits of both \texttt{EBBkC-T} and \texttt{EBBkC-C}. Specifically, 
{\cheng The size of a produced problem instance for \texttt{EBBkC-H} is bounded by $\tau$ (due to the branching at the initial branch based on the truss-based edge ordering),} and thus \texttt{EBBkC-H} achieves the same time complexity as \texttt{EBBkC-T}.
% (as verified in the time complexity analysis part). 
% (as verified below) and run fast in practice due to the color-based pruning rules. 
{\cheng In addition, \texttt{EBBkC-H} enables effective pruning for all branches except for the initial branch (since color-based edge coloring is adopted at these branches), and thus it runs fast in practice as \texttt{EBBkC-C} does.}


\begin{algorithm}[t]
\small
\caption{{\chengB \texttt{EBBkC} with hybrid edge ordering:}
% The edge-oriented BB framework: 
\texttt{EBBkC-H}}
\label{alg:EBBkC-H}
\KwIn{A graph $G=(V,E)$ and an integer $k\geq 3$}
\KwOut{All $k$-cliques within $G$}
\SetKwFunction{List}{\textsf{EBBkC-C\_Rec}}
\SetKwProg{Fn}{Procedure}{}{}
\tcc{Initialization and branching at $(\emptyset,G,k)$}
$\pi_\tau(G)\leftarrow$ the truss-based ordering of edges in $G$\;
\For{each edge $e_i\in E(G)$ following $\pi_\tau(G)$}{
    Obtain $S_i$ and $g_i$ according to Eq.~(\ref{eq:edge-oriented-branching})\;
    % Initialize $V[e_i]\leftarrow V(g_i)$ and $E[e_i]\leftarrow E(g_i)$\;
% }
% \tcc{Edge-oriented branching at $(\emptyset,G,k)$}
% \For{each edge $e$ in $E(G)$}{
    % $S\leftarrow V(e)$ and $g\leftarrow (V[e],E[e])$ according to Eq.~(\ref{eq:edge-oriented-branching})\;
    Do vertex coloring on $g_i$ and get $id(v)$ for each vertex in $V(g_i)$\;
    $\overrightarrow{g_i}\leftarrow(V(g_i),\{u\rightarrow v \mid (u,v)\in E(g_i)  \land id(u)<id(v)\})$\;
    %$\overrightarrow{g}\leftarrow (V(g),\overrightarrow{E}(g))$ where  $\overrightarrow{E}(g)=\{u\rightarrow v \mid (u,v)\in E(g) \text{ \& } id(u)<id(v)\}$\;
    \List{$S_i, \overrightarrow{g_i}, k-2$}\;    
}
\end{algorithm}

\smallskip
\noindent\textbf{Complexity.} The time complexity of \texttt{EBBkC-H} is {\cheng $O(k m  (\tau/2)^{k-2})$, which is} the same as that of \texttt{EBBkC-T}. \marginpar{R4O2(3)}
% , which is 
% also strictly smaller than that of the state-of-the-art, i.e., .

\begin{theorem}
\label{theo:ebbkc-h}
     Given a graph $G=(V,E)$ and an integer $k\geq 3$, the time and {\Revise space complexities of \texttt{EBBkC-H} are} $O(k m  (\tau/2)^{k-2})$ and {\Revise $O(m+n)$}, respectively, where $\tau=\tau(G)$ is strictly smaller than the degeneracy $\delta$ of $G$.
\end{theorem}



\begin{proof}
The proof is similar to that of Theorem~\ref{theo:ebbkc-t}. Since the largest size of the produced graph instance in \texttt{EBBkC-H} can also be bounded by $\tau$, it has the same worst-case time complexity as that of \texttt{EBBkC-T}.
\end{proof}








\subsection{{\Revise Other Potential Applications of \texttt{EBBkC}}}
\label{subsec:discussion}
\marginpar{R3O1\\ R2O1}
{\Revise
Our \texttt{EBBkC} framework can potentially be applied to other problems than the $k$-clique listing problem, which we discuss as follows.
%
\underline{First}, our framework can be easily adapted to solve other clique mining tasks, including maximal clique enumeration (MCE) \cite{eppstein2010listing, naude2016refined, tomita2006worst,jin2022fast}, maximum clique search (MCS) \cite{chang2019efficient, chang2020efficient} and diversified top-$k$ clique search (DCS) \cite{yuan2016diversified, wu2020local}. The rationale is that our framework can explore all possible cliques in an input graph and thus can output only the desired cliques that satisfy some properties (e.g., maximality and diversity) by filtering out others.
%
%Furthermore, with the edge-oriented branch-and-bound framework, it is also possible to improve the theoretical performance. Take the maximal clique enumeration (MCE) as an example. To the best of our knowledge, all existing studies for MCE are based on vertex-oriented branch-and-bound framework. With arbitrary vertex orderings, the well known  Bron–Kerbosch algorithm \cite{bron1973algorithm} (with some carefully designed pivot selection strategies) can enumerate all maximal cliques in a $n$-vertex graph in $O^*(3^{n/3})$ time \cite{tomita2006worst}, where $O^*$ suppresses the polynomials. If the degeneracy ordering is applied to branch the universal search space, the time complexity can be improved to the state-of-the-art $O^*(3^{\delta/3})$ \cite{bello2016neural, eppstein2010listing}, where $\delta$ is the degeneracy of the graph. The reason is that each produced sub-branch after branching at the initial step contains at most $\delta$ vertices. However, if the edge-oriented branch-and-bound framework is applied, specifically with truss-based edge ordering, the time complexity can be further improved to $O^*(3^{\tau/3})$, where $\tau$ has the same definition as that in Eq.~(\ref{eq:tau}) and $\tau<\delta$ theoretically. 
%
\underline{Second}, our framework can be potentially extended to mining other types of \textit{connected} dense subgraphs, e.g., connected $k$-plex. This is because our framework can be used to explore all possible subsets of edges by recursively including an edge, and thus the induced subgraphs will cover all possible connected dense subgraphs.
%
\underline{Third}, there are some potential benefits when adapting our framework to the above tasks. As discussed in Section~\ref{subsec:motivation}, the edge-oriented branching can provide more information (i.e., an edge involving two vertices instead of one vertex) towards designing more effective pivot techniques and/or pruning rules than the existing vertex-oriented branching.


}


==> cover-letter/R1.tex <==
% \newpage

\section*{Comments and Suggestions from Review \#1}



O1. \textit{There are three main techniques in improving the practical efficiency of maximal clique enumeration: (1) use edge-oriented branching at the out-most level, (2) early termination, and (3) graph reduction. The first two are proposed in this paper, while the last one was proposed in [15]. In the experiments, the authors demonstrated the efficiency of the second and third techniques but didn’t fairly evaluate the first technique. Specifically, although the authors evaluated \texttt{HBBMC++} against the existing implementations and their variants in Tables II and IV, it is better to also evaluate \texttt{HBBMC++} against its own variant that does not use the first technique (i.e., edge-oriented branching at the out-most level); this will eliminate biased caused by different implementation details.}


\vspace{1mm}
\textbf{Response:}
{As suggested, we evaluate our}  \texttt{HBBMC++} against three variants. {\yuic We remark that all of them} use the same implementation for the second and the third technique. They only differ in {\yuic the} branching strategies adopted {\yuic at} the initial branch. The details  are as follows. 
\begin{itemize}[leftmargin=*]
    \item \texttt{VBBMC-dgn} uses the vertex-oriented branching strategy {\yuic with the degeneracy vertex ordering at} the initial branch. %The vertex ordering is defined as the degeneracy ordering. 
    
    \item \texttt{HBBMC-dgn} uses edge-oriented branching strategy {\yuic with the \emph{alphabetical} edge ordering at} the initial branch. {\yuic Here, the alphabetical edge ordering is defined as follows. Given the degeneracy odering $\langle v_1,v_2,...,v_n\rangle$ as well as two different edges $e=(v_i,v_j)$ and $e'=(v_{i'},v_{j'})$ such that $1\leq i<j\leq n$ and $1\leq i'<j'\leq n$, one edge $e$ comes before the other $e'$ in the alphabetical edge ordering iff (1) $i<i'$ or (2) $i=i'$ and $j<j'$.}
    
    %The edge ordering is defined in three steps. First, we obtain the degeneracy ordering of the vertices $\langle v_1, v_2, \cdots v_n \rangle$, and for each $u\in V$, let $id(u)$ be the position of a vertex $u$ in the ordering. Second, for each edge $e=(u,v)\in E$ with $id(u)<id(v)$, we define $str(e)$ as a string, which is the concatenation of $id(u)$ and $id(v)$ (i.e., $str(e)=$`$id(u)$+$id(v)$'). Finally, we define the edge ordering as the alphabetical ordering based on $str(e)$ for edges $e\in E$.  That is, one edge $e = (u,v)$ with $id(u)<id(v)$ comes before another edge $e' = (u', v')$ with $id(u')<id(v')$ if (1) $id(u)<id(u')$ or (2) $id(u)=id(u')$ and $id(v)<id(v')$. 
    
    \item \texttt{HBBMC-mdg} uses edge-oriented branching strategy {\yuic with the \emph{non-decreasing} edge ordering at} the initial branch. {\yuic Here, the edge ordering is defined as follows. For an edge $e=(u,v)$, let $ub(e)=\min\{d(u, G), d(v, G)\}$, which is the upper bound of the size of the candidate graph of the sub-branch produced upon the edge $e$. One edge $e$ comes before another $e'$ in the non-decreasing edge ordering iff $ub(e)\le ub(e')$.}
    
    %First, for each edge $e=(u,v)\in E$, we define $ub(e)=\min\{d(u, G), d(v, G)\}$, which is the upper bound of the size of the candidate graph of the sub-branch produced upon the edge $e$. Second, we define the edge ordering as the non-decreasing ordering based on $ub(e)$ for edges $e\in E$. That is, one edge $e$ comes before another edge $e'$ if $ub(e)\le ub(e')$. 
\end{itemize}






{We report the results} in Table~\ref{tab:revise1}. {\yuic We have the following observations. \underline{First},} \texttt{HBBMC++} {\yuic (with the proposed hybrid branching)} outperforms \texttt{VBBMC-dgn} {\yuic (with the existing vertex-oriented branching)} across all datasets, with significant improvements particularly on larger datasets. {\yuic This demonstrates the superiority of the porposed hybrid branching, particularly the edge-oriented branching, and is well aligned with the theoritical results in Theorem~\ref{theo:hbbmc}. \underline{Second}, \texttt{HBBMC++} consistently outperforms both \texttt{HBBMC-dgn} and \texttt{HBBMC-mdg}, which verifies} the {\yuic effectiveness} of truss-based edge ordering {\yuic towards} reducing computational overhead. {\yuic We remark that, without adopting the truss-based edge ordering, \texttt{HBBMC-dgn} and \texttt{HBBMC-mdg} cannot acheive the same time complexity as \texttt{HBBMC++} does.}
%
%Compare {\yuic with} \texttt{VBBMC-dgn}, \texttt{HBBMC++} consistently achieves better performance due to the use of truss-based edge ordering, which is obtained through a greedy procedure that iteratively removes the edge whose vertices have the smallest number of common neighbors. It effectively reduces the size of intermediate graph instances due to the fact $\tau < \delta$, thereby decreasing the search space and computation time. The results show that \texttt{HBBMC++} outperforms \texttt{VBBMC-dgn} across all datasets, with significant improvements particularly on larger datasets.
%
%Compare \texttt{HBBMC++} with \texttt{HBBMC-dgn} and \texttt{HBBMC-mdg}, they all use the edge-oriented branching strategy but differ in what edge ordering is applied. The results demonstrate that \texttt{HBBMC++} consistently outperforms both \texttt{HBBMC-dgn} and \texttt{HBBMC-mdg}, illustrating the efficiency of truss-based edge ordering in reducing computational overhead. This also highlights the effectiveness of truss-based edge ordering in focusing the branching process on more promising edges, resulting in fewer redundant computations and improved performance.


% For each edge $e=(u,v)\in E(g)$ with $id(u)<id(v)$, we define $str(e)$ as a string, which is the concatenation of $id(u)$ and $id(v)$ (i.e., $str(e)=$`$id(u)$+$id(v)$'). Finally, we define the color-based edge ordering as the alphabetical ordering based on $str(e)$ for edges $e\in E(g)$.  That is, one edge $e = (u,v)$ with $id(u)<id(v)$ comes before another edge $e' = (u', v')$ with $id(u')<id(v')$ if (1) $id(u)<id(u')$ or (2) $id(u)=id(u')$ and $id(v)<id(v')$.





\vspace{2mm}
O2. \textit{The time complexity proof for Theorem 2 is too brief and does not seem correct to me. Firstly, the second line of Equation (5) should also include the time of getting the subgraphs. Secondly, it is unclear how the recurrence is solved to get the final time complexity.}


\vspace{1mm}
\textbf{Response:}
We have included more details of the proof in the revised manuscript (Theorem 2). We also summarize some of the details as follows. 


\underline{First}, the time of getting the subgraphs can also be bounded by $O(m \delta)$, where $m$ is the number of edges and $\delta$ is the degeneracy of the graph, respectively. The reason is as follows. First, for all edges $e=(u,v)\in E$, we can compute the set of common neighbors of $u$ and $v$ (i.e., $N(V(e), G)$ for $e\in E$) in $O(m\delta)$ time by any existing triangle listing algorithm, such as \cite{hu2014efficient,chu2011triangle,latapy2008main}. Second, consider an edge $e=(u,v)\in E$. For each $w\in N(V(e), G)$, $w\in V(g_C)$ if both edge $(u, w)$ and edge $(v, w)$ are ordered after $e$; otherwise, $w\in V(g_X)$. This process can also be done in $O(m\delta)$. To see this, we note that $u$, $v$ and $w$ always form a triangle (i.e., 3-clique), indicating that the time cost for getting all subgraphs for the sub-branches is proportional to the number of triangles in $G$. According to the existing triangle listing algorithms \cite{hu2014efficient,chu2011triangle,latapy2008main}, given a graph with its degeneracy number equal to $\delta$, the number of triangles inside is bounded by $O(m\delta)$. With $V(g_C)$ and $V(g_X)$, it is sufficient to recursively conduct the vertex-oriented branching strategy for the remaining branches. 



\underline{Second}, we analyze the time costs for the recursive process. 
% We first show two lemmas that is necessary for the proof. 
% \begin{lemma}[Theorem 3 of \cite{tomita2006worst}] 
% Let $F(n)$ be a function which satisfies the following recurrence relation
% \begin{equation}
%     F(n)\le\left\{
% \begin{array}{lr}
%     \max_{k} \{k\cdot F(n-k)\} + O(n^2) & \quad \text{if } n > 0 \\
%      O(1) & \quad \text{if } n=0
% \end{array}
%     \right.
% \end{equation}
% where $n$ and $k$ are positive integers. Then $F(n) = O(3^{n/3})$.
% \end{lemma}
% \begin{lemma}
%     Given a graph $G=(V, E)$ with its truss number equal to $\tau$. The number of triangles in $G$ is no more than $m\tau$. 
% \end{lemma}
% \begin{proof}
%     Let $\pi_{\tau}=\langle e_1, e_2, \cdots, e_m \rangle$ be the truss-based edge ordering and $sup(e_i)$ be the number of common neighbors in the subgraph induced by $\{e_i, e_{i+1}, \cdots, e_m\}$. Then, the number of triangles in $G$, denoted by $N$, is bounded by
%     \begin{equation}
%         N =\sum_{i=1}^m sup(e_i) \le \sum_{i=1}^m \tau =m\tau
%     \end{equation}
%     The first equation follows from the fact that each triangle is uniquely associated with the earliest edge in the truss-based ordering of its three constituent edges. The inequality follows from the definition of $\tau$. 
% \end{proof}
% Now, we are ready for the analysis. 
Consider a branch $B=(S,g_C,g_X)$ produced after the edge-oriented branching strategy. {\chengC Let} $T(c,x)$ be the time complexity of solving $B$ with $c=|V(g_C)|$ and $x=|V(g_X)|$. 
The time cost consists of three components. First, it would take $O(c\cdot (c+x))$ {\chengC time} to choose the pivot by checking each vertex in $V(g_C)\cup V(g_X)$ to identify the number of its neighbors in $g_C$. Second, assume that the pivot is $v^*$ and $v^*$ has $k$ ($k\le c$) non-neighbors in $g_C$ (denoted by $u_1, \cdots, u_k$), on which the sub-branches are produced. Correspondingly, for each sub-branch produced on $u_i$, it would take $O(c+x)$ {\chengC time} to identify $u_i$'s neighbors in $g_C$ and $g_X$. In total, it would take $O(k\cdot (c+x))$ {\cheng time} 
% in total 
to construct $k$ sub-branches. Third, since $v^*$ is a pivot that has the maximum number of neighbors in $g_C$, i.e., $c-k$ neighbors, for each $u_i\in V(g_C)$, they all have at most $c - k$ neighbors in $g_C$. Thus, we have the following recurrence 
\begin{equation}
\begin{aligned}
    T(c,x) &\le \max_k \{k \cdot T(c-k,x)\} + \lambda \cdot c\cdot (c+x) \\
    % &=(c+x) \cdot \Big( \max_k \{k \cdot \frac{T(c-k,x)}{c+x}\} + \lambda \cdot c \Big) \\
    % &\le (c+x) \cdot \Big( \max_k \{k \cdot \frac{T(c-k,x)}{c-k+x}\} + \lambda \cdot c^2 \Big) \\
\end{aligned}
\end{equation}
% The first inequality follows by summing up the three components of the time cost, where $\lambda>0$ is a constant. The equality follows by extracting $(c+x)$. To see the third inequality, we first have $\lambda\cdot c\le \lambda \cdot c^2$ since $c\ge 1$. Then, let $k^*$ be value of $k$ such that $k \cdot \frac{T(c-k,x)}{c+x}$ reaches the maximum. We have 
% \begin{equation}
% \begin{aligned}
%     \max_k \{k \cdot \frac{T(c-k,x)}{c+x}\} &= k^* \cdot \frac{T(c-k^*,x)}{c+x} \\
%     &\le k^* \cdot \frac{T(c-k^*,x)}{c-k^*+x} \\
%     &\le  \max_k \{k \cdot \frac{T(c-k,x)}{c-k+x}\}
% \end{aligned}
% \end{equation}
% Let $f(c)=T(c,x)/(c+x)$, we have 
% \begin{equation}
%     f(c)\le \max_k \{k \cdot f(c-k)\} + \lambda \cdot c^2
% \end{equation}
where $\lambda$ is a constant. We solve this recurrence with an additional lemma (see Lemma~\ref{lemma:1} in Section~\ref{subsec:HBBMC}), $T(c,x)\le\lambda'\cdot(c+x)\cdot 3^{c/3}$, where $\lambda'>0$ is also a constant. 
% Therefore, $T(c,x)=\lambda'\cdot(c+x)\cdot 3^{c/3}$. 
To compute the total time complexity, {\chengC we have}
\begin{equation}
\begin{aligned}
    \sum_{e\in E} T(c_e, x_e) &=\sum_{e\in E} \lambda' \cdot (c_e + x_e) \cdot 3^{c_e/3}\\
    &\le \lambda' \cdot 3^{\tau/3} \cdot \sum_{e\in E} (c_e + x_e) \le \lambda'  \cdot 3^{\tau/3} \cdot 3m\tau
\end{aligned}
\end{equation}
The first inequality follows from the fact that $c_e\le \tau$ based on the definition of $\tau$. The second inequality follows from the facts that (1) for an edge $e$, $(c_e+x_e)$ is the number of triangles associated with $e$, and (2) the total number of triangles is no larger than $m\tau$ (see Lemma~\ref{lemma:2} in Section~\ref{subsec:HBBMC}). In summary the total time cost of \texttt{HBBMC} is $O(m \delta + m \tau \cdot 3^{\tau/3})$. 

% After we obtain $m$ subgraphs via the edge-oriented branching strategy, we analyze the total time cost $T$ for the recursive process. Let $T(n)$ be the total number of sub-branches that would be produced from a branch $B=(S,g_C,g_X)$ with $n=|V(g_C)|$. We have 
% \begin{equation}
%     T\le \sum_{e\in E} \tau \cdot T(\tau)
% \end{equation}
% The rationale is in twofold. First, for each produced sub-branch via the edge-oriented branching strategy with truss-based edge ordering, $|V(g_C)|\le \tau$. Therefore, for each sub-branch produced from the initial branch, it would further produce at most $T(\tau)$ branches. Second, we notice that the recursive process forms a search tree with each branch being a tree node. At each leaf node of the search tree (where $g_C$ being an empty graph), the algorithm would take at most $O(\tau)$ time to output a maximal clique. 

% To solve the above formula, let $u$ be a pivot vertex in the branch $B$. Assume that $u$ has $k$ non-neighbors in $g_C$, on which the sub-branches are produced. Correspondingly, $u$ has $n-k$ neighbors in $g_C$. Since $u$ is a pivot that has the maximum number of neighbors in $g_C$, for any vertex $v\in V(g_C)$, they all have at most $n - k$ neighbors in $g_C$. Thus, we have the following recurrence $T(n)\le k \cdot T(n-k)$. 
% %
% As proved in \cite{kratsch2010exact}, given a linear recursion function of $F(n)\le\sum_{i=1}^{j} F(n-a_i)$, $F(n)$ can be bounded by $O(\gamma^n)$, where $\gamma$ is the largest positive real root of the equation $x^n - \sum_{i=1}^{j} x^{n-a_i}=0$. By setting different values of $k$, the largest positive real root of $x^n-k\cdot x^{n-k}=0$ reaches the maximum when $k=3$. Thus, we have $T(n)\le 3^{n/3}$, which further indicates that $T$ is bounded by $O(m\tau \cdot 3^{\tau/3})$. 
%




% By solving the recurrence, we obtain the time complexity of \texttt{HBBMC}, {\cheng which} is $O(\delta m + \tau m \cdot 3^{\tau/3})$. 




% Let $T(n)$ be the total time cost to enumerate all maximal cliques within a branch $B=(S, g_C, g_X)$, where $|V(g_C)|=n$. We have the following recurrence. 
% \begin{equation}
% \label{eq:hbbmc}
% T(n) \le \left\{
% \begin{array}{lr}
%     O(\tau) & g_C = G[\emptyset]\\ 
%     O(\delta m) + \sum_{e\in E} T(\tau) &  g_C = G \\ 
%     \max_k \{k\cdot T(n - k)\} + O(m) & g_C\neq G, G[\emptyset] \\
% \end{array}
% \right.
% \end{equation}

% %
% \underline{Second}, 

\vspace{2mm}
O3. \textit{The experiments use ER random graphs, which typically do not contain large cliques. It is better to also use power-law random graphs in the experiments.}

\vspace{1mm}
\textbf{Response:} {\yuic We have conducted additional experiments on power-law random graphs generated by using the Barab\'{a}si–Albert (BA) model~\cite{albert2002statistical}. In specific, the BA model receives two parameters, namely the number of vertices $n$ and the edge density $\rho$, which are set as} 1M and 20 by default. {\yuic We compare our \texttt{HBBkC++} with all baselines on different power-law random graphs by varying $n$ (from 100K to 10M) and $\rho$ (from 5 to 40), and report the running time in {\chengC Figure~\ref{fig:scale-ba} and \ref{fig:density-ba}}, respectively. We observe that our \texttt{HBBkC++} performs the best among all baselines.} More detailed results and analysis are presented in {\chengC Appendix~\ref{subsec:syn-result} of the technical report~\cite{TR}}.

%We followed the suggestion by generating a series of power-law random graphs using the Barab\'{a}si–Albert (BA) model. The BA model is a popular algorithm for generating scale-free networks that follow a power-law degree distribution. In this model, nodes are added to the network one at a time, and each new node is connected to a set number of existing nodes based on preferential attachment. This means that nodes with a higher degree (i.e., those that are already well-connected) are more likely to receive new links, mimicking the “rich get richer” phenomenon observed in many real-world networks, including those we used in real datasets. For parameter settings, we set the number of vertices $n$ and the edge density $\rho$ as 1M and 20 by default, and vary them in the range $n\in$ \{100K, 500K, 1M, 5M, 10M\} and $\rho\in$ \{5, 10, 20, 30, 40\}, respectively. The running time results indicate that our algorithm achieves the best performance among all baselines. More detailed results and analysis are presented in Section~\ref{subsec:syn-result}.
 


\vspace{2mm}
O4. \textit{In the experiments, it mentions that it is not fair to compare \texttt{HBBMC} with \texttt{RRcd} which does not apply the classic pivot selection. According to Tables II and IV, \texttt{RRcd} and \texttt{Rcd++} actually perform very well in practice. It is better to add more discussions on the efficiency of \texttt{RRcd} and \texttt{Rcd++}.} 


\vspace{1mm}
\textbf{Response:}
\texttt{RRcd} \cite{deng2023accelerating} is one of the BK-based algorithms, following {\chengC the} \texttt{BK\_Rcd} framework.
The main difference between \texttt{BK\_Rcd} and other BK-based algorithms (e.g., \texttt{BK\_Degen}) is that \texttt{BK\_Rcd} adopts a \emph{top-to-down} approach that starts from a subgraph and iteratively removes vertices until the subgraph becomes a clique, while other algorithms, in essence, adopt a \emph{bottom-to-up} approach that starts from an individual vertex, adds only one vertex into the result set with one independent recursive call, and discovers a maximal clique utill all its vertices are added into the result set.
When $g_C$ is already a clique or a near-clique (e.g., a clique with only a few edges missing), \texttt{BK\_Rcd} would create less branches than that of \texttt{BK\_Degen}. 
This would help explain why \texttt{BK\_Rcd} sometimes performs better than \texttt{BK\_Degen} in practice. {\chengC We have included the explanation in Part (1) of Section~\ref{subsec:real-result}.}

==> cover-letter/R2.tex <==
\section*{Comments and Suggestions from Review \#2}




O1. \textit{I notice that in the discussion of \texttt{EBBMC}, the authors mention that the ordering of the edges can have an impact. In \texttt{EBBMC}, the authors choose truss-based edge ordering. I would like to know how much effect truss-based edge ordering has. Could you show the results without using the truss-based edge ordering in the ablation experiments?}


\vspace{1mm}
\textbf{Response:}
{\yuic Thanks for your comments. In the revision, we have studied the {\chengC effects} of the ordering of the edges on \texttt{EBBMC} by comparing our \texttt{HBBMC++} with two variants, namely \texttt{HBBMC-dgn}: \texttt{HBBMC++} using the alphabetical edge ordering and \texttt{HBBMC-mdg}: \texttt{HBBMC++} using the non-decreasing edge ordering. {\chengC For details, please} refer to our responses to \#R1O1 or Section~\ref{subsec:real-result} in the revision.}

%We followed the suggestion by evaluating \texttt{HBBMC++} against three variants. \texttt{HBBMC++} and these three variants all use the same implementation for the second and the third technique. They only differ in what branching strategy is adopted for branching the initial branch. The details of the baselines are as follows. 
%\begin{itemize}[leftmargin=*]
%    \item \texttt{VBBMC-dgn} uses the vertex-oriented branching strategy for branching the initial branch. The vertex ordering is defined as the degeneracy ordering. 
    
%    \item \texttt{HBBMC-dgn} uses edge-oriented branching strategy for branching the initial branch. The edge ordering is defined in three steps. First, we obtain the degeneracy ordering of the vertices $\langle v_1, v_2, \cdots v_n \rangle$, and for each $u\in V$, let $id(u)$ be the position of a vertex $u$ in the ordering. Second, for each edge $e=(u,v)\in E$ with $id(u)<id(v)$, we define $str(e)$ as a string, which is the concatenation of $id(u)$ and $id(v)$ (i.e., $str(e)=$`$id(u)$+$id(v)$'). Finally, we define the edge ordering as the alphabetical ordering based on $str(e)$ for edges $e\in E$.  That is, one edge $e = (u,v)$ with $id(u)<id(v)$ comes before another edge $e' = (u', v')$ with $id(u')<id(v')$ if (1) $id(u)<id(u')$ or (2) $id(u)=id(u')$ and $id(v)<id(v')$. 
    
 %   \item \texttt{HBBMC-mdg} uses edge-oriented branching strategy for branching the initial branch. The edge ordering is defined in two steps. First, for each edge $e=(u,v)\in E$, we define $ub(e)=\min\{d(u, G), d(v, G)\}$, which is the upper bound of the size of the candidate graph of the sub-branch produced upon the edge $e$. Second, we define the edge ordering as the non-decreasing ordering based on $ub(e)$ for edges $e\in E$. That is, one edge $e$ comes before another edge $e'$ if $ub(e)\le ub(e')$. 
%\end{itemize}

%The results are presented in Table~\ref{tab:revise1}. Compare \texttt{HBBMC++} with \texttt{VBBMC-dgn}. \texttt{HBBMC++} consistently achieves better performance due to the use of truss-based edge ordering, which is obtained through a greedy procedure that iteratively removes the edge whose vertices have the smallest number of common neighbors. It effectively reduces the size of intermediate graph instances due to the fact $\tau < \delta$, thereby decreasing the search space and computation time. The results show that \texttt{HBBMC++} outperforms \texttt{VBBMC-dgn} across all datasets, with significant improvements particularly on larger datasets.
%
%Compare \texttt{HBBMC++} with \texttt{HBBMC-dgn} and \texttt{HBBMC-mdg}, they all use the edge-oriented branching strategy but differ in what edge ordering is applied. The results demonstrate that \texttt{HBBMC++} consistently outperforms both \texttt{HBBMC-dgn} and \texttt{HBBMC-mdg}, illustrating the efficiency of truss-based edge ordering in reducing computational overhead. This also highlights the effectiveness of truss-based edge ordering in focusing the branching process on more promising edges, resulting in fewer redundant computations and improved performance.



\vspace{2mm}
O2. \textit{The hybrid strategy in \texttt{HBBMC} involves using \texttt{EBBMC} only at the initial branches. I'm curious whether the authors explore other hybrid strategies. For example, how about using edge pivot in more branches?}


\vspace{1mm}
\textbf{Response:} Thanks for your comment. We followed the suggestion to explore alternative hybrid strategies by investigating the use of the edge-oriented branching strategy at varying depths within the recursion tree. Specifically, we applied the edge-oriented branching strategy at the early stages of the tree, up to a depth threshold $d$, beyond which we switched to the pivot-based vertex-oriented branching strategy. By varying $d$ within the range $\{1,2,3\}$, we aimed to identify the optimal balance between the effectiveness of edge-oriented branching and the more granular control provided by vertex-oriented branching at deeper levels. We note that the case $d=1$ corresponds to the branching strategy employed in \texttt{HBBMC++}. Table \ref{tab:hybrid} shows that increasing $d$ typically results in more branching calls and longer runtimes, due to the lack of pivot-based pruning in edge-oriented branching. However, edge-oriented branching is still effective for rapid pruning at the initial stages, and adjusting $d$ allows us to fine-tune when to leverage the strengths of each strategy. The results suggest that carefully choosing the threshold $d$ (i.e., $d=1$) is crucial for optimizing the performance of the hybrid framework, ensuring that the transition between branching strategies is both timely and effective.


\vspace{2mm}
O3. \textit{The early termination technique proposed by the authors applies only when the candidate set in the current branch forms a 2-plex or 3-plex. However, the paper does not provide details on how to detect whether the candidate set is a 2-plex or 3-plex, nor does it analyze the overhead of this process. I would like to know whether the overhead of detecting whether the candidate set is a 2-plex or 3-plex is acceptable, especially when the early termination technique is used frequently.}

\vspace{1mm}
\textbf{Response:}
{\yuic We first clarify that the procedure of detecting whether the candidate set is a 2-plex or 3-plex takes additional $O(|V(g_C)|)$ time at each branch, which is efficient in both theory and practice. We have included the following detailed analysis in Section~\ref{subsec:3-plex}. 
We remark that, for each vertex $v\in V(g_C)\cup V(g_X)$, \texttt{HBBMC} maintains the degree of $v$ in $g_C$, i.e., $d(v, g_C)$, for selecting the pivot. Clearly, $g_C$ is a $k$-plex iff the vertex with the smallest degree in $g_C$ has its degree at least $|V(g_C)|-k$. Hence, we can check whether $g_C$ is a $k$-plex by selecting the vertex with the smallest degree in $g_C$, which takes extra $O(|V(g_C)|)$ time.}

%Recall that in \texttt{HBBMC} framework, we apply the pivoting strategy to pruned the branches that do not hold any maximal cliques: given a branch $B=(S,g_C,g_X)$, the pivoting strategy calculates for each vertex $v\in V(g_C)\cup V(g_X)$ the number of neighbors in $g_C$, i.e., $d(v, g_C)$, and chooses the vertex $v^*\in V(g_C)\cup V(g_X)$ with the maximum value $d(\cdot, g_C)$ as the pivot.
%The condition that whether $g_C$ is a 2-plex (resp. 3-plex) can be done simultaneously when we choose the pivot vertex. Specifically, we can identify $g_C$ is a 2-plex (resp. 3-plex) if the minimum value of $d(\cdot, g_C)$ for a vertex in $V(g_C)$ is no less than $|V(g_C)|-2$ (resp. $|V(g_C)|-3$). The rationale is as follows. Let $u_m\in V(g_C)$ be the vertex with the minimum value of $d(\cdot, g_C)$. Then for any vertex $u\in V(g_C)$, we have $d(u, g_C)\ge d(u_m, g_C)\ge |V(g_C)|-2$ (resp. $|V(g_C)|-3$), indicating that $g_C$ is a 2-plex (resp. 3-plex). The above procedure only takes additional $O(|V(g_C)|)$ time at each branch to find $u_m$. We believe the overhead is acceptable. 


==> cover-letter/R3.tex <==

\section*{Comments and Suggestions from Review \#3}




O1. \textit{The paper seems incremental, making relatively small optimizations in an area that seems already rich with contributions. Maybe in the graph data mining community readers can be more enthusiastic about this kind of work. In the ICDE community, it's a bit harder to be very interested in the problem.}


\vspace{1mm}
\textbf{Response:}
We appreciate the reviewer's comment and would like to clarify (1) the significance of the maximal clique enumeration (MCE) problem and (2) our contributions.

\underline{First}, the maximal clique enumeration (MCE) problem is a fundamental but challenging task, with its worst-case time complexity {\chengC increasing} exponentially with input size. Its importance remains high due to its extensive applicability across various real-world domains, such as fraud detection, community search in social networks, topic extraction from document collections, and biological network analysis,
% These diverse applications underscore the continued relevance of research in this area. 
% The inherent computational difficulty and real-world impact of MCE reinforce its significance across multiple domains, 
making it as a central problem for both theoretical and applied research within the ICDE and broader database communities (e.g., {\chengC many papers on this problem have been published at SIGMOD and VLDB~\cite{deng2023accelerating, dai2022fast, blanuvsa2020manycore, pan2022fairness, zhang2019efficient, li2021finding, sun2017mining}}). 
% Consequently, the development of novel techniques and their extensions in different applications within these communities \cite{deng2023accelerating, dai2022fast, blanuvsa2020manycore, pan2022fairness, zhang2019efficient, li2021finding, sun2017mining} remain crucial. 
As real-world graphs grow increasingly complex, enhancing MCE algorithms to improve scalability and applicability to larger datasets constitutes an essential contribution, closely aligned with the ICDE community's commitment to advancing methods for managing intricate data environments.



\underline{Second}, our work introduces advancements over existing studies, both theoretically and practically. Theoretically, we propose the \texttt{HBBMC} algorithm, which integrates vertex-oriented and edge-oriented branching strategies, where the latter is newly introduced in this paper, offering better asymptotic performance on many real-world graphs. Furthermore, our early termination technique boosts practical performance by directly constructing maximal cliques in dense subgraphs, reducing computation time in these cases. In extensive experiments on real and synthetic datasets, our method achieves up to 4x faster results compared to the best existing algorithms, demonstrating its clear advantage in both efficiency and scalability. These improvements make our approach highly relevant for practical applications involving large and complex graphs. 


% In summary, our contributions extend beyond marginal improvements, offering significant theoretical advancements and practical performance gains that could provide valuable insights and inspiration to the ICDE and database communities.

% \begin{enumerate}[leftmargin=*]
    % \item \textbf{A Fundamental and Hard Problem.} 
    % The maximal clique enumeration problem is a fundamental and notoriously hard computational problem, with its worst-case time complexity growing exponentially wrt the size of the input. The problem also remains critical due to its broad applicability in numerous real-world scenarios and practical applications, such as fraud detection, community search in social networks, mining document collections for topic extraction, and biological network analysis. These diverse use cases reinforce the relevance of continuing research in this area. The inherent computational difficulty, combined with its real-world significance, ensures that any advancements can have a profound impact across multiple domains, making this a key problem for both theory and application in the ICDE and broader research communities.
    
    % The maximal clique enumeration problem is indeed a fundamental and notoriously hard computational problem. Its worse-case time complexity is exponential with respect to the size of the input, making it a challenging area even after decades of research. The intractable nature of the problem means that any improvements, especially those that significantly impact practical computation times, can have meaningful contributions. This is because each improvement potentially broadens the range of datasets and real-world applications where these algorithms become computationally feasible.

    % \item \textbf{Efficiency as a Core Goal.} In the context of the database and ICDE community, efficiency has always been a primary objective due to the inherent complexity of the maximal clique enumeration problem. Although various techniques have been proposed over the years, the need for continued innovation remains. As real-world graphs become more intricate, making such algorithms scalable and applicable to larger datasets is a crucial contribution that aligns with the core interests of the ICDE community. Thus, further efficiency improvements in this domain are essential and highly relevant to advancing the community's ability to handle increasingly complex data environments.

    % \item \textbf{Our Techniques Are Not Incremental.} 
    
% \end{enumerate}



% The proposed techniques bring unique contributions to the problem that distinguish them from previous works. Specifically, our approach leverages [specific techniques/methods], which have not been employed in this context before. These innovations result in a measurable improvement in both theoretical and empirical performance, pushing the boundaries of what has previously been achieved. Moreover, our comprehensive evaluation on real-world datasets demonstrates that the proposed techniques can handle graph structures that were previously intractable with existing algorithms, 
% Non-Incremental Contribution of Our Work: Contrary to the reviewer’s perception, our proposed methods are not mere incremental optimizations. We introduce [briefly describe the core techniques], which, to the best of our knowledge, have not been applied in the MCE context before. These techniques significantly reduce runtime compared to existing methods (as shown in our experiments on both real-world and synthetic datasets). Our results demonstrate the clear impact of our contributions on scaling MCE for large graphs, marking a meaningful advance in the state-of-the-art.



\vspace{2mm}
O2. \textit{The experimental evaluation leaves are hard to interpret for what concerns the real datasets. We do not know what they are; they are characterized by 2 letters each. Further, the authors edited the datasets a bit: removed labels, edge directions, and self-loops (I don't know why the self-loops?) What I am missing is: how is this result of clique search on these datasets, relevant or interesting?
E.g., say that one dataset is about DBLP publications: there are People nodes, Conference Nodes and Paper nodes, people publish papers, papers appear in conferences, people also chair conferences. What does it mean for three nodes to be all connected, in such a setting? How interesting is this query? Can we ask it with SQL or another graph query language?}


\vspace{1mm}
\textbf{Response:} 
We shall clarify (1) the interpretation of the datasets and the results, (2) how we can use the enumeration results in real application scenarios and (3) whether the problem can be translated into SQL or graph query language to resolve the reviewer's concern. 


\underline{First}, we incorporated additional dataset descriptions as suggested, presenting each dataset’s full name, abbreviation, and category in Table~\ref{tab:data}. Following the existing studies \cite{deng2023accelerating, li2019fast}, we prepared the datasets such that each graph is undirected and unweighted. In some datasets, particularly social networks, self-loops are present due to user self-interactions, such as liking one's own posts. We removed self-loops, as they do not contribute meaningful information to maximal clique identification and can lead to redundant computations, which is consistent with prior studies. Additionally, our approach is naturally extendable to directed or weighted graphs. By first extracting all maximal cliques without regard to direction or weight, we can subsequently filter cliques to include only those satisfying user-defined directional or weighted conditions.




\underline{Second}, maximal clique enumeration finds diverse applications across various domains. In most cases, the graph is homogeneous, meaning all vertices are of the same type, and the relationships between vertices are uniform. For example, in the DBLP dataset, as mentioned by the reviewer, vertices exclusively represent researchers, and edges denote co-authorship between two individuals who have collaborated on at least one publication. In this context, maximal cliques reveal tightly connected research groups or frequent collaborators.

While many applications involve vertices representing individuals (e.g., in social or collaboration networks), where maximal cliques correspond to groups of people with shared interests, there are several other scenarios where vertices have different meanings. One notable application is in frequent itemset mining \cite{kumar2012logical}. In this context, transaction data is transformed to a graph where each product is represented by a vertex, and edges connect vertices when the corresponding products are frequently purchased together, based on a user-defined transaction frequency threshold. A maximal clique in this graph identifies groups of products that are commonly co-purchased, providing insights for product bundling, inventory management, and targeted marketing strategies.
%
% The other significant application is in computational biology, where maximal clique enumeration is extensively used to analyze large protein-protein interaction (PPI) networks in microarray experiments \cite{abu2005relative, yang2014protein}. In these networks, proteins or genes are represented as vertices, with edges indicating interactions or regulatory relationships between them. Identifying maximal cliques in these graphs helps uncover groups of densely interacting proteins or co-regulated genes, which often correspond to protein complexes playing critical roles in cellular processes such as signal transduction and metabolism. These cliques provide biologically significant insights into cellular functions and aid in identifying molecular targets for drug discovery.
{\chengC Since the maximal clique enumeration (MCE) problem has been studied extensively and its applications have been elaborated sufficiently and well recognized in prior studies, we decide not to restate its applications as explained above in detail in this paper.}


\underline{Third}, languages like SQL or GraphSQL (e.g., those designed by Neo4j or GraphScope) do not natively support maximal clique enumeration due to the complexity of the problem. They are typically designed for graph queries that could finish in polynomial time, such as finding shortest paths, strong connected components or simple comminuties like $k$-cores. To address this limitation, businesses can integrate specialized graph libraries or algorithms for maximal clique detection into their database systems, potentially through user-defined functions or custom extensions, enabling seamless analysis of large datasets within their existing infrastructure.


% \underline{Second}, maximal clique enumeration has diverse applications across various domains. However, the graph is generally homogeneous, which indicates that all vertices are of the same type, and the relationships between vertices follow a consistent pattern. For instance, in the DBLP dataset, as mentioned, vertices only represent individuals in the research community, with edges between two vertices indicating co-authorship on at least one paper, so maximal cliques highlight closely connected research groups or frequent collaborators. 
% %
% Despite the applications in which the vertices are usually persons (i.e., social networks or collaboration networks), another interesting application of the maximal clique enumeration lies in frequent itemset mining, where it aids in identifying sets of products that are frequently purchased or appear together. In this context, the  transaction data is modeled as a graph, with each product represented as a node, and edges are formed between two nodes when the products are frequently bought together, typically based on a user-defined threshold for the number of transactions that include both products. A maximal clique in this graph signifies the group of products that are often co-purchased, uncovering strong associations that can inform strategies for product bundling, inventory management, and targeted marketing campaigns.



% In web graphs, maximal cliques similarly reveal interlinked clusters, often representing communities focused on specific topics or related content. For example, in the WebSK dataset, vertices represent web pages, and edges indicate hyperlinks between them. Maximal cliques in this dataset uncover tightly connected groups of pages, which benefits search engine optimization (SEO) and content analysis by identifying networks likely to share or amplify similar information, thereby impacting content ranking and information flow.
%
% One is in frequent itemset mining, where it aids in identifying sets of products that are frequently purchased or appear together. In this context, purchase data is modeled as a graph, with each product represented as a node, and edges are formed between two nodes when the products are frequently bought together, typically based on a user-defined threshold for the number of transactions that include both products. A maximal clique in this graph signifies the largest group of products that are often co-purchased, uncovering strong associations that can inform strategies for product bundling, inventory management, and targeted marketing campaigns.
%
% The other is widely used in computational biology to analyze large datasets, such as those from microarray experiments and protein-protein interaction (PPI) networks. In these networks, proteins or genes are represented as nodes, and edges represent interactions or regulatory relationships between them. Identifying maximal cliques in these graphs helps uncover groups of densely interacting proteins or co-regulated genes, often corresponding to protein complexes that play crucial roles in cellular processes like signal transduction and metabolism. These cliques provide biologically significant insights into the functioning of cells and assist in identifying molecular targets for drug discovery. 
% Algorithms such as the Bron-Kerbosch algorithm, including its improved versions, are used to efficiently enumerate maximal cliques in these complex biological networks. Their ability to handle dense graphs makes them particularly useful for high-throughput biological data analysis, revealing important gene expression patterns and protein complexes, which are vital for understanding diseases and developing new treatments.
 





\vspace{2mm}
M1. \textit{The numbers reported in the experimental section (in all the tables) should be right aligned so that readers can compare them easily at a glance.}

\vspace{1mm}
\textbf{Response:}
We followed the suggestion and right-aligned all tables in the experimental section. 

\vspace{2mm}
M2. \textit{A few typos, e.g., "satistics".} 


\vspace{1mm}
\textbf{Response:} Thank you for your careful checking. We have fixed the typo in the revised version and further proof-read the revised paper carefully.

==> cover-letter/thank.tex <==

% \textbf{We thank the reviewers for their constructive comments and suggestions, and have very carefully followed and cleaned up every raised issue. Apart from addressing these concerns, we have also further polished the manuscript. We provide a detailed account of the changes that we have made in response to comments that the reviewers have provided (shaded). The corresponding changes in the revised manuscript are colored in {\color{blue} blue}. }
\noindent
{\large
\textbf{Response to Reviewers of Paper Titled ``Maximal Clique Enumeration with Hybrid Branching and Early Termination'' (ICDE 2025 Paper ID = 196)}}
%\label{sec:response}

\smallskip\noindent Dear ICDE Meta-reviewer and Reviewers,

\smallskip
We would like to thank you for your constructive and inspiring comments. We have gone through these comments carefully and revised our draft accordingly. Below we summarize the major changes.

\begin{enumerate}
  \item We have included more details of Theorem~\ref{theo:hbbmc} to show the time complexity of \texttt{HBBMC}. The detailed proof can be found in the technical report~\cite{TR}.
  
  \item We have included how we check the condition for the early-termination technique, showing that the overhead is acceptable in Section~\ref{subsec:3-plex}. 
  
  \item We have included the descriptions {\chengC of} how we prepare the datasets in Table~\ref{tab:data} and Section~\ref{sec:exp}. 
  
  \item We have included more explanations on why the baseline \texttt{RRcd} performs well in Section~\ref{subsec:real-result}. 

  \item We have included more experimental results {\chengC of} ablation studies from different aspects in Section~\ref{subsec:real-result}. 

  \item We have included synthetic datasets generated by another graph generator model and presented the results in the technical report~\cite{TR}. 
\end{enumerate}
%}

% These major changes are highlighted in blue in the revised paper.
% Appended please find our detailed responses to both the reviewers' and meta-reviewer's comments.
% Thank you for your time reading them.

We highlight the major changes with the {\color{blue} blue} color in the revised manuscript. Appended please find our detailed responses to all reviewers' comments. We really appreciate your feedback and time.

\smallskip\noindent Yours sincerely, \\
Kaixin, Kaiqiang, Cheng
